Solving Without Stopping: On-Policy Distillation at Small Scale

On-policy distillation, where a student learns from a stronger teacher's feedback on its own outputs, is a common way to pass reasoning to smaller models. We analyze what it transfers at small scale, distilling Qwen3-8B into Qwen3 4B, 1.7B and 0.6B students, in thinking mode (reason at length, then end the reasoning and answer) and, for comparison, in non-thinking mode (no separate reasoning phase). Long reasoning needs two abilities, solving a problem and knowing when it is solved, and we find that distillation transfers the first, but in thinking mode not the second. Solving improves at every size, up to two ceilings, which we measure comprehensively across both modes and all student sizes: a student's single attempt never exceeds what it could already reach in many attempts before training, and the smaller the student, the further it stays below the teacher. Stopping is where the modes part. In non-thinking mode every student keeps stopping; in thinking mode students stop ending their reasoning early in training, and the smaller the student, the less of this ability survives: the teacher signals a stop almost only where a student already ends its reasoning, so distillation teaches no new stops; it only keeps the student's existing stops that land on a right answer, and a weak student has few such stops. The smallest students often reach the right value but do not commit to it: they either rarely mark it or mark it and write past it. Together, these results describe how small students behave under on-policy distillation, and a diagnostic that separates answer marking, correctness and stopping.

==> tables/app_behavior.tex <==
\begingroup
\scriptsize
\setlength{\tabcolsep}{2.6pt}
\setlength{\LTcapwidth}{\linewidth}
\begin{longtable}{>{\raggedright\arraybackslash}p{3.55cm}ccccccccccc@{}}
\caption{\textbf{How every model writes, closes and ends its answers, per benchmark.} \emph{Answer rate}:
fraction of samples that contain a marked answer (a \texttt{\textbackslash boxed\{\}} or an answer line).
\emph{Acc.\ given an answer}: lenient accuracy among those samples, unmatched (for comparisons between
models use the matched version, Table~\ref{tab:app-matched}); within a benchmark the lenient $p@1$ of
Table~\ref{tab:app-scores} equals the product of these two columns. \emph{Abandonment}: among samples that
contain a correct boxed answer, the fraction whose last boxed answer is wrong. \emph{Answers} and
\emph{distinct}: boxed answers and distinct boxed values per sample. \emph{Switches}: times consecutive boxed
answers change value within a sample. \emph{First answer at}: position of the first \texttt{\textbackslash
boxed\{\}} as a fraction of the sample's characters, among samples that have one. \emph{Closure}: fraction of
samples that emit \think; it is undefined for non-thinking models, whose thinking block is closed in the
prompt. \emph{Truncation}: fraction of samples that reach the evaluation cap. \emph{Tokens}: generated tokens,
mean and 90th percentile. $^\dagger$\,Evaluated with fewer samples: the officially post-trained 0.6B with 16 per problem on AIME 2026 and AMC23 and 4 on GSM8K-200; that model after 20 thinking steps and the 1{,}024-token run with 4 per problem, on GSM8K-200 only.}\label{tab:app-behavior}\\
\toprule
& Answer & Acc.\ given & Aban- & Answers & Distinct & Swit- & First & Clo- & Trun- & \multicolumn{2}{c}{Tokens} \\
\cmidrule(lr){11-12}
Model & rate & an answer & donment & /sample & /sample & ches & answer at & sure & cation & mean & p90 \\
\midrule
\endfirsthead
\multicolumn{12}{l}{\textit{Table~\ref{tab:app-behavior}, continued}}\\
\toprule
& Answer & Acc.\ given & Aban- & Answers & Distinct & Swit- & First & Clo- & Trun- & \multicolumn{2}{c}{Tokens} \\
\cmidrule(lr){11-12}
Model & rate & an answer & donment & /sample & /sample & ches & answer at & sure & cation & mean & p90 \\
\midrule
\endhead
\midrule
\multicolumn{12}{r}{\textit{continued on the next page}}\\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{12}{@{}l}{\textbf{AIME 2026}\quad 30 problems, 48 samples each, 30{,}720-token cap} \\*
Teacher (thinking) & 0.908 & 0.742 & 0.007 & 2.4 & 0.94 & 0.1 & 0.90 & 0.907 & 0.107 & 16,128 & 30,720 \\
Teacher (non-thinking) & 0.926 & 0.175 & 0.000 & 3.7 & 1.17 & 0.8 & 0.96 & -- & 0.081 & 5,756 & 11,874 \\
\addlinespace[2pt]
4B pretrained-only & 0.792 & 0.104 & 0.000 & 3.0 & 0.79 & 0.0 & 0.98 & -- & 0.158 & 6,326 & 30,720 \\
4B non-thinking route & 0.875 & 0.161 & 0.005 & 347.3 & 1.16 & 1.6 & 0.64 & -- & 0.441 & 15,222 & 30,720 \\
4B short-solution start & 0.463 & 0.319 & 0.000 & 2.2 & 0.47 & 0.0 & 0.81 & 0.453 & 0.546 & 18,883 & 30,720 \\
\quad + thinking route & 0.465 & 0.709 & 0.006 & 1.3 & 0.48 & 0.0 & 0.90 & 0.459 & 0.554 & 23,796 & 30,720 \\
4B teacher-solution start & 0.181 & 0.642 & 0.030 & 0.7 & 0.20 & 0.0 & 0.76 & 0.206 & 0.755 & 24,700 & 30,720 \\
\quad + thinking route & 0.469 & 0.673 & 0.011 & 1.4 & 0.49 & 0.1 & 0.90 & 0.466 & 0.557 & 24,067 & 30,720 \\
\quad + thinking route, 212 steps & 0.496 & 0.674 & 0.023 & 1.5 & 0.53 & 0.1 & 0.89 & 0.489 & 0.531 & 23,536 & 30,720 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.700 & 0.020 & 0.000 & 0.7 & 0.70 & 0.0 & 0.99 & -- & 0.222 & 7,811 & 30,720 \\
1.7B non-thinking route & 0.749 & 0.106 & 0.018 & 36.5 & 1.36 & 3.5 & 0.89 & -- & 0.308 & 12,117 & 30,720 \\
1.7B short-solution start & 0.360 & 0.081 & 0.048 & 2.7 & 0.39 & 0.0 & 0.79 & 0.333 & 0.660 & 21,436 & 30,720 \\
\quad + thinking route & 0.158 & 0.360 & 0.061 & 0.8 & 0.19 & 0.1 & 0.89 & 0.129 & 0.863 & 28,811 & 30,720 \\
1.7B teacher-solution start & 0.039 & 0.339 & 0.000 & 0.9 & 0.04 & 0.0 & 0.51 & 0.370 & 0.820 & 25,349 & 30,720 \\
\quad + thinking route & 0.139 & 0.485 & 0.536 & 71.5 & 0.65 & 1.2 & 0.53 & 0.000 & 1.000 & 30,720 & 30,720 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.208 & 0.020 & 0.500 & 27.0 & 7.02 & 8.1 & 0.77 & -- & 0.758 & 23,529 & 30,720 \\
0.6B non-thinking route & 0.639 & 0.028 & 0.038 & 19.6 & 0.94 & 2.3 & 0.88 & -- & 0.406 & 15,107 & 30,720 \\
0.6B short-solution start & 0.515 & 0.011 & 0.250 & 21.3 & 0.60 & 0.5 & 0.66 & 0.413 & 0.560 & 18,406 & 30,720 \\
\quad + thinking route & 0.149 & 0.023 & 0.400 & 1.0 & 0.16 & 0.1 & 0.87 & 0.085 & 0.884 & 29,212 & 30,720 \\
0.6B teacher-solution start & 0.032 & 0.043 & 0.500 & 3.8 & 0.04 & 0.3 & 0.50 & 0.294 & 0.849 & 26,170 & 30,720 \\
\quad + thinking route & 0.067 & 0.041 & 0.250 & 43.4 & 0.09 & 1.0 & 0.56 & 0.000 & 1.000 & 30,720 & 30,720 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 0.952 & 0.122 & 0.054 & 2.3 & 1.05 & 0.1 & 0.92 & 0.952 & 0.062 & 16,385 & 29,109 \\
\midrule
\multicolumn{12}{@{}l}{\textbf{AMC23}\quad 40 problems, 48 samples each, 30{,}720-token cap} \\*
Teacher (thinking) & 0.986 & 0.974 & 0.001 & 2.5 & 1.00 & 0.0 & 0.85 & 0.985 & 0.019 & 8,734 & 17,270 \\
Teacher (non-thinking) & 0.980 & 0.708 & 0.003 & 5.5 & 1.15 & 2.1 & 0.96 & -- & 0.031 & 2,601 & 3,990 \\
\addlinespace[2pt]
4B pretrained-only & 0.829 & 0.529 & 0.004 & 1.0 & 0.84 & 0.0 & 0.98 & -- & 0.150 & 5,566 & 30,720 \\
4B non-thinking route & 0.963 & 0.609 & 0.002 & 292.8 & 1.19 & 5.9 & 0.70 & -- & 0.280 & 9,690 & 30,720 \\
4B short-solution start & 0.758 & 0.723 & 0.003 & 2.5 & 0.77 & 0.0 & 0.79 & 0.747 & 0.252 & 10,313 & 30,720 \\
\quad + thinking route & 0.770 & 0.945 & 0.001 & 2.1 & 0.78 & 0.0 & 0.86 & 0.768 & 0.240 & 14,413 & 30,720 \\
4B teacher-solution start & 0.435 & 0.947 & 0.005 & 1.4 & 0.44 & 0.0 & 0.77 & 0.378 & 0.487 & 17,485 & 30,720 \\
\quad + thinking route & 0.772 & 0.943 & 0.003 & 2.2 & 0.79 & 0.0 & 0.86 & 0.769 & 0.242 & 14,743 & 30,720 \\
\quad + thinking route, 212 steps & 0.809 & 0.946 & 0.013 & 2.3 & 0.84 & 0.0 & 0.85 & 0.804 & 0.206 & 13,608 & 30,720 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.763 & 0.349 & 0.000 & 0.8 & 0.76 & 0.0 & 0.98 & -- & 0.169 & 5,897 & 30,720 \\
1.7B non-thinking route & 0.910 & 0.450 & 0.009 & 18.3 & 1.16 & 1.2 & 0.91 & -- & 0.115 & 5,362 & 30,720 \\
1.7B short-solution start & 0.609 & 0.491 & 0.012 & 2.3 & 0.64 & 0.0 & 0.79 & 0.558 & 0.404 & 14,015 & 30,720 \\
\quad + thinking route & 0.460 & 0.788 & 0.032 & 2.0 & 0.56 & 0.2 & 0.87 & 0.416 & 0.568 & 21,753 & 30,720 \\
1.7B teacher-solution start & 0.148 & 0.870 & 0.029 & 5.3 & 0.17 & 0.1 & 0.55 & 0.383 & 0.754 & 23,567 & 30,720 \\
\quad + thinking route & 0.446 & 0.833 & 0.516 & 334.5 & 3.13 & 5.2 & 0.30 & 0.000 & 1.000 & 30,720 & 30,720 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.205 & 0.260 & 0.029 & 8.4 & 1.10 & 1.3 & 0.79 & -- & 0.774 & 23,937 & 30,720 \\
0.6B non-thinking route & 0.850 & 0.327 & 0.006 & 12.1 & 1.13 & 2.1 & 0.91 & -- & 0.180 & 7,594 & 30,720 \\
0.6B short-solution start & 0.669 & 0.259 & 0.045 & 26.3 & 0.76 & 1.8 & 0.68 & 0.559 & 0.406 & 13,965 & 30,720 \\
\quad + thinking route & 0.356 & 0.595 & 0.052 & 4.2 & 0.39 & 0.1 & 0.85 & 0.232 & 0.706 & 25,343 & 30,720 \\
0.6B teacher-solution start & 0.070 & 0.410 & 0.148 & 7.0 & 0.12 & 0.1 & 0.50 & 0.323 & 0.834 & 25,810 & 30,720 \\
\quad + thinking route & 0.252 & 0.653 & 0.172 & 259.8 & 0.34 & 0.6 & 0.39 & 0.000 & 1.000 & 30,720 & 30,720 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 0.983 & 0.513 & 0.028 & 2.4 & 1.04 & 0.1 & 0.87 & 0.983 & 0.017 & 10,182 & 21,589 \\
\midrule
\multicolumn{12}{@{}l}{\textbf{GSM8K-200}\quad 200 problems, 32 samples each, 8{,}192-token cap} \\*
Teacher (thinking) & 0.993 & 0.944 & 0.002 & 2.3 & 1.01 & 0.1 & 0.81 & 0.993 & 0.009 & 2,269 & 4,367 \\
Teacher (non-thinking) & 1.000 & 0.929 & 0.001 & 1.3 & 1.02 & 0.0 & 0.93 & -- & 0.000 & 308 & 450 \\
\addlinespace[2pt]
4B pretrained-only & 0.871 & 0.874 & 0.001 & 1.4 & 0.86 & 0.0 & 0.96 & -- & 0.090 & 987 & 592 \\
4B non-thinking route & 1.000 & 0.919 & 0.002 & 2.6 & 1.09 & 0.2 & 0.85 & -- & 0.006 & 393 & 505 \\
4B short-solution start & 0.980 & 0.918 & 0.001 & 2.7 & 0.99 & 0.4 & 0.80 & 0.978 & 0.022 & 1,241 & 1,746 \\
\quad + thinking route & 0.951 & 0.943 & 0.001 & 2.3 & 0.98 & 0.1 & 0.87 & 0.949 & 0.059 & 3,478 & 6,368 \\
4B teacher-solution start & 0.484 & 0.953 & 0.001 & 1.3 & 0.49 & 0.0 & 0.80 & 0.417 & 0.430 & 4,792 & 8,192 \\
\quad + thinking route & 0.962 & 0.939 & 0.015 & 2.3 & 1.00 & 0.1 & 0.86 & 0.961 & 0.054 & 3,458 & 6,424 \\
\quad + thinking route, 212 steps & 0.970 & 0.943 & 0.063 & 2.5 & 1.13 & 0.2 & 0.82 & 0.968 & 0.067 & 3,179 & 6,609 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.792 & 0.758 & 0.000 & 0.8 & 0.79 & 0.0 & 0.97 & -- & 0.043 & 626 & 461 \\
1.7B non-thinking route & 0.999 & 0.831 & 0.000 & 1.5 & 1.10 & 0.1 & 0.89 & -- & 0.001 & 379 & 515 \\
1.7B short-solution start & 0.911 & 0.820 & 0.013 & 2.3 & 0.96 & 0.1 & 0.81 & 0.866 & 0.096 & 1,828 & 3,450 \\
\quad + thinking route & 0.828 & 0.915 & 0.002 & 2.2 & 0.85 & 0.1 & 0.90 & 0.808 & 0.190 & 4,866 & 8,192 \\
1.7B teacher-solution start & 0.267 & 0.908 & 0.022 & 1.9 & 0.29 & 0.2 & 0.67 & 0.438 & 0.643 & 5,680 & 8,192 \\
\quad + thinking route & 0.811 & 0.916 & 0.259 & 150.7 & 1.62 & 1.4 & 0.49 & 0.000 & 1.000 & 8,192 & 8,192 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.169 & 0.518 & 0.009 & 2.9 & 0.56 & 0.6 & 0.83 & -- & 0.811 & 6,710 & 8,192 \\
0.6B non-thinking route & 0.992 & 0.694 & 0.002 & 1.9 & 1.10 & 0.2 & 0.90 & -- & 0.010 & 545 & 811 \\
0.6B short-solution start & 0.831 & 0.644 & 0.019 & 4.5 & 0.92 & 0.3 & 0.76 & 0.697 & 0.209 & 2,632 & 8,192 \\
\quad + thinking route & 0.758 & 0.879 & 0.020 & 3.1 & 0.79 & 0.1 & 0.87 & 0.705 & 0.291 & 5,494 & 8,192 \\
0.6B teacher-solution start & 0.165 & 0.820 & 0.066 & 5.0 & 0.19 & 0.1 & 0.59 & 0.350 & 0.758 & 6,409 & 8,192 \\
\quad + thinking route & 0.681 & 0.910 & 0.119 & 147.7 & 0.79 & 0.6 & 0.54 & 0.000 & 1.000 & 8,192 & 8,192 \\
\addlinespace[2pt]
0.6B short-solution start, 1{,}024-token budget$^\dagger$ & 0.670 & 0.827 & 0.009 & 10.8 & 0.69 & 0.1 & 0.70 & 0.259 & 0.534 & 6,173 & 8,192 \\
officially post-trained 0.6B$^\dagger$ & 0.975 & 0.797 & 0.008 & 2.3 & 1.00 & 0.1 & 0.80 & 0.975 & 0.030 & 2,136 & 5,147 \\
\quad + 20 thinking steps (16{,}384)$^\dagger$ & 0.884 & 0.857 & 0.002 & 2.3 & 0.90 & 0.2 & 0.85 & 0.877 & 0.131 & 3,964 & 8,192 \\
\midrule
\multicolumn{12}{@{}l}{\textbf{Mean of the three}\quad unweighted mean over AIME 2026, AMC23 and GSM8K-200} \\*
Teacher (thinking) & 0.962 & 0.887 & 0.004 & 2.4 & 0.98 & 0.1 & 0.85 & 0.962 & 0.045 & 9,044 & 17,452 \\
Teacher (non-thinking) & 0.969 & 0.604 & 0.001 & 3.5 & 1.11 & 1.0 & 0.95 & -- & 0.037 & 2,888 & 5,438 \\
\addlinespace[2pt]
4B pretrained-only & 0.830 & 0.502 & 0.002 & 1.8 & 0.83 & 0.0 & 0.97 & -- & 0.133 & 4,293 & 20,677 \\
4B non-thinking route & 0.946 & 0.563 & 0.003 & 214.3 & 1.15 & 2.6 & 0.73 & -- & 0.242 & 8,435 & 20,648 \\
4B short-solution start & 0.734 & 0.653 & 0.001 & 2.5 & 0.74 & 0.2 & 0.80 & 0.726 & 0.274 & 10,146 & 21,062 \\
\quad + thinking route & 0.728 & 0.866 & 0.003 & 1.9 & 0.75 & 0.0 & 0.88 & 0.725 & 0.284 & 13,896 & 22,603 \\
4B teacher-solution start & 0.366 & 0.848 & 0.012 & 1.1 & 0.38 & 0.0 & 0.78 & 0.333 & 0.557 & 15,659 & 23,211 \\
\quad + thinking route & 0.734 & 0.852 & 0.010 & 1.9 & 0.76 & 0.0 & 0.87 & 0.732 & 0.284 & 14,089 & 22,621 \\
\quad + thinking route, 212 steps & 0.758 & 0.854 & 0.033 & 2.1 & 0.83 & 0.1 & 0.85 & 0.753 & 0.268 & 13,441 & 22,683 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.752 & 0.376 & 0.000 & 0.8 & 0.75 & 0.0 & 0.98 & -- & 0.145 & 4,778 & 20,634 \\
1.7B non-thinking route & 0.886 & 0.462 & 0.009 & 18.8 & 1.21 & 1.6 & 0.90 & -- & 0.141 & 5,953 & 20,652 \\
1.7B short-solution start & 0.627 & 0.464 & 0.024 & 2.5 & 0.66 & 0.1 & 0.79 & 0.585 & 0.387 & 12,426 & 21,630 \\
\quad + thinking route & 0.482 & 0.688 & 0.032 & 1.7 & 0.53 & 0.1 & 0.89 & 0.451 & 0.540 & 18,477 & 23,211 \\
1.7B teacher-solution start & 0.151 & 0.706 & 0.017 & 2.7 & 0.17 & 0.1 & 0.58 & 0.397 & 0.739 & 18,199 & 23,211 \\
\quad + thinking route & 0.466 & 0.745 & 0.437 & 185.5 & 1.80 & 2.6 & 0.44 & 0.000 & 1.000 & 23,211 & 23,211 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.194 & 0.266 & 0.179 & 12.8 & 2.89 & 3.3 & 0.80 & -- & 0.781 & 18,059 & 23,211 \\
0.6B non-thinking route & 0.827 & 0.350 & 0.015 & 11.2 & 1.06 & 1.6 & 0.90 & -- & 0.199 & 7,749 & 20,750 \\
0.6B short-solution start & 0.672 & 0.304 & 0.105 & 17.4 & 0.76 & 0.8 & 0.70 & 0.556 & 0.392 & 11,668 & 23,211 \\
\quad + thinking route & 0.421 & 0.499 & 0.157 & 2.8 & 0.45 & 0.1 & 0.86 & 0.340 & 0.627 & 20,016 & 23,211 \\
0.6B teacher-solution start & 0.089 & 0.425 & 0.238 & 5.3 & 0.12 & 0.2 & 0.53 & 0.323 & 0.814 & 19,463 & 23,211 \\
\quad + thinking route & 0.333 & 0.535 & 0.180 & 150.3 & 0.41 & 0.7 & 0.50 & 0.000 & 1.000 & 23,211 & 23,211 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 0.970 & 0.478 & 0.030 & 2.3 & 1.03 & 0.1 & 0.86 & 0.970 & 0.037 & 9,568 & 18,615 \\
\end{longtable}
\endgroup



==> tables/app_cases.tex <==
\begin{table}[p]
\centering
\caption{\textbf{Every evaluation sample in one of five cases by its marked answers, per benchmark and model.} A marked
answer is a \texttt{\textbackslash boxed\{\}} or an \emph{Answer:} / \emph{final answer is} line anywhere in the
output. \emph{One value, right}: every marked answer has the same value, and it is correct; \emph{several values,
last right}: the last one is correct; \emph{right, then overwritten}: a correct value was marked but the last marked
one is wrong; \emph{only wrong}: no marked value is correct. The first three sum to lenient $p@1$. \emph{No marked
answer, and truncated}: the share of all samples that have no marked answer and reached the evaluation cap; after
thinking-route distillation it equals the no-answer share on every benchmark. Figure~\ref{fig:cases} shows the
three-benchmark means. Names as in Table~\ref{tab:app-scores}.
$^\dagger$\,Fewer samples: the officially post-trained 0.6B with 16 per problem on AIME 2026 and AMC23 and 4 on GSM8K-200; that model after 20 thinking steps and the 1{,}024-token run with 4 per problem, on GSM8K-200 only.}
\label{tab:app-cases}
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lcccccc@{}}
\toprule
& \multicolumn{3}{c}{a right answer was marked (lenient $p@1$)} & & \multicolumn{2}{c}{no marked answer} \\
\cmidrule(lr){2-4}\cmidrule(lr){6-7}
Model & \makecell{one value,\\right} & \makecell{several values,\\last right} & \makecell{right, then\\overwritten} & \makecell{only\\wrong} & all & \makecell{and\\truncated} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{AIME 2026}\quad 30 problems, 30{,}720-token cap} \\*
Teacher (thinking) & 0.665 & 0.005 & 0.005 & 0.234 & 0.092 & 0.092 \\
Teacher (non-thinking) & 0.147 & 0.015 & 0.000 & 0.763 & 0.074 & 0.074 \\
\addlinespace[2pt]
4B pretrained-only & 0.083 & 0.000 & 0.000 & 0.709 & 0.208 & 0.150 \\
4B non-thinking route & 0.122 & 0.018 & 0.001 & 0.734 & 0.125 & 0.125 \\
4B short-solution start & 0.148 & 0.000 & 0.000 & 0.315 & 0.537 & 0.537 \\
\quad + thinking route & 0.324 & 0.003 & 0.002 & 0.135 & 0.535 & 0.535 \\
4B teacher-solution start & 0.110 & 0.003 & 0.004 & 0.065 & 0.819 & 0.740 \\
\quad + thinking route & 0.306 & 0.006 & 0.004 & 0.153 & 0.531 & 0.531 \\
\quad + thinking route, 212 steps & 0.322 & 0.004 & 0.008 & 0.162 & 0.504 & 0.504 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.014 & 0.000 & 0.000 & 0.686 & 0.300 & 0.220 \\
1.7B non-thinking route & 0.068 & 0.010 & 0.001 & 0.669 & 0.251 & 0.251 \\
1.7B short-solution start & 0.026 & 0.001 & 0.001 & 0.331 & 0.640 & 0.640 \\
\quad + thinking route & 0.050 & 0.004 & 0.004 & 0.101 & 0.842 & 0.842 \\
1.7B teacher-solution start & 0.011 & 0.002 & 0.000 & 0.026 & 0.961 & 0.801 \\
\quad + thinking route & 0.029 & 0.003 & 0.036 & 0.071 & 0.861 & 0.861 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.002 & 0.000 & 0.002 & 0.204 & 0.792 & 0.745 \\
0.6B non-thinking route & 0.013 & 0.004 & 0.001 & 0.621 & 0.361 & 0.361 \\
0.6B short-solution start & 0.004 & 0.001 & 0.001 & 0.509 & 0.485 & 0.485 \\
\quad + thinking route & 0.002 & 0.000 & 0.001 & 0.145 & 0.851 & 0.851 \\
0.6B teacher-solution start & 0.001 & 0.000 & 0.001 & 0.031 & 0.968 & 0.835 \\
\quad + thinking route & 0.002 & 0.000 & 0.001 & 0.065 & 0.933 & 0.933 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 0.108 & 0.002 & 0.006 & 0.835 & 0.048 & 0.048 \\
\midrule
\multicolumn{7}{@{}l}{\textbf{AMC23}\quad 40 problems, 30{,}720-token cap} \\*
Teacher (thinking) & 0.950 & 0.009 & 0.001 & 0.026 & 0.014 & 0.014 \\
Teacher (non-thinking) & 0.622 & 0.069 & 0.002 & 0.286 & 0.020 & 0.020 \\
\addlinespace[2pt]
4B pretrained-only & 0.435 & 0.001 & 0.002 & 0.391 & 0.171 & 0.147 \\
4B non-thinking route & 0.490 & 0.096 & 0.001 & 0.376 & 0.037 & 0.037 \\
4B short-solution start & 0.544 & 0.003 & 0.002 & 0.210 & 0.242 & 0.242 \\
\quad + thinking route & 0.721 & 0.006 & 0.001 & 0.042 & 0.230 & 0.230 \\
4B teacher-solution start & 0.406 & 0.004 & 0.002 & 0.023 & 0.565 & 0.474 \\
\quad + thinking route & 0.719 & 0.007 & 0.002 & 0.044 & 0.228 & 0.228 \\
\quad + thinking route, 212 steps & 0.747 & 0.009 & 0.010 & 0.044 & 0.191 & 0.191 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.265 & 0.002 & 0.000 & 0.497 & 0.237 & 0.167 \\
1.7B non-thinking route & 0.354 & 0.053 & 0.004 & 0.500 & 0.090 & 0.090 \\
1.7B short-solution start & 0.290 & 0.006 & 0.004 & 0.310 & 0.391 & 0.391 \\
\quad + thinking route & 0.307 & 0.044 & 0.011 & 0.097 & 0.540 & 0.540 \\
1.7B teacher-solution start & 0.116 & 0.009 & 0.004 & 0.019 & 0.852 & 0.697 \\
\quad + thinking route & 0.162 & 0.018 & 0.192 & 0.074 & 0.554 & 0.554 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.050 & 0.002 & 0.002 & 0.152 & 0.795 & 0.759 \\
0.6B non-thinking route & 0.216 & 0.060 & 0.002 & 0.572 & 0.150 & 0.150 \\
0.6B short-solution start & 0.145 & 0.020 & 0.008 & 0.496 & 0.331 & 0.331 \\
\quad + thinking route & 0.183 & 0.019 & 0.010 & 0.144 & 0.644 & 0.644 \\
0.6B teacher-solution start & 0.022 & 0.003 & 0.004 & 0.041 & 0.930 & 0.805 \\
\quad + thinking route & 0.120 & 0.019 & 0.026 & 0.087 & 0.748 & 0.748 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 0.477 & 0.014 & 0.014 & 0.478 & 0.017 & 0.017 \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[p]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
{\small\textit{Table~\ref{tab:app-cases}, continued: five answer cases, GSM8K-200.}}\par\medskip
\begin{tabular}{@{}lcccccc@{}}
\toprule
& \multicolumn{3}{c}{a right answer was marked (lenient $p@1$)} & & \multicolumn{2}{c}{no marked answer} \\
\cmidrule(lr){2-4}\cmidrule(lr){6-7}
Model & \makecell{one value,\\right} & \makecell{several values,\\last right} & \makecell{right, then\\overwritten} & \makecell{only\\wrong} & all & \makecell{and\\truncated} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{GSM8K-200}\quad 200 problems, 8{,}192-token cap} \\*
Teacher (thinking) & 0.930 & 0.005 & 0.002 & 0.056 & 0.007 & 0.007 \\
Teacher (non-thinking) & 0.915 & 0.013 & 0.001 & 0.071 & 0.000 & 0.000 \\
\addlinespace[2pt]
4B pretrained-only & 0.755 & 0.005 & 0.001 & 0.110 & 0.129 & 0.080 \\
4B non-thinking route & 0.864 & 0.053 & 0.002 & 0.081 & 0.000 & 0.000 \\
4B short-solution start & 0.897 & 0.002 & 0.001 & 0.081 & 0.020 & 0.020 \\
\quad + thinking route & 0.878 & 0.018 & 0.001 & 0.054 & 0.050 & 0.050 \\
4B teacher-solution start & 0.453 & 0.007 & 0.001 & 0.023 & 0.516 & 0.416 \\
\quad + thinking route & 0.879 & 0.011 & 0.014 & 0.059 & 0.038 & 0.038 \\
\quad + thinking route, 212 steps & 0.845 & 0.012 & 0.058 & 0.056 & 0.030 & 0.030 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.599 & 0.002 & 0.000 & 0.191 & 0.208 & 0.042 \\
1.7B non-thinking route & 0.778 & 0.052 & 0.000 & 0.169 & 0.001 & 0.001 \\
1.7B short-solution start & 0.722 & 0.015 & 0.010 & 0.164 & 0.089 & 0.088 \\
\quad + thinking route & 0.745 & 0.011 & 0.001 & 0.071 & 0.172 & 0.172 \\
1.7B teacher-solution start & 0.229 & 0.008 & 0.005 & 0.025 & 0.733 & 0.571 \\
\quad + thinking route & 0.534 & 0.017 & 0.192 & 0.068 & 0.189 & 0.189 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.083 & 0.003 & 0.001 & 0.081 & 0.831 & 0.801 \\
0.6B non-thinking route & 0.647 & 0.040 & 0.001 & 0.304 & 0.008 & 0.008 \\
0.6B short-solution start & 0.493 & 0.032 & 0.010 & 0.296 & 0.169 & 0.167 \\
\quad + thinking route & 0.646 & 0.008 & 0.013 & 0.092 & 0.242 & 0.242 \\
\quad + thinking route, 1{,}024-token budget$^\dagger$ & 0.537 & 0.011 & 0.005 & 0.116 & 0.330 & 0.330 \\
0.6B teacher-solution start & 0.120 & 0.006 & 0.009 & 0.030 & 0.835 & 0.703 \\
\quad + thinking route & 0.507 & 0.038 & 0.074 & 0.061 & 0.319 & 0.319 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 0.762 & 0.009 & 0.006 & 0.198 & 0.025 & 0.025 \\
\quad + 20 thinking steps (16{,}384-token budget)$^\dagger$ & 0.752 & 0.004 & 0.001 & 0.126 & 0.116 & 0.116 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_ceiling.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{Per benchmark, no distilled student's lenient $p@1$ exceeds its own starting lenient $p@n$, and that
starting $p@n$ mostly does not move.} Lenient scoring; $p@n$ over $n=48$ samples on AIME 2026 and AMC23 and 32 on
GSM8K-200. \emph{Start}: the pretrained-only student (non-thinking route) or the cold-started student (thinking
routes); \emph{after}: that student after distillation. (a)~Left: after $p@1$ minus start $p@n$, paired problem
bootstrap ($B=10{,}000$), 95\% percentile interval. Every difference is below zero; the interval contains zero in
four cells, all on AIME 2026 (the 4B on both thinking routes, the 1.7B and 0.6B from the teacher's own solutions).
Right: the ratio of the two; its maximum over all 27 cells is 0.96. (b)~Lenient $p@n$ before $\to$ after, and the
change with its paired bootstrap interval. Only three changes reach $+0.2$: the 4B thinking routes on AIME 2026 and
the pretrained-only 0.6B on GSM8K-200, a start that rarely marks an answer. Three-benchmark means:
Table~\ref{tab:ceiling}.}
\label{tab:app-ceiling}
\scriptsize
\setlength{\tabcolsep}{4pt}
{\small (a) After $p@1$ against start $p@n$}\par\smallskip
\begin{tabular}{@{}lcccccc@{}}
\toprule
& \multicolumn{3}{c}{after $p@1$ $-$ start $p@n$ [95\% CI]} & \multicolumn{3}{c}{after $p@1$ / start $p@n$} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Student & AIME 2026 & AMC23 & GSM8K-200 & AIME 2026 & AMC23 & GSM8K-200 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Non-thinking route}} \\
\quad 4B & \makecell{$-0.192$\\$[-0.328, -0.075]$} & \makecell{$-0.314$\\$[-0.421, -0.210]$} & \makecell{$-0.056$\\$[-0.084, -0.032]$} & 0.42 & 0.65 & 0.94 \\
\quad 1.7B & \makecell{$-0.054$\\$[-0.125, -0.002]$} & \makecell{$-0.415$\\$[-0.538, -0.296]$} & \makecell{$-0.150$\\$[-0.188, -0.114]$} & 0.59 & 0.50 & 0.85 \\
\quad 0.6B & \makecell{$-0.149$\\$[-0.283, -0.032]$} & \makecell{$-0.347$\\$[-0.473, -0.222]$} & \makecell{$-0.056$\\$[-0.106, -0.008]$} & 0.11 & 0.44 & 0.92 \\
\addlinespace[3pt]
\multicolumn{7}{@{}l}{\textit{Thinking route, short external solutions}} \\
\quad 4B & \makecell{$-0.071$\\$[-0.176, +0.023]$} & \makecell{$-0.197$\\$[-0.294, -0.112]$} & \makecell{$-0.084$\\$[-0.114, -0.056]$} & 0.82 & 0.79 & 0.91 \\
\quad 1.7B & \makecell{$-0.176$\\$[-0.311, -0.063]$} & \makecell{$-0.412$\\$[-0.550, -0.282]$} & \makecell{$-0.228$\\$[-0.270, -0.187]$} & 0.24 & 0.47 & 0.77 \\
\quad 0.6B & \makecell{$-0.163$\\$[-0.296, -0.033]$} & \makecell{$-0.463$\\$[-0.602, -0.328]$} & \makecell{$-0.263$\\$[-0.315, -0.214]$} & 0.02 & 0.31 & 0.72 \\
\addlinespace[3pt]
\multicolumn{7}{@{}l}{\textit{Thinking route, teacher's own solutions}} \\
\quad 4B & \makecell{$-0.084$\\$[-0.185, +0.003]$} & \makecell{$-0.172$\\$[-0.265, -0.090]$} & \makecell{$-0.042$\\$[-0.074, -0.011]$} & 0.79 & 0.81 & 0.96 \\
\quad 1.7B & \makecell{$-0.033$\\$[-0.102, +0.019]$} & \makecell{$-0.178$\\$[-0.289, -0.082]$} & \makecell{$-0.157$\\$[-0.194, -0.121]$} & 0.67 & 0.68 & 0.83 \\
\quad 0.6B & \makecell{$-0.031$\\$[-0.094, +0.002]$} & \makecell{$-0.235$\\$[-0.359, -0.124]$} & \makecell{$-0.145$\\$[-0.191, -0.100]$} & 0.08 & 0.41 & 0.81 \\
\bottomrule
\end{tabular}
\par\medskip
{\small (b) Does the start's $p@n$ move? Lenient $p@n$, start $\to$ after, and the change [95\% CI]}\par\smallskip
\begin{tabular}{@{}lcccc@{}}
\toprule
Student & AIME 2026 & AMC23 & GSM8K-200 & three-benchmark mean \\
\midrule
\multicolumn{5}{@{}l}{\textit{Non-thinking route}} \\
\quad 4B & \makecell{0.333\,$\to$\,0.467\\$+0.133$ $[+0.033, +0.267]$} & \makecell{0.900\,$\to$\,0.925\\$+0.025$ $[+0.000, +0.075]$} & \makecell{0.975\,$\to$\,0.980\\$+0.005$ $[-0.015, +0.030]$} & \makecell{0.736\,$\to$\,0.791\\$+0.054$ $[+0.014, +0.102]$} \\
\quad 1.7B & \makecell{0.133\,$\to$\,0.300\\$+0.167$ $[+0.033, +0.300]$} & \makecell{0.825\,$\to$\,0.900\\$+0.075$ $[-0.025, +0.175]$} & \makecell{0.980\,$\to$\,0.975\\$-0.005$ $[-0.025, +0.015]$} & \makecell{0.646\,$\to$\,0.725\\$+0.079$ $[+0.024, +0.139]$} \\
\quad 0.6B & \makecell{0.167\,$\to$\,0.133\\$-0.033$ $[-0.167, +0.100]$} & \makecell{0.625\,$\to$\,0.700\\$+0.075$ $[-0.075, +0.225]$} & \makecell{0.745\,$\to$\,0.945\\$+0.200$ $[+0.145, +0.260]$} & \makecell{0.512\,$\to$\,0.593\\$+0.081$ $[+0.008, +0.151]$} \\
\addlinespace[3pt]
\multicolumn{5}{@{}l}{\textit{Thinking route, short external solutions}} \\
\quad 4B & \makecell{0.400\,$\to$\,0.700\\$+0.300$ $[+0.133, +0.467]$} & \makecell{0.925\,$\to$\,0.900\\$-0.025$ $[-0.075, +0.000]$} & \makecell{0.980\,$\to$\,0.965\\$-0.015$ $[-0.035, +0.000]$} & \makecell{0.768\,$\to$\,0.855\\$+0.087$ $[+0.031, +0.147]$} \\
\quad 1.7B & \makecell{0.233\,$\to$\,0.200\\$-0.033$ $[-0.100, +0.000]$} & \makecell{0.775\,$\to$\,0.725\\$-0.050$ $[-0.175, +0.075]$} & \makecell{0.985\,$\to$\,0.960\\$-0.025$ $[-0.055, +0.000]$} & \makecell{0.664\,$\to$\,0.628\\$-0.036$ $[-0.084, +0.008]$} \\
\quad 0.6B & \makecell{0.167\,$\to$\,0.067\\$-0.100$ $[-0.200, +0.000]$} & \makecell{0.675\,$\to$\,0.600\\$-0.075$ $[-0.250, +0.075]$} & \makecell{0.930\,$\to$\,0.895\\$-0.035$ $[-0.075, +0.005]$} & \makecell{0.591\,$\to$\,0.521\\$-0.070$ $[-0.137, -0.007]$} \\
\addlinespace[3pt]
\multicolumn{5}{@{}l}{\textit{Thinking route, teacher's own solutions}} \\
\quad 4B & \makecell{0.400\,$\to$\,0.733\\$+0.333$ $[+0.167, +0.500]$} & \makecell{0.900\,$\to$\,0.950\\$+0.050$ $[+0.000, +0.125]$} & \makecell{0.945\,$\to$\,0.965\\$+0.020$ $[+0.005, +0.040]$} & \makecell{0.748\,$\to$\,0.883\\$+0.134$ $[+0.075, +0.198]$} \\
\quad 1.7B & \makecell{0.100\,$\to$\,0.233\\$+0.133$ $[+0.033, +0.267]$} & \makecell{0.550\,$\to$\,0.675\\$+0.125$ $[+0.000, +0.250]$} & \makecell{0.900\,$\to$\,0.950\\$+0.050$ $[+0.015, +0.090]$} & \makecell{0.517\,$\to$\,0.619\\$+0.103$ $[+0.047, +0.165]$} \\
\quad 0.6B & \makecell{0.033\,$\to$\,0.067\\$+0.033$ $[+0.000, +0.100]$} & \makecell{0.400\,$\to$\,0.475\\$+0.075$ $[-0.050, +0.200]$} & \makecell{0.765\,$\to$\,0.880\\$+0.115$ $[+0.065, +0.170]$} & \makecell{0.399\,$\to$\,0.474\\$+0.074$ $[+0.025, +0.127]$} \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_ci.tex <==
\begin{landscape}
\begingroup
\footnotesize
\setlength{\tabcolsep}{5pt}
\setlength{\LTcapwidth}{\linewidth}
\begin{longtable}{@{}lcccccc@{}}
\caption{\textbf{Every paired interval on the three-benchmark mean.} Paired, problem-level bootstrap:
problems are resampled with replacement within each benchmark, the same draw is used for both models of a
pair, each metric is computed per benchmark and the three are averaged without weights; 10{,}000 resamples,
95\% percentile intervals. The first three blocks follow each route from its start (A) to its endpoint (B);
the next two compare the two routes head to head at equal size; the sixth sets each pretrained-only student
against the non-thinking route one size smaller; the last compares the two thinking starts after distillation.
\emph{Accuracy given an answer, matched} is computed on the problems both models answered at least once,
weighting problems equally, so A and B there are the matched values. The GPQA-Diamond rows exist for
non-thinking models only and use the choice-aware scorer on committed and strict scoring, never lenient;
GPQA-Diamond is never averaged with the open-ended benchmarks. Intervals that contain 0 are set in grey: those
pairs are indistinguishable.}\label{tab:app-ci}\\
\toprule
& \multicolumn{2}{c}{4B} & \multicolumn{2}{c}{1.7B} & \multicolumn{2}{c}{0.6B} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Metric & A $\to$ B & B $-$ A [95\% CI] & A $\to$ B & B $-$ A [95\% CI] & A $\to$ B & B $-$ A [95\% CI] \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{Table~\ref{tab:app-ci}, continued}}\\
\toprule
& \multicolumn{2}{c}{4B} & \multicolumn{2}{c}{1.7B} & \multicolumn{2}{c}{0.6B} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Metric & A $\to$ B & B $-$ A [95\% CI] & A $\to$ B & B $-$ A [95\% CI] & A $\to$ B & B $-$ A [95\% CI] \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{\textit{continued on the next page}}\\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{7}{@{}l}{\textbf{Pretrained-only start (A) $\to$ non-thinking route (B)}} \\*
answer rate & 0.830\,$\to$\,0.946 & $+0.115$ $[+0.088, +0.143]$ & 0.752\,$\to$\,0.886 & $+0.134$ $[+0.106, +0.161]$ & 0.194\,$\to$\,0.827 & $+0.633$ $[+0.598, +0.667]$ \\
matched accuracy (marked) & 0.491\,$\to$\,0.554 & $+0.063$ $[+0.041, +0.088]$ & 0.371\,$\to$\,0.451 & $+0.080$ $[+0.054, +0.111]$ & 0.248\,$\to$\,0.340 & $+0.092$ $[+0.065, +0.118]$ \\
lenient $p@1$ & 0.427\,$\to$\,0.549 & $+0.121$ $[+0.097, +0.149]$ & 0.294\,$\to$\,0.440 & $+0.146$ $[+0.118, +0.177]$ & 0.048\,$\to$\,0.328 & $+0.280$ $[+0.249, +0.310]$ \\
lenient $p@n$ & 0.736\,$\to$\,0.791 & $+0.054$ $[+0.014, +0.102]$ & 0.646\,$\to$\,0.725 & $+0.079$ $[+0.024, +0.139]$ & 0.512\,$\to$\,0.593 & $+0.081$ $[+0.008, +0.151]$ \\
maj@$n$ & 0.553\,$\to$\,0.599 & \textcolor{cMuted!70}{$+0.046$ $[-0.016, +0.111]$} & 0.481\,$\to$\,0.519 & $+0.039$ $[+0.003, +0.082]$ & 0.344\,$\to$\,0.449 & $+0.104$ $[+0.052, +0.159]$ \\
committed $p@1$ & 0.426\,$\to$\,0.547 & $+0.121$ $[+0.097, +0.148]$ & 0.293\,$\to$\,0.438 & $+0.145$ $[+0.118, +0.176]$ & 0.047\,$\to$\,0.327 & $+0.280$ $[+0.250, +0.311]$ \\
strict $p@1$ & 0.426\,$\to$\,0.505 & $+0.080$ $[+0.058, +0.103]$ & 0.294\,$\to$\,0.437 & $+0.143$ $[+0.116, +0.174]$ & 0.046\,$\to$\,0.327 & $+0.280$ $[+0.250, +0.311]$ \\
GPQA-Diamond, committed $p@1$ & 0.157\,$\to$\,0.397 & $+0.239$ $[+0.198, +0.282]$ & 0.191\,$\to$\,0.275 & $+0.084$ $[+0.050, +0.117]$ & 0.049\,$\to$\,0.234 & $+0.185$ $[+0.155, +0.215]$ \\
GPQA-Diamond, strict $p@1$ & 0.157\,$\to$\,0.361 & $+0.204$ $[+0.163, +0.247]$ & 0.189\,$\to$\,0.270 & $+0.081$ $[+0.048, +0.114]$ & 0.049\,$\to$\,0.233 & $+0.184$ $[+0.155, +0.214]$ \\
GPQA-Diamond, committed $p@n$ & 0.606\,$\to$\,0.798 & $+0.192$ $[+0.126, +0.258]$ & 0.651\,$\to$\,0.717 & \textcolor{cMuted!70}{$+0.066$ $[-0.010, +0.136]$} & 0.288\,$\to$\,0.732 & $+0.444$ $[+0.364, +0.520]$ \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Short-solution start (A) $\to$ thinking route (B)}} \\*
answer rate & 0.734\,$\to$\,0.728 & \textcolor{cMuted!70}{$-0.006$ $[-0.043, +0.033]$} & 0.627\,$\to$\,0.482 & $-0.145$ $[-0.180, -0.110]$ & 0.672\,$\to$\,0.421 & $-0.251$ $[-0.290, -0.210]$ \\
matched accuracy (marked) & 0.584\,$\to$\,0.773 & $+0.190$ $[+0.142, +0.243]$ & 0.439\,$\to$\,0.545 & $+0.106$ $[+0.072, +0.145]$ & 0.286\,$\to$\,0.402 & $+0.115$ $[+0.089, +0.142]$ \\
lenient $p@1$ & 0.532\,$\to$\,0.651 & $+0.119$ $[+0.083, +0.158]$ & 0.358\,$\to$\,0.392 & $+0.034$ $[+0.013, +0.057]$ & 0.238\,$\to$\,0.294 & $+0.056$ $[+0.035, +0.077]$ \\
lenient $p@n$ & 0.768\,$\to$\,0.855 & $+0.087$ $[+0.031, +0.147]$ & 0.664\,$\to$\,0.628 & \textcolor{cMuted!70}{$-0.036$ $[-0.084, +0.008]$} & 0.591\,$\to$\,0.521 & $-0.070$ $[-0.137, -0.007]$ \\
maj@$n$ & 0.656\,$\to$\,0.792 & $+0.136$ $[+0.071, +0.206]$ & 0.502\,$\to$\,0.511 & \textcolor{cMuted!70}{$+0.009$ $[-0.015, +0.043]$} & 0.400\,$\to$\,0.398 & \textcolor{cMuted!70}{$-0.002$ $[-0.033, +0.030]$} \\
committed $p@1$ & 0.531\,$\to$\,0.650 & $+0.119$ $[+0.084, +0.157]$ & 0.353\,$\to$\,0.387 & $+0.033$ $[+0.013, +0.056]$ & 0.232\,$\to$\,0.281 & $+0.049$ $[+0.028, +0.070]$ \\
strict $p@1$ & 0.529\,$\to$\,0.645 & $+0.116$ $[+0.081, +0.153]$ & 0.339\,$\to$\,0.372 & $+0.033$ $[+0.013, +0.054]$ & 0.201\,$\to$\,0.251 & $+0.050$ $[+0.032, +0.068]$ \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Teacher-solution start (A) $\to$ thinking route (B)}} \\*
answer rate & 0.366\,$\to$\,0.735 & $+0.368$ $[+0.334, +0.403]$ & 0.151\,$\to$\,0.465 & $+0.314$ $[+0.281, +0.349]$ & 0.089\,$\to$\,0.333 & $+0.244$ $[+0.214, +0.276]$ \\
matched accuracy (marked) & 0.713\,$\to$\,0.816 & $+0.104$ $[+0.063, +0.147]$ & 0.566\,$\to$\,0.627 & $+0.061$ $[+0.018, +0.110]$ & 0.369\,$\to$\,0.455 & $+0.087$ $[+0.051, +0.124]$ \\
lenient $p@1$ & 0.330\,$\to$\,0.649 & $+0.319$ $[+0.284, +0.357]$ & 0.128\,$\to$\,0.394 & $+0.266$ $[+0.232, +0.301]$ & 0.055\,$\to$\,0.262 & $+0.207$ $[+0.180, +0.237]$ \\
lenient $p@n$ & 0.748\,$\to$\,0.883 & $+0.134$ $[+0.075, +0.198]$ & 0.517\,$\to$\,0.619 & $+0.103$ $[+0.047, +0.165]$ & 0.399\,$\to$\,0.474 & $+0.074$ $[+0.025, +0.127]$ \\
maj@$n$ & 0.678\,$\to$\,0.801 & $+0.122$ $[+0.064, +0.185]$ & 0.483\,$\to$\,0.548 & $+0.065$ $[+0.015, +0.119]$ & 0.320\,$\to$\,0.400 & $+0.080$ $[+0.042, +0.123]$ \\
committed $p@1$ & 0.328\,$\to$\,0.643 & $+0.315$ $[+0.279, +0.353]$ & 0.124\,$\to$\,0.254 & $+0.130$ $[+0.109, +0.150]$ & 0.050\,$\to$\,0.225 & $+0.174$ $[+0.152, +0.198]$ \\
strict $p@1$ & 0.227\,$\to$\,0.636 & $+0.409$ $[+0.371, +0.448]$ & 0.066\,$\to$\,0.000 & $-0.066$ $[-0.079, -0.055]$ & 0.031\,$\to$\,0.000 & $-0.031$ $[-0.036, -0.026]$ \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Non-thinking route (A) vs thinking route from short external solutions (B)}} \\*
answer rate & 0.946\,$\to$\,0.728 & $-0.217$ $[-0.267, -0.169]$ & 0.886\,$\to$\,0.482 & $-0.404$ $[-0.447, -0.361]$ & 0.827\,$\to$\,0.421 & $-0.406$ $[-0.449, -0.362]$ \\
lenient $p@1$ & 0.549\,$\to$\,0.651 & $+0.102$ $[+0.060, +0.147]$ & 0.440\,$\to$\,0.392 & $-0.047$ $[-0.076, -0.018]$ & 0.328\,$\to$\,0.294 & $-0.034$ $[-0.059, -0.010]$ \\
lenient $p@n$ & 0.791\,$\to$\,0.855 & \textcolor{cMuted!70}{$+0.064$ $[+0.000, +0.132]$} & 0.725\,$\to$\,0.628 & $-0.097$ $[-0.166, -0.032]$ & 0.593\,$\to$\,0.521 & $-0.072$ $[-0.133, -0.014]$ \\
maj@$n$ & 0.599\,$\to$\,0.792 & $+0.193$ $[+0.120, +0.268]$ & 0.519\,$\to$\,0.511 & \textcolor{cMuted!70}{$-0.008$ $[-0.048, +0.030]$} & 0.449\,$\to$\,0.398 & $-0.051$ $[-0.104, -0.003]$ \\
committed $p@1$ & 0.547\,$\to$\,0.650 & $+0.103$ $[+0.061, +0.147]$ & 0.438\,$\to$\,0.387 & $-0.051$ $[-0.080, -0.022]$ & 0.327\,$\to$\,0.281 & $-0.046$ $[-0.071, -0.023]$ \\
strict $p@1$ & 0.505\,$\to$\,0.645 & $+0.140$ $[+0.100, +0.182]$ & 0.437\,$\to$\,0.372 & $-0.065$ $[-0.093, -0.037]$ & 0.327\,$\to$\,0.251 & $-0.076$ $[-0.100, -0.053]$ \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Non-thinking route (A) vs thinking route from the teacher's own solutions (B)}} \\*
answer rate & 0.946\,$\to$\,0.735 & $-0.211$ $[-0.258, -0.166]$ & 0.886\,$\to$\,0.465 & $-0.420$ $[-0.464, -0.378]$ & 0.827\,$\to$\,0.333 & $-0.493$ $[-0.533, -0.453]$ \\
lenient $p@1$ & 0.549\,$\to$\,0.649 & $+0.100$ $[+0.061, +0.142]$ & 0.440\,$\to$\,0.394 & $-0.045$ $[-0.074, -0.018]$ & 0.328\,$\to$\,0.262 & $-0.066$ $[-0.092, -0.041]$ \\
lenient $p@n$ & 0.791\,$\to$\,0.883 & $+0.092$ $[+0.039, +0.150]$ & 0.725\,$\to$\,0.619 & $-0.106$ $[-0.169, -0.046]$ & 0.593\,$\to$\,0.474 & $-0.119$ $[-0.189, -0.051]$ \\
maj@$n$ & 0.599\,$\to$\,0.801 & $+0.202$ $[+0.127, +0.279]$ & 0.519\,$\to$\,0.548 & \textcolor{cMuted!70}{$+0.029$ $[-0.028, +0.090]$} & 0.449\,$\to$\,0.400 & $-0.049$ $[-0.099, -0.003]$ \\
committed $p@1$ & 0.547\,$\to$\,0.643 & $+0.095$ $[+0.056, +0.137]$ & 0.438\,$\to$\,0.254 & $-0.184$ $[-0.220, -0.149]$ & 0.327\,$\to$\,0.225 & $-0.102$ $[-0.128, -0.079]$ \\
strict $p@1$ & 0.505\,$\to$\,0.636 & $+0.131$ $[+0.094, +0.169]$ & 0.437\,$\to$\,0.000 & $-0.437$ $[-0.485, -0.391]$ & 0.327\,$\to$\,0.000 & $-0.327$ $[-0.364, -0.290]$ \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Pretrained-only student one size larger (A) vs non-thinking route (B), in the column of B's size: 4B (A) vs 1.7B (B), and 1.7B (A) vs 0.6B (B)}} \\*
answer rate & -- & -- & 0.830\,$\to$\,0.886 & $+0.056$ $[+0.025, +0.086]$ & 0.752\,$\to$\,0.827 & $+0.075$ $[+0.043, +0.106]$ \\
lenient $p@1$ & -- & -- & 0.427\,$\to$\,0.440 & \textcolor{cMuted!70}{$+0.012$ $[-0.014, +0.039]$} & 0.294\,$\to$\,0.328 & $+0.035$ $[+0.015, +0.054]$ \\
lenient $p@n$ & -- & -- & 0.736\,$\to$\,0.725 & \textcolor{cMuted!70}{$-0.011$ $[-0.065, +0.042]$} & 0.646\,$\to$\,0.593 & $-0.053$ $[-0.107, -0.003]$ \\
maj@$n$ & -- & -- & 0.553\,$\to$\,0.519 & \textcolor{cMuted!70}{$-0.033$ $[-0.094, +0.028]$} & 0.481\,$\to$\,0.449 & \textcolor{cMuted!70}{$-0.032$ $[-0.081, +0.018]$} \\
committed $p@1$ & -- & -- & 0.426\,$\to$\,0.438 & \textcolor{cMuted!70}{$+0.012$ $[-0.014, +0.038]$} & 0.293\,$\to$\,0.327 & $+0.034$ $[+0.014, +0.054]$ \\
strict $p@1$ & -- & -- & 0.426\,$\to$\,0.437 & \textcolor{cMuted!70}{$+0.011$ $[-0.015, +0.037]$} & 0.294\,$\to$\,0.327 & $+0.033$ $[+0.013, +0.053]$ \\
GPQA-Diamond, committed $p@1$ & -- & -- & 0.157\,$\to$\,0.275 & $+0.117$ $[+0.081, +0.154]$ & 0.191\,$\to$\,0.234 & $+0.044$ $[+0.011, +0.076]$ \\
GPQA-Diamond, strict $p@1$ & -- & -- & 0.157\,$\to$\,0.270 & $+0.114$ $[+0.077, +0.150]$ & 0.189\,$\to$\,0.233 & $+0.044$ $[+0.012, +0.077]$ \\
GPQA-Diamond, committed $p@n$ & -- & -- & 0.606\,$\to$\,0.717 & $+0.111$ $[+0.025, +0.197]$ & 0.651\,$\to$\,0.732 & $+0.081$ $[+0.005, +0.157]$ \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Thinking route: from short external solutions (A) vs from the teacher's own solutions (B), at equal size}} \\*
answer rate & 0.728\,$\to$\,0.735 & \textcolor{cMuted!70}{$+0.006$ $[-0.009, +0.021]$} & 0.482\,$\to$\,0.465 & $-0.017$ $[-0.033, -0.001]$ & 0.421\,$\to$\,0.333 & $-0.088$ $[-0.112, -0.065]$ \\
lenient $p@1$ & 0.651\,$\to$\,0.649 & \textcolor{cMuted!70}{$-0.002$ $[-0.014, +0.010]$} & 0.392\,$\to$\,0.394 & \textcolor{cMuted!70}{$+0.002$ $[-0.010, +0.014]$} & 0.294\,$\to$\,0.262 & $-0.032$ $[-0.044, -0.021]$ \\
lenient $p@n$ & 0.855\,$\to$\,0.883 & \textcolor{cMuted!70}{$+0.028$ $[+0.000, +0.064]$} & 0.628\,$\to$\,0.619 & \textcolor{cMuted!70}{$-0.009$ $[-0.047, +0.031]$} & 0.521\,$\to$\,0.474 & \textcolor{cMuted!70}{$-0.047$ $[-0.101, +0.006]$} \\
maj@$n$ & 0.792\,$\to$\,0.801 & \textcolor{cMuted!70}{$+0.008$ $[-0.025, +0.044]$} & 0.511\,$\to$\,0.548 & \textcolor{cMuted!70}{$+0.037$ $[-0.003, +0.083]$} & 0.398\,$\to$\,0.400 & \textcolor{cMuted!70}{$+0.002$ $[-0.015, +0.023]$} \\
committed $p@1$ & 0.650\,$\to$\,0.643 & \textcolor{cMuted!70}{$-0.007$ $[-0.020, +0.004]$} & 0.387\,$\to$\,0.254 & $-0.133$ $[-0.167, -0.102]$ & 0.281\,$\to$\,0.225 & $-0.056$ $[-0.070, -0.043]$ \\
strict $p@1$ & 0.645\,$\to$\,0.636 & \textcolor{cMuted!70}{$-0.009$ $[-0.021, +0.002]$} & 0.372\,$\to$\,0.000 & $-0.372$ $[-0.420, -0.325]$ & 0.251\,$\to$\,0.000 & $-0.251$ $[-0.284, -0.220]$ \\
\end{longtable}
\endgroup
\end{landscape}



==> tables/app_ci_bench.tex <==
\begin{landscape}
\begingroup
\footnotesize
\setlength{\tabcolsep}{4.5pt}
\setlength{\LTcapwidth}{\linewidth}
\begin{longtable}{@{}llcccccc@{}}
\caption{\textbf{The same intervals, benchmark by benchmark.} Head-to-head comparisons of the two routes at equal
size (first two blocks); the change from each route's start to its endpoint (next three blocks); each
pretrained-only student against the non-thinking route one size smaller, and the two thinking starts against
each other after distillation (last two blocks). Every block is on each open-ended benchmark separately.
Same bootstrap as Table~\ref{tab:app-ci}, resampling the benchmark's problems only. Intervals that contain 0
are set in grey: those pairs are indistinguishable. On AIME 2026, with 30 problems and the smaller students
near zero accuracy, several intervals are wide or degenerate: one problem moves maj@$n$ by one thirtieth.}\label{tab:app-ci-bench}\\
\toprule
& & \multicolumn{2}{c}{AIME 2026} & \multicolumn{2}{c}{AMC23} & \multicolumn{2}{c}{GSM8K-200} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Size & Metric & A $\to$ B & B $-$ A [95\% CI] & A $\to$ B & B $-$ A [95\% CI] & A $\to$ B & B $-$ A [95\% CI] \\
\midrule
\endfirsthead
\multicolumn{8}{l}{\textit{Table~\ref{tab:app-ci-bench}, continued}}\\
\toprule
& & \multicolumn{2}{c}{AIME 2026} & \multicolumn{2}{c}{AMC23} & \multicolumn{2}{c}{GSM8K-200} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Size & Metric & A $\to$ B & B $-$ A [95\% CI] & A $\to$ B & B $-$ A [95\% CI] & A $\to$ B & B $-$ A [95\% CI] \\
\midrule
\endhead
\midrule
\multicolumn{8}{r}{\textit{continued on the next page}}\\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{8}{@{}l}{\textbf{Head to head: non-thinking route (A) vs thinking route from short external solutions (B)}} \\*
4B & answer rate & 0.875\,$\to$\,0.465 & $-0.410$ $[-0.526, -0.296]$ & 0.963\,$\to$\,0.770 & $-0.193$ $[-0.288, -0.107]$ & 1.000\,$\to$\,0.951 & $-0.049$ $[-0.066, -0.035]$ \\*
 & lenient $p@1$ & 0.141\,$\to$\,0.329 & $+0.188$ $[+0.100, +0.284]$ & 0.587\,$\to$\,0.728 & $+0.141$ $[+0.055, +0.231]$ & 0.919\,$\to$\,0.896 & \textcolor{cMuted!70}{$-0.022$ $[-0.048, +0.002]$} \\*
 & maj@$n$ & 0.167\,$\to$\,0.567 & $+0.400$ $[+0.233, +0.567]$ & 0.700\,$\to$\,0.875 & $+0.175$ $[+0.050, +0.325]$ & 0.930\,$\to$\,0.935 & \textcolor{cMuted!70}{$+0.005$ $[-0.025, +0.035]$} \\
\addlinespace[2pt]
1.7B & answer rate & 0.749\,$\to$\,0.158 & $-0.590$ $[-0.663, -0.512]$ & 0.910\,$\to$\,0.460 & $-0.451$ $[-0.552, -0.348]$ & 0.999\,$\to$\,0.828 & $-0.171$ $[-0.202, -0.142]$ \\*
 & lenient $p@1$ & 0.079\,$\to$\,0.057 & \textcolor{cMuted!70}{$-0.022$ $[-0.080, +0.037]$} & 0.410\,$\to$\,0.362 & \textcolor{cMuted!70}{$-0.047$ $[-0.106, +0.006]$} & 0.830\,$\to$\,0.757 & $-0.072$ $[-0.101, -0.044]$ \\*
 & maj@$n$ & 0.133\,$\to$\,0.133 & \textcolor{cMuted!70}{$+0.000$ $[+0.000, +0.000]$} & 0.550\,$\to$\,0.525 & \textcolor{cMuted!70}{$-0.025$ $[-0.125, +0.075]$} & 0.875\,$\to$\,0.875 & \textcolor{cMuted!70}{$+0.000$ $[-0.035, +0.035]$} \\
\addlinespace[2pt]
0.6B & answer rate & 0.639\,$\to$\,0.149 & $-0.490$ $[-0.568, -0.408]$ & 0.850\,$\to$\,0.356 & $-0.493$ $[-0.585, -0.400]$ & 0.992\,$\to$\,0.758 & $-0.234$ $[-0.274, -0.195]$ \\*
 & lenient $p@1$ & 0.018\,$\to$\,0.004 & $-0.015$ $[-0.034, -0.001]$ & 0.278\,$\to$\,0.212 & $-0.066$ $[-0.131, -0.004]$ & 0.689\,$\to$\,0.667 & \textcolor{cMuted!70}{$-0.022$ $[-0.051, +0.007]$} \\*
 & maj@$n$ & 0.067\,$\to$\,0.000 & \textcolor{cMuted!70}{$-0.067$ $[-0.167, +0.000]$} & 0.475\,$\to$\,0.375 & \textcolor{cMuted!70}{$-0.100$ $[-0.225, +0.000]$} & 0.805\,$\to$\,0.820 & \textcolor{cMuted!70}{$+0.015$ $[-0.025, +0.055]$} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Head to head: non-thinking route (A) vs thinking route from the teacher's own solutions (B)}} \\*
4B & answer rate & 0.875\,$\to$\,0.469 & $-0.406$ $[-0.513, -0.300]$ & 0.963\,$\to$\,0.772 & $-0.191$ $[-0.283, -0.106]$ & 1.000\,$\to$\,0.962 & $-0.038$ $[-0.054, -0.024]$ \\*
 & lenient $p@1$ & 0.141\,$\to$\,0.316 & $+0.175$ $[+0.099, +0.260]$ & 0.587\,$\to$\,0.728 & $+0.142$ $[+0.057, +0.230]$ & 0.919\,$\to$\,0.903 & \textcolor{cMuted!70}{$-0.016$ $[-0.042, +0.009]$} \\*
 & maj@$n$ & 0.167\,$\to$\,0.567 & $+0.400$ $[+0.233, +0.567]$ & 0.700\,$\to$\,0.900 & $+0.200$ $[+0.075, +0.350]$ & 0.930\,$\to$\,0.935 & \textcolor{cMuted!70}{$+0.005$ $[-0.025, +0.035]$} \\
\addlinespace[2pt]
1.7B & answer rate & 0.749\,$\to$\,0.139 & $-0.610$ $[-0.683, -0.532]$ & 0.910\,$\to$\,0.446 & $-0.464$ $[-0.565, -0.361]$ & 0.999\,$\to$\,0.811 & $-0.188$ $[-0.220, -0.158]$ \\*
 & lenient $p@1$ & 0.079\,$\to$\,0.067 & \textcolor{cMuted!70}{$-0.012$ $[-0.061, +0.033]$} & 0.410\,$\to$\,0.372 & \textcolor{cMuted!70}{$-0.038$ $[-0.104, +0.022]$} & 0.830\,$\to$\,0.743 & $-0.087$ $[-0.117, -0.057]$ \\*
 & maj@$n$ & 0.133\,$\to$\,0.200 & \textcolor{cMuted!70}{$+0.067$ $[+0.000, +0.167]$} & 0.550\,$\to$\,0.575 & \textcolor{cMuted!70}{$+0.025$ $[-0.125, +0.175]$} & 0.875\,$\to$\,0.870 & \textcolor{cMuted!70}{$-0.005$ $[-0.035, +0.030]$} \\
\addlinespace[2pt]
0.6B & answer rate & 0.639\,$\to$\,0.067 & $-0.572$ $[-0.640, -0.497]$ & 0.850\,$\to$\,0.252 & $-0.597$ $[-0.678, -0.515]$ & 0.992\,$\to$\,0.681 & $-0.312$ $[-0.357, -0.267]$ \\*
 & lenient $p@1$ & 0.018\,$\to$\,0.003 & \textcolor{cMuted!70}{$-0.015$ $[-0.037, +0.000]$} & 0.278\,$\to$\,0.165 & $-0.113$ $[-0.184, -0.048]$ & 0.689\,$\to$\,0.620 & $-0.069$ $[-0.099, -0.039]$ \\*
 & maj@$n$ & 0.067\,$\to$\,0.000 & \textcolor{cMuted!70}{$-0.067$ $[-0.167, +0.000]$} & 0.475\,$\to$\,0.400 & \textcolor{cMuted!70}{$-0.075$ $[-0.175, +0.025]$} & 0.805\,$\to$\,0.800 & \textcolor{cMuted!70}{$-0.005$ $[-0.050, +0.035]$} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Pretrained-only start (A) $\to$ non-thinking route (B)}} \\*
4B & answer rate & 0.792\,$\to$\,0.875 & $+0.083$ $[+0.017, +0.149]$ & 0.829\,$\to$\,0.963 & $+0.134$ $[+0.090, +0.181]$ & 0.871\,$\to$\,1.000 & $+0.129$ $[+0.114, +0.144]$ \\*
 & acc.\ given an answer, matched & 0.095\,$\to$\,0.147 & $+0.052$ $[+0.009, +0.109]$ & 0.505\,$\to$\,0.596 & $+0.091$ $[+0.048, +0.136]$ & 0.873\,$\to$\,0.919 & $+0.046$ $[+0.027, +0.066]$ \\*
 & lenient $p@1$ & 0.083\,$\to$\,0.141 & $+0.058$ $[+0.015, +0.116]$ & 0.438\,$\to$\,0.587 & $+0.148$ $[+0.098, +0.201]$ & 0.761\,$\to$\,0.919 & $+0.158$ $[+0.134, +0.182]$ \\
\addlinespace[2pt]
1.7B & answer rate & 0.700\,$\to$\,0.749 & \textcolor{cMuted!70}{$+0.049$ $[-0.024, +0.119]$} & 0.763\,$\to$\,0.910 & $+0.147$ $[+0.108, +0.188]$ & 0.792\,$\to$\,0.999 & $+0.207$ $[+0.187, +0.227]$ \\*
 & acc.\ given an answer, matched & 0.018\,$\to$\,0.085 & $+0.067$ $[+0.005, +0.141]$ & 0.330\,$\to$\,0.434 & $+0.104$ $[+0.060, +0.150]$ & 0.763\,$\to$\,0.834 & $+0.070$ $[+0.046, +0.096]$ \\*
 & lenient $p@1$ & 0.014\,$\to$\,0.079 & $+0.065$ $[+0.005, +0.138]$ & 0.266\,$\to$\,0.410 & $+0.144$ $[+0.095, +0.198]$ & 0.601\,$\to$\,0.830 & $+0.229$ $[+0.201, +0.256]$ \\
\addlinespace[2pt]
0.6B & answer rate & 0.208\,$\to$\,0.639 & $+0.431$ $[+0.346, +0.512]$ & 0.205\,$\to$\,0.850 & $+0.645$ $[+0.586, +0.701]$ & 0.169\,$\to$\,0.992 & $+0.824$ $[+0.804, +0.842]$ \\*
 & acc.\ given an answer, matched & 0.030\,$\to$\,0.023 & \textcolor{cMuted!70}{$-0.008$ $[-0.040, +0.021]$} & 0.231\,$\to$\,0.302 & $+0.071$ $[+0.005, +0.134]$ & 0.483\,$\to$\,0.695 & $+0.212$ $[+0.177, +0.247]$ \\*
 & lenient $p@1$ & 0.004\,$\to$\,0.018 & \textcolor{cMuted!70}{$+0.014$ $[-0.002, +0.037]$} & 0.053\,$\to$\,0.278 & $+0.225$ $[+0.150, +0.302]$ & 0.087\,$\to$\,0.689 & $+0.601$ $[+0.556, +0.646]$ \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Short-solution start (A) $\to$ thinking route (B)}} \\*
4B & answer rate & 0.463\,$\to$\,0.465 & \textcolor{cMuted!70}{$+0.001$ $[-0.085, +0.090]$} & 0.758\,$\to$\,0.770 & \textcolor{cMuted!70}{$+0.011$ $[-0.059, +0.083]$} & 0.980\,$\to$\,0.951 & $-0.029$ $[-0.044, -0.016]$ \\*
 & acc.\ given an answer, matched & 0.184\,$\to$\,0.522 & $+0.338$ $[+0.217, +0.469]$ & 0.654\,$\to$\,0.864 & $+0.210$ $[+0.132, +0.291]$ & 0.913\,$\to$\,0.935 & $+0.022$ $[+0.005, +0.039]$ \\*
 & lenient $p@1$ & 0.148\,$\to$\,0.329 & $+0.181$ $[+0.105, +0.267]$ & 0.548\,$\to$\,0.728 & $+0.179$ $[+0.110, +0.256]$ & 0.899\,$\to$\,0.896 & \textcolor{cMuted!70}{$-0.003$ $[-0.023, +0.017]$} \\
\addlinespace[2pt]
1.7B & answer rate & 0.360\,$\to$\,0.158 & $-0.202$ $[-0.269, -0.135]$ & 0.609\,$\to$\,0.460 & $-0.149$ $[-0.228, -0.069]$ & 0.911\,$\to$\,0.828 & $-0.083$ $[-0.108, -0.060]$ \\*
 & acc.\ given an answer, matched & 0.084\,$\to$\,0.186 & $+0.102$ $[+0.027, +0.194]$ & 0.433\,$\to$\,0.571 & $+0.137$ $[+0.076, +0.206]$ & 0.799\,$\to$\,0.879 & $+0.080$ $[+0.057, +0.103]$ \\*
 & lenient $p@1$ & 0.029\,$\to$\,0.057 & \textcolor{cMuted!70}{$+0.028$ $[+0.000, +0.065]$} & 0.299\,$\to$\,0.362 & $+0.063$ $[+0.017, +0.116]$ & 0.747\,$\to$\,0.757 & \textcolor{cMuted!70}{$+0.011$ $[-0.014, +0.035]$} \\
\addlinespace[2pt]
0.6B & answer rate & 0.515\,$\to$\,0.149 & $-0.366$ $[-0.430, -0.301]$ & 0.669\,$\to$\,0.356 & $-0.312$ $[-0.406, -0.218]$ & 0.831\,$\to$\,0.758 & $-0.073$ $[-0.105, -0.041]$ \\*
 & acc.\ given an answer, matched & 0.010\,$\to$\,0.016 & \textcolor{cMuted!70}{$+0.007$ $[-0.004, +0.022]$} & 0.231\,$\to$\,0.389 & $+0.158$ $[+0.089, +0.232]$ & 0.619\,$\to$\,0.800 & $+0.181$ $[+0.150, +0.211]$ \\*
 & lenient $p@1$ & 0.006\,$\to$\,0.004 & \textcolor{cMuted!70}{$-0.002$ $[-0.004, +0.000]$} & 0.173\,$\to$\,0.212 & \textcolor{cMuted!70}{$+0.039$ $[-0.019, +0.098]$} & 0.536\,$\to$\,0.667 & $+0.131$ $[+0.104, +0.158]$ \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Teacher-solution start (A) $\to$ thinking route (B)}} \\*
4B & answer rate & 0.181\,$\to$\,0.469 & $+0.289$ $[+0.219, +0.365]$ & 0.435\,$\to$\,0.772 & $+0.337$ $[+0.272, +0.405]$ & 0.484\,$\to$\,0.962 & $+0.478$ $[+0.447, +0.510]$ \\*
 & acc.\ given an answer, matched & 0.368\,$\to$\,0.606 & $+0.238$ $[+0.138, +0.354]$ & 0.849\,$\to$\,0.915 & $+0.067$ $[+0.008, +0.131]$ & 0.920\,$\to$\,0.926 & \textcolor{cMuted!70}{$+0.006$ $[-0.009, +0.022]$} \\*
 & lenient $p@1$ & 0.116\,$\to$\,0.316 & $+0.200$ $[+0.126, +0.281]$ & 0.412\,$\to$\,0.728 & $+0.316$ $[+0.249, +0.388]$ & 0.461\,$\to$\,0.903 & $+0.442$ $[+0.407, +0.476]$ \\
\addlinespace[2pt]
1.7B & answer rate & 0.039\,$\to$\,0.139 & $+0.100$ $[+0.047, +0.164]$ & 0.148\,$\to$\,0.446 & $+0.298$ $[+0.222, +0.376]$ & 0.267\,$\to$\,0.811 & $+0.544$ $[+0.516, +0.571]$ \\*
 & acc.\ given an answer, matched & 0.181\,$\to$\,0.282 & $+0.101$ $[+0.007, +0.225]$ & 0.686\,$\to$\,0.722 & \textcolor{cMuted!70}{$+0.036$ $[-0.043, +0.115]$} & 0.830\,$\to$\,0.877 & $+0.047$ $[+0.024, +0.071]$ \\*
 & lenient $p@1$ & 0.013\,$\to$\,0.067 & $+0.054$ $[+0.009, +0.113]$ & 0.129\,$\to$\,0.372 & $+0.243$ $[+0.162, +0.327]$ & 0.243\,$\to$\,0.743 & $+0.500$ $[+0.467, +0.532]$ \\
\addlinespace[2pt]
0.6B & answer rate & 0.032\,$\to$\,0.067 & $+0.035$ $[+0.002, +0.077]$ & 0.070\,$\to$\,0.252 & $+0.182$ $[+0.112, +0.259]$ & 0.165\,$\to$\,0.681 & $+0.516$ $[+0.476, +0.556]$ \\*
 & acc.\ given an answer, matched & 0.051\,$\to$\,0.036 & \textcolor{cMuted!70}{$-0.015$ $[-0.071, +0.019]$} & 0.326\,$\to$\,0.484 & $+0.158$ $[+0.070, +0.255]$ & 0.729\,$\to$\,0.846 & $+0.118$ $[+0.081, +0.156]$ \\*
 & lenient $p@1$ & 0.001\,$\to$\,0.003 & \textcolor{cMuted!70}{$+0.001$ $[+0.000, +0.004]$} & 0.029\,$\to$\,0.165 & $+0.136$ $[+0.068, +0.213]$ & 0.135\,$\to$\,0.620 & $+0.484$ $[+0.440, +0.528]$ \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Pretrained-only student one size larger (A) vs non-thinking route (B); the size is B's}} \\*
1.7B & answer rate & 0.792\,$\to$\,0.749 & \textcolor{cMuted!70}{$-0.043$ $[-0.113, +0.031]$} & 0.829\,$\to$\,0.910 & $+0.082$ $[+0.028, +0.135]$ & 0.871\,$\to$\,0.999 & $+0.128$ $[+0.114, +0.144]$ \\*
 & lenient $p@1$ & 0.083\,$\to$\,0.079 & \textcolor{cMuted!70}{$-0.004$ $[-0.032, +0.030]$} & 0.438\,$\to$\,0.410 & \textcolor{cMuted!70}{$-0.028$ $[-0.092, +0.036]$} & 0.761\,$\to$\,0.830 & $+0.069$ $[+0.038, +0.099]$ \\*
 & committed $p@1$ & 0.083\,$\to$\,0.078 & \textcolor{cMuted!70}{$-0.005$ $[-0.033, +0.029]$} & 0.436\,$\to$\,0.406 & \textcolor{cMuted!70}{$-0.030$ $[-0.094, +0.034]$} & 0.759\,$\to$\,0.830 & $+0.070$ $[+0.039, +0.100]$ \\
\addlinespace[2pt]
0.6B & answer rate & 0.700\,$\to$\,0.639 & \textcolor{cMuted!70}{$-0.061$ $[-0.137, +0.010]$} & 0.763\,$\to$\,0.850 & $+0.086$ $[+0.029, +0.140]$ & 0.792\,$\to$\,0.992 & $+0.200$ $[+0.180, +0.221]$ \\*
 & lenient $p@1$ & 0.014\,$\to$\,0.018 & \textcolor{cMuted!70}{$+0.004$ $[-0.018, +0.026]$} & 0.266\,$\to$\,0.278 & \textcolor{cMuted!70}{$+0.011$ $[-0.033, +0.058]$} & 0.601\,$\to$\,0.689 & $+0.088$ $[+0.056, +0.120]$ \\*
 & committed $p@1$ & 0.014\,$\to$\,0.017 & \textcolor{cMuted!70}{$+0.004$ $[-0.019, +0.024]$} & 0.266\,$\to$\,0.276 & \textcolor{cMuted!70}{$+0.010$ $[-0.035, +0.057]$} & 0.598\,$\to$\,0.688 & $+0.089$ $[+0.057, +0.122]$ \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Thinking route: from short external solutions (A) vs from the teacher's own solutions (B)}} \\*
4B & answer rate & 0.465\,$\to$\,0.469 & \textcolor{cMuted!70}{$+0.005$ $[-0.034, +0.046]$} & 0.770\,$\to$\,0.772 & \textcolor{cMuted!70}{$+0.002$ $[-0.017, +0.021]$} & 0.951\,$\to$\,0.962 & $+0.012$ $[+0.002, +0.021]$ \\*
 & lenient $p@1$ & 0.329\,$\to$\,0.316 & \textcolor{cMuted!70}{$-0.013$ $[-0.042, +0.013]$} & 0.728\,$\to$\,0.728 & \textcolor{cMuted!70}{$+0.001$ $[-0.021, +0.022]$} & 0.896\,$\to$\,0.903 & \textcolor{cMuted!70}{$+0.007$ $[-0.003, +0.016]$} \\*
 & committed $p@1$ & 0.327\,$\to$\,0.312 & \textcolor{cMuted!70}{$-0.015$ $[-0.044, +0.012]$} & 0.727\,$\to$\,0.726 & \textcolor{cMuted!70}{$-0.001$ $[-0.023, +0.020]$} & 0.896\,$\to$\,0.889 & \textcolor{cMuted!70}{$-0.007$ $[-0.018, +0.004]$} \\
\addlinespace[2pt]
1.7B & answer rate & 0.158\,$\to$\,0.139 & \textcolor{cMuted!70}{$-0.019$ $[-0.057, +0.017]$} & 0.460\,$\to$\,0.446 & \textcolor{cMuted!70}{$-0.013$ $[-0.043, +0.015]$} & 0.828\,$\to$\,0.811 & $-0.017$ $[-0.031, -0.002]$ \\*
 & lenient $p@1$ & 0.057\,$\to$\,0.067 & \textcolor{cMuted!70}{$+0.010$ $[-0.011, +0.035]$} & 0.362\,$\to$\,0.372 & \textcolor{cMuted!70}{$+0.009$ $[-0.015, +0.034]$} & 0.757\,$\to$\,0.743 & $-0.014$ $[-0.028, -0.001]$ \\*
 & committed $p@1$ & 0.053\,$\to$\,0.031 & \textcolor{cMuted!70}{$-0.022$ $[-0.068, +0.009]$} & 0.350\,$\to$\,0.180 & $-0.171$ $[-0.264, -0.088]$ & 0.756\,$\to$\,0.551 & $-0.205$ $[-0.226, -0.183]$ \\
\addlinespace[2pt]
0.6B & answer rate & 0.149\,$\to$\,0.067 & $-0.081$ $[-0.133, -0.037]$ & 0.356\,$\to$\,0.252 & $-0.104$ $[-0.152, -0.060]$ & 0.758\,$\to$\,0.681 & $-0.078$ $[-0.097, -0.060]$ \\*
 & lenient $p@1$ & 0.004\,$\to$\,0.003 & \textcolor{cMuted!70}{$-0.001$ $[-0.003, +0.001]$} & 0.212\,$\to$\,0.165 & $-0.047$ $[-0.082, -0.019]$ & 0.667\,$\to$\,0.620 & $-0.047$ $[-0.063, -0.032]$ \\*
 & committed $p@1$ & 0.002\,$\to$\,0.002 & \textcolor{cMuted!70}{$+0.000$ $[-0.002, +0.002]$} & 0.189\,$\to$\,0.126 & $-0.064$ $[-0.100, -0.030]$ & 0.651\,$\to$\,0.546 & $-0.105$ $[-0.122, -0.088]$ \\
\end{longtable}
\endgroup
\end{landscape}



==> tables/app_components.tex <==
\begin{table}[!htbp]
\centering
\footnotesize
\caption{\textbf{Each route moves two things: how often the student answers, and how often it is right when it
does.} For every route and benchmark, the change from the route's start to its endpoint in the answer rate
(the horizontal component of an arrow in Figure~\ref{fig:headtohead}) and in the accuracy given a marked answer
(the vertical component). Both are unmatched, as plotted; the matched version of the second is in
Table~\ref{tab:app-matched}. From short external solutions, the answer rate barely moves at 4B (on the
three-benchmark mean the change, $-0.006$, is a tie) and falls at 1.7B and 0.6B on every benchmark. From the
teacher's own solutions it rises everywhere, from a start that seldom answers, and the accuracy given an
answer is within 0.04 of zero in the four cells where it is not positive. For reference, the non-thinking
route's point estimates are positive in every cell, but two of its changes on AIME 2026 are ties: the answer
rate at 1.7B ($+0.049$ $[-0.024, +0.119]$, Table~\ref{tab:app-ci-bench}) and, at 0.6B, the matched accuracy
given an answer, whose point estimate is negative (Table~\ref{tab:app-matched}).}
\label{tab:app-components}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lcccccc@{}}
\toprule
& \multicolumn{2}{c}{AIME 2026} & \multicolumn{2}{c}{AMC23} & \multicolumn{2}{c}{GSM8K-200} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& answer & acc.\ given & answer & acc.\ given & answer & acc.\ given \\
Size & rate & an answer & rate & an answer & rate & an answer \\
\midrule
\multicolumn{7}{@{}l}{\textit{Thinking route from short external solutions (the arrows of Figure~\ref{fig:headtohead})}} \\
4B & $+0.001$ & $+0.389$ & $+0.012$ & $+0.222$ & $-0.029$ & $+0.026$ \\
1.7B & $-0.202$ & $+0.279$ & $-0.150$ & $+0.297$ & $-0.083$ & $+0.095$ \\
0.6B & $-0.366$ & $+0.013$ & $-0.312$ & $+0.336$ & $-0.073$ & $+0.235$ \\
\midrule
\multicolumn{7}{@{}l}{\textit{Thinking route from the teacher's own solutions}} \\
4B & $+0.289$ & $+0.031$ & $+0.337$ & $-0.004$ & $+0.478$ & $-0.015$ \\
1.7B & $+0.100$ & $+0.146$ & $+0.298$ & $-0.037$ & $+0.544$ & $+0.008$ \\
0.6B & $+0.036$ & $-0.002$ & $+0.182$ & $+0.243$ & $+0.516$ & $+0.090$ \\
\midrule
\multicolumn{7}{@{}l}{\textit{For reference: pretrained-only start $\to$ non-thinking route}} \\
4B & $+0.083$ & $+0.057$ & $+0.134$ & $+0.081$ & $+0.129$ & $+0.045$ \\
1.7B & $+0.049$ & $+0.086$ & $+0.147$ & $+0.101$ & $+0.207$ & $+0.072$ \\
0.6B & $+0.431$ & $+0.008$ & $+0.645$ & $+0.067$ & $+0.824$ & $+0.176$ \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_controls.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{What each control varies, what it holds fixed, and in which arm it was run.} A control speaks to the
closure collapse only if it has runs in the thinking arm; both curriculum runs are in the non-thinking arm.
\emph{Collapse onset}: the first step at which the run's closure falls below 0.75 times its own steps 1--4
level (Table~\ref{tab:app-windows}); runs that start from a low closure (the teacher's own solutions, the
1{,}024-token budget) cross that line from a low level. Non-thinking runs have no closure to lose. Per-run
curves are in Tables~\ref{tab:app-windows}, \ref{tab:app-steps} and~\ref{tab:app-val}.}
\label{tab:app-controls}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{1.45cm}>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}p{1.05cm}>{\raggedright\arraybackslash}p{1.9cm}>{\raggedright\arraybackslash}p{2.35cm}@{}}
\toprule
Control & What varies & Held fixed & Arm & Runs & Collapse onset (step) \\
\midrule
Independent reruns & nothing by design (same configuration and data order; the seed was not passed to the trainer) & everything else & thinking & 2 at 4B, 2 at 0.6B, short-solution start & 4B: 6, 6; 0.6B: 6, 6 \\
\addlinespace[3pt]
Cold-start set & 5,878 short external solutions vs 1,524 of the teacher's own solutions & size, training problems, 7,168-token budget, teacher mode & thinking & 3 sizes $\times$ 2 starts & short: 6, 6, 6; teacher's own: 11, 6, 6 (4B, 1.7B, 0.6B) \\
\addlinespace[3pt]
Rollout budget & 1,024 / 7,168 / 16,384 tokens & 0.6B short-solution start, training problems, teacher mode; the 1,024-token run also uses one update per step & thinking & 0.6B: 1, 2 and 1 runs & 5 / 6, 6 / 7 \\
\addlinespace[3pt]
Starting point & officially post-trained 0.6B instead of the cold-started 0.6B & size, 16,384-token budget, training problems, teacher mode & thinking & 0.6B: 2 runs & 6, 6 (cold-started: 7) \\
\addlinespace[3pt]
Teacher's mode & thinking vs non-thinking chat template & student weights, training problems and order, 16,384-token budget & both & officially post-trained 0.6B: 2 thinking, 1 non-thinking & 6, 6 / none: the only control that removes the collapse \\
\addlinespace[3pt]
Easy-to-hard curriculum & problem order; 856 problems with statements truncated upstream dropped (12,741 left) & student, non-thinking teacher, 7,168-token budget & non-thinking only & 4B, 1.7B: 99 steps each & not applicable: says nothing about the collapse \\
\midrule
\multicolumn{6}{p{0.97\textwidth}}{\textit{Not run:} a curriculum in the thinking arm; a 4B or 1.7B run at a rollout budget other than 7,168 tokens; a forward-KL objective.} \\
\bottomrule
\end{tabularx}
\end{table}



==> tables/app_enum.tex <==
\begin{table}[!htbp]
\centering
\scriptsize
\caption{\textbf{Where the lenient score could be inflated by listing answers, and where it is not.}
The lenient score credits a sample if any marked answer in it is correct, so a sample that lists several
candidates could be credited by enumeration alone. \emph{Answers}: boxed answers per sample;
\emph{distinct}: distinct boxed values per sample. \emph{Enumeration only}: the fraction of samples that
contain a correct boxed answer, end on a wrong one, and hold at least two distinct values, i.e.\ lenient credit
that the committed score would not give and that could come from listing; the last column removes it. Only
the 1.7B and 0.6B students distilled from the thinking teacher after the teacher-solution start draw material
credit this way, and their committed scores are reported beside the lenient ones throughout. The many answers
per sample of the non-thinking students are repetitions of one value (distinct answers stay near 1) and earn
no extra credit. $^\dagger$\,Evaluated with fewer samples: 16 per problem on AIME 2026 and AMC23, 4 on GSM8K-200.}
\label{tab:app-enum}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lcccccc@{}}
\toprule
& Answers & Distinct & Lenient & Committed & Enumeration & Lenient minus \\
Model & per sample & answers & $p@1$ & $p@1$ & only & enumeration \\
\midrule
\multicolumn{7}{@{}l}{\textit{(a) Every model, mean of the three open-ended benchmarks}} \\
Teacher (thinking) & 2.4 & 0.98 & 0.857 & 0.854 & 0.003 & 0.854 \\
Teacher (non-thinking) & 3.5 & 1.11 & 0.595 & 0.594 & 0.001 & 0.594 \\
\addlinespace[2pt]
4B pretrained-only & 1.8 & 0.83 & 0.427 & 0.426 & 0.001 & 0.427 \\
4B non-thinking route & 214.3 & 1.15 & 0.549 & 0.547 & 0.001 & 0.547 \\
4B short-solution start & 2.5 & 0.74 & 0.532 & 0.531 & 0.001 & 0.531 \\
\quad + thinking route & 1.9 & 0.75 & 0.651 & 0.650 & 0.001 & 0.650 \\
4B teacher-solution start & 1.1 & 0.38 & 0.330 & 0.328 & 0.002 & 0.328 \\
\quad + thinking route & 1.9 & 0.76 & 0.649 & 0.643 & 0.006 & 0.643 \\
\quad + thinking route, 212 steps & 2.1 & 0.83 & 0.671 & 0.646 & 0.025 & 0.646 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.8 & 0.75 & 0.294 & 0.293 & 0.000 & 0.294 \\
1.7B non-thinking route & 18.8 & 1.21 & 0.440 & 0.438 & 0.002 & 0.438 \\
1.7B short-solution start & 2.5 & 0.66 & 0.358 & 0.353 & 0.005 & 0.354 \\
\quad + thinking route & 1.7 & 0.53 & 0.392 & 0.387 & 0.005 & 0.387 \\
1.7B teacher-solution start & 2.7 & 0.17 & 0.128 & 0.124 & 0.003 & 0.125 \\
\quad + thinking route & 185.5 & 1.80 & 0.394 & 0.254 & 0.138 & 0.256 \\
\addlinespace[2pt]
0.6B pretrained-only & 12.8 & 2.89 & 0.048 & 0.047 & 0.002 & 0.047 \\
0.6B non-thinking route & 11.2 & 1.06 & 0.328 & 0.327 & 0.001 & 0.327 \\
0.6B short-solution start & 17.4 & 0.76 & 0.238 & 0.232 & 0.006 & 0.232 \\
\quad + thinking route & 2.8 & 0.45 & 0.294 & 0.281 & 0.008 & 0.286 \\
0.6B teacher-solution start & 5.3 & 0.12 & 0.055 & 0.050 & 0.004 & 0.051 \\
\quad + thinking route & 150.3 & 0.41 & 0.262 & 0.225 & 0.031 & 0.231 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 2.3 & 1.03 & 0.466 & 0.457 & 0.009 & 0.457 \\
\midrule
\multicolumn{7}{@{}l}{\textit{(b) Per benchmark, the five students that write the most answers per sample}} \\
\multicolumn{7}{@{}l}{1.7B teacher-solution start + thinking route} \\*
\quad AIME 2026 & 71.5 & 0.65 & 0.067 & 0.031 & 0.035 & 0.033 \\
\quad AMC23 & 334.5 & 3.13 & 0.372 & 0.180 & 0.191 & 0.181 \\
\quad GSM8K-200 & 150.7 & 1.62 & 0.743 & 0.551 & 0.188 & 0.555 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{0.6B teacher-solution start + thinking route} \\*
\quad AIME 2026 & 43.4 & 0.09 & 0.003 & 0.002 & 0.001 & 0.002 \\
\quad AMC23 & 259.8 & 0.34 & 0.165 & 0.126 & 0.025 & 0.139 \\
\quad GSM8K-200 & 147.7 & 0.79 & 0.620 & 0.546 & 0.067 & 0.553 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{4B non-thinking route} \\*
\quad AIME 2026 & 347.3 & 1.16 & 0.141 & 0.140 & 0.001 & 0.140 \\
\quad AMC23 & 292.8 & 1.19 & 0.587 & 0.585 & 0.001 & 0.586 \\
\quad GSM8K-200 & 2.6 & 1.09 & 0.919 & 0.917 & 0.002 & 0.916 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{1.7B non-thinking route} \\*
\quad AIME 2026 & 36.5 & 1.36 & 0.079 & 0.078 & 0.001 & 0.078 \\
\quad AMC23 & 18.3 & 1.16 & 0.410 & 0.406 & 0.004 & 0.406 \\
\quad GSM8K-200 & 1.5 & 1.10 & 0.830 & 0.830 & 0.000 & 0.830 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{0.6B non-thinking route} \\*
\quad AIME 2026 & 19.6 & 0.94 & 0.018 & 0.017 & 0.001 & 0.017 \\
\quad AMC23 & 12.1 & 1.13 & 0.278 & 0.276 & 0.002 & 0.276 \\
\quad GSM8K-200 & 1.9 & 1.10 & 0.689 & 0.688 & 0.001 & 0.687 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_floors.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{The divergence to the non-thinking teacher settles to a floor ordered by size, and the student's accuracy
on a training problem rises with how often the teacher solves it.} (a)~Per-token divergence to the teacher, the
mean of $|\log\pi_{\text{student}} - \log\pi_{\text{teacher}}|$ over the tokens of the student's own rollouts
before clipping, read from the training log and fitted as $c + a\,e^{-t/\tau}$ from step 10 on; intervals from a
residual bootstrap. The two thinking-route fits are against the thinking teacher and stop at the last logged step.
(b)~Paired, problem-level bootstrap of the gain in strict $p@1$ from the pretrained-only start to the non-thinking
route. The left block is an early analysis that averaged the four benchmarks, GPQA-Diamond included, with the
stored scorer, which under-credits GPQA-Diamond (Appendix~\ref{app:scoring}); its levels are superseded, the paper
averages no scores across GPQA-Diamond and the open-ended benchmarks, and only its interval widths are
informative. The right block is the strict interval on the three open-ended benchmarks from
Appendix~\ref{app:ci}, which the scoring fix does not touch, for comparison. (c)~Strict accuracy of the
non-thinking-route students on training problems in the second epoch (steps 107--212), grouped by how many of the
teacher's four attempts on the problem were correct, for each teacher mode.}
\label{tab:app-floors}
\scriptsize
\setlength{\tabcolsep}{4pt}
{\small (a) Divergence floors}\par\smallskip
\begin{tabular}{lccccccc}
\toprule
& steps & \multicolumn{2}{c}{floor $c$} & \multicolumn{2}{c}{time constant $\tau$ (steps)} & amplitude & residual \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Run & fitted & estimate & 95\% CI & estimate & 95\% CI & $a$ & s.d. \\
\midrule
4B, non-thinking route & 10--212 & 0.161 & [0.159, 0.162] & 6.0 & [5.5, 6.5] & 1.48 & 0.010 \\
1.7B, non-thinking route & 10--212 & 0.254 & [0.252, 0.255] & 8.4 & [7.8, 8.9] & 1.14 & 0.012 \\
0.6B, non-thinking route & 10--212 & 0.341 & [0.338, 0.343] & 8.5 & [7.9, 9.1] & 1.29 & 0.016 \\
\addlinespace[3pt]
4B, thinking route, short-solution start, run 1 & 10--170 & 0.316 & [0.297, 0.330] & 29.0 & [21.1, 40.3] & 0.36 & 0.058 \\
4B, thinking route, short-solution start, run 2 & 10--167 & 0.290 & [0.234, 0.318] & 48.8 & [32.6, 85.7] & 0.32 & 0.069 \\
\bottomrule
\end{tabular}
\par\medskip
{\small (b) Bootstrap gains in strict $p@1$, pretrained-only to non-thinking route}\par\smallskip
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{four benchmarks, stored scorer} & \multicolumn{3}{c}{three open-ended benchmarks} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Student & gain & 95\% CI & width & gain & 95\% CI & width \\
\midrule
4B & $+0.107$ & [$+0.088$, $+0.127$] & 0.040 & $+0.080$ & [$+0.058$, $+0.103$] & 0.046 \\
1.7B & $+0.125$ & [$+0.102$, $+0.150$] & 0.047 & $+0.143$ & [$+0.116$, $+0.174$] & 0.058 \\
0.6B & $+0.253$ & [$+0.229$, $+0.275$] & 0.046 & $+0.280$ & [$+0.250$, $+0.311$] & 0.061 \\
\bottomrule
\end{tabular}
\par\medskip
{\small (c) Accuracy on training problems by the teacher's solve count}\par\smallskip
\begin{tabular}{lcccc}
\toprule
& \multicolumn{4}{c}{teacher's correct attempts out of 4} \\
\cmidrule(lr){2-5}
 & 0/4 & 1--2/4 & 3/4 & 4/4 \\
\midrule
\multicolumn{5}{l}{\textit{grouped by the non-thinking teacher's correct attempts}} \\
\quad problems & 1,653 & 1,262 & 709 & 1,364 \\
\quad 4B non-thinking route & 0.059 & 0.270 & 0.516 & 0.756 \\
\quad 1.7B non-thinking route & 0.034 & 0.116 & 0.257 & 0.485 \\
\quad 0.6B non-thinking route & 0.034 & 0.069 & 0.120 & 0.224 \\
\multicolumn{5}{l}{\textit{grouped by the thinking teacher's correct attempts}} \\
\quad problems & 1,568 & 694 & 519 & 2,207 \\
\quad 4B non-thinking route & 0.109 & 0.246 & 0.355 & 0.593 \\
\quad 1.7B non-thinking route & 0.078 & 0.112 & 0.162 & 0.345 \\
\quad 0.6B non-thinking route & 0.065 & 0.068 & 0.108 & 0.149 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_forced.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{Forcing an answer recovers few unfinished samples, mostly on problems the model could already solve.}
Every unclosed sample of the same-prompt probe (Table~\ref{tab:app-sameprompt}) is fed back to the model that
wrote it with \think{} appended, and the model continues for up to 1{,}024 tokens (temperature 0.6, top-$p$ 0.95,
top-$k$ 20). \emph{Recovered}: the continuation's answer is correct under strict scoring. Groups count how many
of the start model's four samples on that problem were stopped and correct; for the start model the 3--4/4
group holds a single sample. \emph{Continuation hits 1{,}024 tokens}: the fraction of continuations that
reach that limit without finishing.}
\label{tab:app-forced}
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{2}{c}{all unclosed} & \multicolumn{6}{c}{by the start model's correct samples on the problem} & continuation \\
\cmidrule(lr){2-3}\cmidrule(lr){4-9}
& & & \multicolumn{2}{c}{0/4} & \multicolumn{2}{c}{1--2/4} & \multicolumn{2}{c}{3--4/4} & hits \\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
Model & $n$ & recovered & $n$ & recovered & $n$ & recovered & $n$ & recovered & 1{,}024 tokens \\
\midrule
officially post-trained 0.6B, before training & 104 & 0.067 & 84 & 0.036 & 19 & 0.158 & 1 & 1.000 & 0.250 \\
after 20 thinking steps (run 2) & 288 & 0.101 & 206 & 0.049 & 60 & 0.183 & 22 & 0.364 & 0.639 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_gpqa.tex <==
\begin{table}[!htbp]
\centering
\scriptsize
\caption{\textbf{GPQA-Diamond is reported for non-thinking models only, on committed and strict scoring.} (a) The
non-thinking teacher, the pretrained-only students and the non-thinking route. Left: lenient $p@1$ on the three
open-ended benchmarks and their unweighted mean, as in Table~\ref{tab:main}. Right: GPQA-Diamond with the
choice-aware scorer (Table~\ref{tab:app-gpqafix}), scored committed (the last marked answer is the right option)
and strict (the sample also stopped before the cap), never leniently, because with four options any correct
answer anywhere would credit listing several options; it is never averaged with the open-ended benchmarks.
\emph{Minus chance}: committed $p@1$ minus the four-option chance level of 0.250, with a 95\% interval from the
problem bootstrap of Appendix~\ref{app:ci}; grey intervals contain 0. \emph{Truncation}: fraction of samples that
reach the 16{,}384-token cap. Every pretrained-only start is below chance, largely because it often does not
finish an answer; distillation raises every size, but only the distilled 4B is above chance, and the distilled
1.7B and 0.6B are indistinguishable from it. Committed and strict $p@1$ rank the seven models identically.
(b) The fraction of GPQA-Diamond samples that reach the same cap, for every thinking-mode model; their scores
there would reflect the cap rather than the model, and with four options the answer-behavior measurements are
not comparable either. $^\dagger$\,4 samples per problem instead of 8.}
\label{tab:app-gpqa}
\setlength{\tabcolsep}{3pt}
\textit{(a) Non-thinking models}\par\smallskip
\begin{tabular}{@{}lccccccccc@{}}
\toprule
& \multicolumn{4}{c}{Open-ended benchmarks, lenient $p@1$} & \multicolumn{5}{c}{GPQA-Diamond} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-10}
Model & AIME 2026 & AMC23 & GSM8K-200 & mean & \makecell{committed\\$p@1$} & \makecell{minus chance\\{[}95\% CI{]}} & \makecell{strict\\$p@1$} & \makecell{committed\\$p@n$} & truncation \\
\midrule
Teacher (non-thinking) & 0.163 & 0.694 & 0.929 & 0.595 & 0.499 & \makecell{$+0.249$\\$[+0.200, +0.300]$} & 0.497 & 0.808 & 0.026 \\
\addlinespace[2pt]
4B pretrained-only & 0.083 & 0.438 & 0.761 & 0.427 & 0.157 & \makecell{$-0.093$\\$[-0.118, -0.067]$} & 0.157 & 0.606 & 0.462 \\
4B non-thinking route & 0.141 & 0.587 & 0.919 & 0.549 & 0.397 & \makecell{$+0.146$\\$[+0.099, +0.195]$} & 0.361 & 0.798 & 0.125 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.014 & 0.266 & 0.601 & 0.294 & 0.191 & \makecell{$-0.059$\\$[-0.088, -0.028]$} & 0.189 & 0.651 & 0.181 \\
1.7B non-thinking route & 0.079 & 0.410 & 0.830 & 0.440 & 0.275 & \textcolor{cMuted!70}{\makecell{$+0.025$\\$[-0.011, +0.062]$}} & 0.270 & 0.717 & 0.111 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.004 & 0.053 & 0.087 & 0.048 & 0.049 & \makecell{$-0.201$\\$[-0.213, -0.188]$} & 0.049 & 0.288 & 0.581 \\
0.6B non-thinking route & 0.018 & 0.278 & 0.689 & 0.328 & 0.234 & \textcolor{cMuted!70}{\makecell{$-0.016$\\$[-0.047, +0.017]$}} & 0.233 & 0.732 & 0.154 \\
\bottomrule
\end{tabular}
\par\bigskip
\textit{(b) Thinking-mode models, fraction of GPQA-Diamond samples truncated (scores not reported)}\par\smallskip
\begin{tabular}{@{}lc@{\hspace{2.5em}}lc@{}}
\toprule
Model & truncation & Model & truncation \\
\midrule
Teacher (thinking) & 0.095 & 1.7B teacher-solution start & 0.799 \\
4B short-solution start & 0.401 & 1.7B teacher-solution start + thinking route & 1.000 \\
4B short-solution start + thinking route & 0.397 & 0.6B short-solution start & 0.354 \\
4B teacher-solution start & 0.742 & 0.6B short-solution start + thinking route & 0.750 \\
4B teacher-solution start + thinking route & 0.410 & 0.6B teacher-solution start & 0.915 \\
4B teacher-solution start + thinking route, 212 steps & 0.387 & 0.6B teacher-solution start + thinking route & 1.000 \\
1.7B short-solution start & 0.522 & officially post-trained 0.6B$^\dagger$ & 0.035 \\
1.7B short-solution start + thinking route & 0.685 & officially post-trained 0.6B + 20 thinking steps (16{,}384)$^\dagger$ & 0.351 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_gpqafix.tex <==
\begin{table}[!htbp]
\centering
\scriptsize
\caption{\textbf{The GPQA-Diamond scoring fix lands almost entirely on the non-thinking models.} Committed and
strict $p@1$ on GPQA-Diamond as originally scored and after the choice-aware fix; GPQA-Diamond is never scored
leniently in this paper, because with four options any correct answer anywhere would credit listing several
options. The original scorer credited a multiple-choice answer only when the boxed content was a bare letter,
so \texttt{\textbackslash boxed\{\textbackslash text\{A\}\}} or \texttt{\textbackslash boxed\{D.\ 33.4\}}
scored 0 with the right key. The fix reads the leading option letter; it is gated on a single-letter ground
truth, so the three open-ended benchmarks are bit-identical before and after, and it only adds credit. The
non-thinking teacher gains the most. Among the thinking-mode models, every endpoint of the two thinking routes
changes by at most 0.001 and their cold starts by at most 0.002; the thinking teacher changes by 0.008, and
the officially post-trained 0.6B by 0.013 before and 0.004 after 20 thinking steps. \emph{Samples}: samples
per problem; \emph{trunc.}: fraction of samples that reach the 16{,}384-token cap, which is why GPQA-Diamond is
reported only for non-thinking models (Table~\ref{tab:app-gpqa}).}
\label{tab:app-gpqafix}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llccccccc@{}}
\toprule
& & & \multicolumn{3}{c}{Committed $p@1$} & \multicolumn{2}{c}{Strict $p@1$} & \\
\cmidrule(lr){4-6}\cmidrule(lr){7-8}
Model & Mode & Samples & original & fixed & change & original & fixed & Trunc. \\
\midrule
Teacher (thinking) & thinking & 8 & 0.555 & 0.562 & $+0.008$ & 0.546 & 0.554 & 0.095 \\
Teacher (non-thinking) & non-thinking & 8 & 0.254 & 0.499 & $+0.246$ & 0.253 & 0.497 & 0.026 \\
\addlinespace[2pt]
4B pretrained-only & non-thinking & 8 & 0.141 & 0.157 & $+0.016$ & 0.140 & 0.157 & 0.462 \\
4B non-thinking route & non-thinking & 8 & 0.365 & 0.397 & $+0.031$ & 0.331 & 0.361 & 0.125 \\
4B short-solution start & thinking & 8 & 0.295 & 0.295 & $+0.000$ & 0.295 & 0.295 & 0.401 \\
\quad + thinking route & thinking & 8 & 0.342 & 0.342 & $+0.000$ & 0.328 & 0.328 & 0.397 \\
4B teacher-solution start & thinking & 8 & 0.117 & 0.117 & $+0.000$ & 0.064 & 0.064 & 0.742 \\
\quad + thinking route & thinking & 8 & 0.323 & 0.323 & $+0.001$ & 0.313 & 0.314 & 0.410 \\
\quad + thinking route, 212 steps & thinking & 8 & 0.340 & 0.340 & $+0.000$ & 0.324 & 0.324 & 0.387 \\
\addlinespace[2pt]
1.7B pretrained-only & non-thinking & 8 & 0.182 & 0.191 & $+0.008$ & 0.181 & 0.189 & 0.181 \\
1.7B non-thinking route & non-thinking & 8 & 0.253 & 0.275 & $+0.021$ & 0.250 & 0.270 & 0.111 \\
1.7B short-solution start & thinking & 8 & 0.168 & 0.170 & $+0.002$ & 0.161 & 0.163 & 0.522 \\
\quad + thinking route & thinking & 8 & 0.139 & 0.139 & $+0.000$ & 0.122 & 0.122 & 0.685 \\
1.7B teacher-solution start & thinking & 8 & 0.034 & 0.034 & $+0.000$ & 0.018 & 0.018 & 0.799 \\
\quad + thinking route & thinking & 8 & 0.072 & 0.072 & $+0.000$ & 0.000 & 0.000 & 1.000 \\
\addlinespace[2pt]
0.6B pretrained-only & non-thinking & 8 & 0.042 & 0.049 & $+0.007$ & 0.042 & 0.049 & 0.581 \\
0.6B non-thinking route & non-thinking & 8 & 0.212 & 0.234 & $+0.022$ & 0.211 & 0.233 & 0.154 \\
0.6B short-solution start & thinking & 8 & 0.189 & 0.191 & $+0.002$ & 0.169 & 0.170 & 0.354 \\
\quad + thinking route & thinking & 8 & 0.085 & 0.085 & $+0.000$ & 0.071 & 0.071 & 0.750 \\
0.6B teacher-solution start & thinking & 8 & 0.018 & 0.018 & $+0.000$ & 0.014 & 0.014 & 0.915 \\
\quad + thinking route & thinking & 8 & 0.061 & 0.061 & $+0.000$ & 0.000 & 0.000 & 1.000 \\
\addlinespace[2pt]
officially post-trained 0.6B & thinking & 4 & 0.261 & 0.274 & $+0.013$ & 0.261 & 0.274 & 0.035 \\
\quad + 20 thinking steps (16{,}384) & thinking & 4 & 0.186 & 0.189 & $+0.004$ & 0.178 & 0.182 & 0.351 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_hparams.tex <==
\begin{table}[!htbp]
\centering
\footnotesize
\caption{\textbf{Settings shared by every run, and the few that differ.} Distillation, cold-start fine-tuning,
data and evaluation settings, read from the launch scripts and configurations. The student, the data and the
optimizer are the same in both arms; only the teacher's mode, the student's starting point and, in the budget
controls, the rollout budget change between runs.}
\label{tab:app-hparams}
\begin{tabularx}{\linewidth}{@{}p{3.1cm}>{\raggedright\arraybackslash}X@{}}
\toprule
Setting & Value \\
\midrule
\multicolumn{2}{@{}l}{\textbf{On-policy distillation (all runs)}} \\
Teacher & Qwen3-8B, one set of weights in two modes; the student runs in the teacher's mode \\
Rollouts & one response per prompt, temperature 1.0, 128 prompts per step \\
Per-token advantage & $A_t=-\mathrm{clip}(\log\pi_{\text{student}}-\log\pi_{\text{teacher}},-1,1)$ on the student's own tokens; no task reward \\
End-of-thinking token & scored like every other token \\
Update & PPO-style clipped policy gradient, mini-batch 32 (4 updates per step) \\
Loss aggregation & sequence mean of token sums, divided by a constant equal to the rollout budget \\
Optimizer & AdamW, learning rate $3\times10^{-6}$, constant after 10 warm-up steps, gradient clipping 1.0, weight decay 0.01 \\
Length & 2 epochs = 212 steps \\
Rollout budget & 7{,}168 tokens \\
Checkpoints & saved every 71 steps, last three kept; the runs of the three routes keep only the evaluated step, while the 1{,}024-token, curriculum and officially post-trained 0.6B runs also hold intermediate checkpoints (Appendix~\ref{app:notes}) \\
\addlinespace[3pt]
\multicolumn{2}{@{}l}{\textbf{Run-specific departures}} \\
16{,}384-token runs & loss constant kept at 7{,}168, so only the rollout budget changes \\
1{,}024-token run & mini-batch 128 (one update per step), loss constant 1{,}024 \\
Curriculum runs & 99 steps over 12{,}741 problems ordered easy to hard (non-thinking arm) \\
\addlinespace[3pt]
\multicolumn{2}{@{}l}{\textbf{Cold-start supervised fine-tuning (identical recipe at every size)}} \\
Short external solutions & every solution of at most 2{,}048 tokens in SFT-Math-45k, a quality-filtered subset of OpenR1-Math-220k (Apache-2.0): 5{,}878 solutions, mean 1{,}530 tokens; maximum sequence length 4{,}096 \\
The teacher's own solutions & the shortest correct of the thinking teacher's 4 samples per problem (5{,}000 training problems, temperature 0.6, top-$p$ 0.95, top-$k$ 20), if at most 7{,}000 tokens and not mainly Chinese: 1{,}524 solutions, mean 4{,}809 tokens; maximum sequence length 10{,}240 \\
Optimization & global batch 16, AdamW, learning rate $2\times10^{-5}$, cosine to $0.1\times$, warm-up ratio 0.01, 2 epochs \\
Target & loss on the response only; the chat template keeps the thinking block in the target \\
\addlinespace[3pt]
\multicolumn{2}{@{}l}{\textbf{Training data}} \\
Source & DAPO-Math-17k, 17{,}398 problems \\
Cleaning & 15{,}827 problems remain \\
Exact duplicates & 924 removed \\
Near-duplicates & 167 removed (13-gram Jaccard similarity $\ge 0.7$) \\
Decontamination & 1{,}139 removed against AIME 2024--2026, AMC23 and MATH; GSM8K was not in the list \\
Training set & 13{,}597 problems; 12{,}741 in the curriculum runs, which drop 856 problems whose statements were truncated upstream \\
\addlinespace[3pt]
\multicolumn{2}{@{}l}{\textbf{Evaluation}} \\
AIME 2026 & 30 problems, 48 samples per problem, cap 30{,}720 tokens \\
AMC23 & 40 problems, 48 samples per problem, cap 30{,}720 tokens \\
GSM8K-200 & 200 problems, 32 samples per problem, cap 8{,}192 tokens \\
GPQA-Diamond & 198 problems, 8 samples per problem, cap 16{,}384 tokens (reported for non-thinking models only) \\
Sampling & temperature 0.6, top-$p$ 0.95, top-$k$ 20 \\
Checkpoints & fixed steps (142, 212, or 20 for the officially post-trained start); none selected \\
Reduced evaluations & the officially post-trained 0.6B, that model after 20 steps, and the 1{,}024-token run (Table~\ref{tab:app-runs}) \\
In-training validation & every 20 steps on AIME 2025 (30) and AMC23 (40), 8 samples, temperature 0.6, at a 16{,}384-token cap, above the rollout budget; never used to select \\
\addlinespace[3pt]
\multicolumn{2}{@{}l}{\textbf{Compute}} \\
Hardware and cost & 3 nodes of 4 A100-40GB: the teacher on one node (vLLM), the student on two (FSDP); a 212-step 4B run takes about 11 hours \\
\bottomrule
\end{tabularx}
\end{table}



==> tables/app_length.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{The median rollout reaches whatever budget it is given.} (a)~Median response length on training
rollouts as a fraction of that run's own rollout budget, over the first ten steps and at steps 20 and 30
(lengths re-tokenized with each student's own tokenizer). (b)~The 0.6B cold-started on short external
solutions at three rollout budgets, same model and training problems: absolute median length in tokens and
the fraction of rollouts that reach the budget. At 7{,}168 and 16{,}384 tokens the median leaves its early
level at step 5 or 6 and sits at the budget by step 7; at 1{,}024 tokens it is at the budget from the first
step. The same model therefore has no target length of its own. Rows as in Table~\ref{tab:app-windows};
runs whose rollouts were not re-tokenized are omitted.}
\label{tab:app-length}
\scriptsize
\setlength{\tabcolsep}{3.2pt}
{\small (a) Median length / rollout budget}\par\smallskip
\begin{tabular}{lccccccccccccc}
\toprule
& & \multicolumn{12}{c}{training step} \\
\cmidrule(lr){3-14}
Run & budget & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 20 & 30 \\
\midrule
\multicolumn{14}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 7,168 & 0.65 & 0.64 & 0.75 & 0.73 & 0.96 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\quad 4B, run 2$^\dagger$ & 7,168 & 0.63 & 0.65 & 0.64 & 0.73 & 0.84 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\quad 1.7B & 7,168 & 0.68 & 0.71 & 0.64 & 0.72 & 0.93 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\quad 0.6B, run 2$^\dagger$ & 7,168 & 0.54 & 0.53 & 0.54 & 0.50 & 0.68 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\addlinespace[3pt]
\multicolumn{14}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 7,168 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\quad 1.7B & 7,168 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\quad 0.6B & 7,168 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\addlinespace[3pt]
\multicolumn{14}{l}{\textit{0.6B cold-started on short external solutions, other rollout budgets}} \\
\quad 1,024-token budget & 1,024 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\quad 16,384-token budget & 16,384 & 0.26 & 0.20 & 0.23 & 0.21 & 0.27 & 0.59 & 1.00 & -- & -- & -- & -- & -- \\
\addlinespace[3pt]
\multicolumn{14}{l}{\textit{Officially post-trained 0.6B, 16,384-token budget}} \\
\quad thinking template, run 1 & 16,384 & 0.80 & 0.66 & 0.74 & 0.71 & 0.83 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & -- \\
\quad thinking template, run 2$^\dagger$ & 16,384 & 0.79 & 0.67 & 0.66 & 0.72 & 0.88 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & -- \\
\quad non-thinking template & 16,384 & 0.05 & 0.06 & 0.05 & 0.06 & 0.07 & 0.09 & 0.12 & 0.14 & 0.17 & 0.17 & 0.15 & -- \\
\addlinespace[3pt]
\multicolumn{14}{l}{\textit{Non-thinking route, pretrained-only start}} \\
\quad 4B & 7,168 & 0.11 & 0.12 & 0.13 & 0.12 & 0.14 & 0.13 & 0.13 & 0.16 & 0.15 & 0.16 & 0.24 & 0.25 \\
\quad 1.7B & 7,168 & 0.06 & 0.07 & 0.07 & 0.08 & 0.08 & 0.08 & 0.08 & 0.10 & 0.12 & 0.11 & 0.26 & 0.26 \\
\quad 0.6B & 7,168 & 0.10 & 0.12 & 0.10 & 0.10 & 0.11 & 0.11 & 0.11 & 0.11 & 0.10 & 0.14 & 0.33 & 0.32 \\
\bottomrule
\end{tabular}
\par\medskip
{\small (b) The three rollout budgets at 0.6B, steps 1--7}\par\smallskip
\begin{tabular}{lccccccc}
\toprule
& \multicolumn{7}{c}{training step} \\
\cmidrule(lr){2-8}
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\
\midrule
\multicolumn{8}{l}{\textit{1,024-token budget}} \\
\quad median tokens & 1,024 & 1,024 & 1,024 & 1,024 & 1,024 & 1,024 & 1,024 \\
\quad fraction at the budget & 0.852 & 0.883 & 0.852 & 0.867 & 0.883 & 0.875 & 0.938 \\
\addlinespace[3pt]
\multicolumn{8}{l}{\textit{7,168-token budget (run 2)}} \\
\quad median tokens & 3,882 & 3,801 & 3,840 & 3,575 & 4,895 & 7,167 & 7,168 \\
\quad fraction at the budget & 0.180 & 0.102 & 0.109 & 0.133 & 0.227 & 0.617 & 0.836 \\
\addlinespace[3pt]
\multicolumn{8}{l}{\textit{16,384-token budget}} \\
\quad median tokens & 4,227 & 3,196 & 3,723 & 3,515 & 4,378 & 9,666 & 16,384 \\
\quad fraction at the budget & 0.008 & 0.039 & 0.031 & 0.000 & 0.031 & 0.320 & 0.789 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_matched.tex <==
\begin{table}[!htbp]
\centering
\scriptsize
\caption{\textbf{Accuracy given an answer rises along every route once both models are scored on the same
problems.} \emph{Answered}: problems on which model A / model B wrote at least one marked answer, out of
30, 40 and 200. \emph{Common}: problems both answered; the matched accuracy of each model is its accuracy
given an answer on those problems, averaged with equal weight per problem, and the mean rows average the
three benchmarks. \emph{Unmatched}: the same problem-weighted accuracy over each model's own answered
problems, which flatters a model that answers only the problems it finds easy. Weighting samples instead of
problems inflates these changes to roughly $+0.20$ at every size, because a model that answers more
contributes many samples on easy problems. Intervals as in Table~\ref{tab:app-ci}; those that contain 0 are
in grey.
The only non-positive matched changes are on AIME 2026 at 0.6B, where accuracy is a few percent on 13 to
30 problems.}
\label{tab:app-matched}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llccccc@{}}
\toprule
& & Answered & & Unmatched & Matched & Matched change \\
Size & Benchmark & A / B & Common & A $\to$ B & A $\to$ B & B $-$ A [95\% CI] \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Pretrained-only start (A) $\to$ non-thinking route (B)}} \\*
4B & AIME 2026 & 30 / 30 & 30 & 0.095\,$\to$\,0.147 & 0.095\,$\to$\,0.147 & $+0.052$ $[+0.009, +0.109]$ \\
 & AMC23 & 40 / 40 & 40 & 0.505\,$\to$\,0.596 & 0.505\,$\to$\,0.596 & $+0.091$ $[+0.048, +0.136]$ \\
 & GSM8K-200 & 200 / 200 & 200 & 0.873\,$\to$\,0.919 & 0.873\,$\to$\,0.919 & $+0.046$ $[+0.027, +0.066]$ \\
 & mean & -- & 270 & 0.491\,$\to$\,0.554 & 0.491\,$\to$\,0.554 & $+0.063$ $[+0.041, +0.088]$ \\
\addlinespace[2pt]
1.7B & AIME 2026 & 30 / 30 & 30 & 0.018\,$\to$\,0.085 & 0.018\,$\to$\,0.085 & $+0.067$ $[+0.005, +0.141]$ \\
 & AMC23 & 40 / 40 & 40 & 0.330\,$\to$\,0.434 & 0.330\,$\to$\,0.434 & $+0.104$ $[+0.060, +0.150]$ \\
 & GSM8K-200 & 199 / 200 & 199 & 0.763\,$\to$\,0.830 & 0.763\,$\to$\,0.834 & $+0.070$ $[+0.046, +0.096]$ \\
 & mean & -- & 269 & 0.371\,$\to$\,0.450 & 0.371\,$\to$\,0.451 & $+0.080$ $[+0.054, +0.111]$ \\
\addlinespace[2pt]
0.6B & AIME 2026 & 30 / 30 & 30 & 0.030\,$\to$\,0.023 & 0.030\,$\to$\,0.023 & \textcolor{cMuted!70}{$-0.008$ $[-0.040, +0.021]$} \\
 & AMC23 & 40 / 40 & 40 & 0.231\,$\to$\,0.302 & 0.231\,$\to$\,0.302 & $+0.071$ $[+0.005, +0.134]$ \\
 & GSM8K-200 & 194 / 200 & 194 & 0.483\,$\to$\,0.692 & 0.483\,$\to$\,0.695 & $+0.212$ $[+0.177, +0.247]$ \\
 & mean & -- & 264 & 0.248\,$\to$\,0.339 & 0.248\,$\to$\,0.340 & $+0.092$ $[+0.065, +0.118]$ \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Short-solution start (A) $\to$ thinking route (B)}} \\*
4B & AIME 2026 & 30 / 29 & 29 & 0.177\,$\to$\,0.522 & 0.184\,$\to$\,0.522 & $+0.338$ $[+0.217, +0.469]$ \\
 & AMC23 & 40 / 39 & 39 & 0.639\,$\to$\,0.864 & 0.654\,$\to$\,0.864 & $+0.210$ $[+0.132, +0.291]$ \\
 & GSM8K-200 & 200 / 200 & 200 & 0.913\,$\to$\,0.935 & 0.913\,$\to$\,0.935 & $+0.022$ $[+0.005, +0.039]$ \\
 & mean & -- & 268 & 0.576\,$\to$\,0.773 & 0.584\,$\to$\,0.773 & $+0.190$ $[+0.142, +0.243]$ \\
\addlinespace[2pt]
1.7B & AIME 2026 & 30 / 21 & 21 & 0.059\,$\to$\,0.186 & 0.084\,$\to$\,0.186 & $+0.102$ $[+0.027, +0.194]$ \\
 & AMC23 & 40 / 35 & 35 & 0.387\,$\to$\,0.571 & 0.433\,$\to$\,0.571 & $+0.137$ $[+0.076, +0.206]$ \\
 & GSM8K-200 & 200 / 200 & 200 & 0.799\,$\to$\,0.879 & 0.799\,$\to$\,0.879 & $+0.080$ $[+0.057, +0.103]$ \\
 & mean & -- & 256 & 0.415\,$\to$\,0.545 & 0.439\,$\to$\,0.545 & $+0.106$ $[+0.072, +0.145]$ \\
\addlinespace[2pt]
0.6B & AIME 2026 & 30 / 24 & 24 & 0.010\,$\to$\,0.016 & 0.010\,$\to$\,0.016 & \textcolor{cMuted!70}{$+0.007$ $[-0.004, +0.022]$} \\
 & AMC23 & 40 / 39 & 39 & 0.228\,$\to$\,0.389 & 0.231\,$\to$\,0.389 & $+0.158$ $[+0.089, +0.232]$ \\
 & GSM8K-200 & 200 / 198 & 198 & 0.614\,$\to$\,0.800 & 0.619\,$\to$\,0.800 & $+0.181$ $[+0.150, +0.211]$ \\
 & mean & -- & 261 & 0.284\,$\to$\,0.402 & 0.286\,$\to$\,0.402 & $+0.115$ $[+0.089, +0.142]$ \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Teacher-solution start (A) $\to$ thinking route (B)}} \\*
4B & AIME 2026 & 20 / 29 & 20 & 0.368\,$\to$\,0.503 & 0.368\,$\to$\,0.606 & $+0.238$ $[+0.138, +0.354]$ \\
 & AMC23 & 38 / 39 & 37 & 0.827\,$\to$\,0.881 & 0.849\,$\to$\,0.915 & $+0.067$ $[+0.008, +0.131]$ \\
 & GSM8K-200 & 197 / 200 & 197 & 0.920\,$\to$\,0.927 & 0.920\,$\to$\,0.926 & \textcolor{cMuted!70}{$+0.006$ $[-0.009, +0.022]$} \\
 & mean & -- & 254 & 0.705\,$\to$\,0.771 & 0.713\,$\to$\,0.816 & $+0.104$ $[+0.063, +0.147]$ \\
\addlinespace[2pt]
1.7B & AIME 2026 & 16 / 17 & 12 & 0.135\,$\to$\,0.253 & 0.181\,$\to$\,0.282 & $+0.101$ $[+0.007, +0.225]$ \\
 & AMC23 & 29 / 34 & 28 & 0.662\,$\to$\,0.615 & 0.686\,$\to$\,0.722 & \textcolor{cMuted!70}{$+0.036$ $[-0.043, +0.115]$} \\
 & GSM8K-200 & 196 / 200 & 196 & 0.830\,$\to$\,0.875 & 0.830\,$\to$\,0.877 & $+0.047$ $[+0.024, +0.071]$ \\
 & mean & -- & 236 & 0.542\,$\to$\,0.581 & 0.566\,$\to$\,0.627 & $+0.061$ $[+0.018, +0.110]$ \\
\addlinespace[2pt]
0.6B & AIME 2026 & 19 / 19 & 13 & 0.035\,$\to$\,0.025 & 0.051\,$\to$\,0.036 & \textcolor{cMuted!70}{$-0.015$ $[-0.071, +0.019]$} \\
 & AMC23 & 32 / 32 & 27 & 0.286\,$\to$\,0.410 & 0.326\,$\to$\,0.484 & $+0.158$ $[+0.070, +0.255]$ \\
 & GSM8K-200 & 184 / 193 & 180 & 0.724\,$\to$\,0.818 & 0.729\,$\to$\,0.846 & $+0.118$ $[+0.081, +0.156]$ \\
 & mean & -- & 220 & 0.348\,$\to$\,0.417 & 0.369\,$\to$\,0.455 & $+0.087$ $[+0.051, +0.124]$ \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_nullmodel.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{Lengthening alone reproduces most of the lost wrong closes but not the kept correct ones.} The
same-prompt probe of Table~\ref{tab:app-sameprompt}, pooled over its 128 problems (512 samples per
model): the officially post-trained 0.6B before training, a null model built from those same samples, and the
model after 20 steps of distillation from the thinking teacher (16{,}384-token budget, run~2). The null model
multiplies the position at which each start-model sample closes by one factor $k$ and keeps the close only if
it still falls within the probe's 16{,}384-token limit; everything else about the sample, including its
answer, is unchanged. $k$ is fitted so that the null model's closure matches the observed closure after
training, so the first column agrees by construction; the other two columns are the test. Cells are fractions
of all samples; the last two add up to the first. No interval was computed for this comparison.}
\label{tab:app-nullmodel}
\footnotesize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccc}
\toprule
& closed & closed and correct & closed and wrong \\
\midrule
start model, before training & 0.797 & 0.305 & 0.492 \\
\addlinespace[2pt]
null model: start model's closes stretched by $k = 1.71$ & 0.439 & 0.229 & 0.211 \\
observed after 20 thinking steps & 0.438 & 0.311 & 0.127 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_passk.tex <==
\begingroup
\scriptsize
\setlength{\tabcolsep}{4pt}
\setlength{\LTcapwidth}{\linewidth}
\begin{longtable}{>{\raggedright\arraybackslash}p{4.3cm}cccccccc@{}}
\caption{\textbf{Strict pass@$k$ on the three open-ended benchmarks.} The unbiased estimate of the probability
that at least one of $k$ samples is strictly correct (closed or stopped before the cap,
and correct), from the $n$ samples per problem; $k=1$ equals strict $p@1$ in Table~\ref{tab:app-scores}.
Columns beyond $n$ are empty. The 1.7B and 0.6B students distilled from the thinking teacher after the
teacher-solution start never close their reasoning at evaluation, so every entry is 0.000 for them; their
lenient and committed scores are in Table~\ref{tab:app-scores}.}\label{tab:app-passk}\\
\toprule
Model & $n$ & $k=1$ & $k=2$ & $k=4$ & $k=8$ & $k=16$ & $k=32$ & $k=48$ \\
\midrule
\endfirsthead
\multicolumn{9}{l}{\textit{Table~\ref{tab:app-passk}, continued}}\\
\toprule
Model & $n$ & $k=1$ & $k=2$ & $k=4$ & $k=8$ & $k=16$ & $k=32$ & $k=48$ \\
\midrule
\endhead
\midrule
\multicolumn{9}{r}{\textit{continued on the next page}}\\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{9}{@{}l}{\textbf{AIME 2026}\quad 30 problems, 48 samples each, 30{,}720-token cap} \\*
Teacher (thinking) & 48 & 0.667 & 0.758 & 0.820 & 0.859 & 0.883 & 0.896 & 0.900 \\
Teacher (non-thinking) & 48 & 0.163 & 0.218 & 0.290 & 0.379 & 0.477 & 0.589 & 0.667 \\
\addlinespace[2pt]
4B pretrained-only & 48 & 0.083 & 0.125 & 0.172 & 0.224 & 0.277 & 0.317 & 0.333 \\
4B non-thinking route & 48 & 0.117 & 0.157 & 0.201 & 0.249 & 0.305 & 0.363 & 0.400 \\
4B short-solution start & 48 & 0.146 & 0.200 & 0.247 & 0.291 & 0.332 & 0.374 & 0.400 \\
\quad + thinking route & 48 & 0.322 & 0.392 & 0.446 & 0.502 & 0.569 & 0.648 & 0.700 \\
4B teacher-solution start & 48 & 0.084 & 0.136 & 0.195 & 0.252 & 0.306 & 0.348 & 0.367 \\
\quad + thinking route & 48 & 0.304 & 0.385 & 0.462 & 0.537 & 0.616 & 0.692 & 0.733 \\
\quad + thinking route, 212 steps & 48 & 0.319 & 0.390 & 0.452 & 0.511 & 0.570 & 0.617 & 0.633 \\
\addlinespace[2pt]
1.7B pretrained-only & 48 & 0.014 & 0.026 & 0.045 & 0.070 & 0.097 & 0.121 & 0.133 \\
1.7B non-thinking route & 48 & 0.078 & 0.108 & 0.133 & 0.156 & 0.185 & 0.230 & 0.267 \\
1.7B short-solution start & 48 & 0.026 & 0.046 & 0.074 & 0.107 & 0.142 & 0.181 & 0.200 \\
\quad + thinking route & 48 & 0.051 & 0.076 & 0.100 & 0.120 & 0.138 & 0.155 & 0.167 \\
1.7B teacher-solution start & 48 & 0.008 & 0.015 & 0.028 & 0.049 & 0.075 & 0.096 & 0.100 \\
\quad + thinking route & 48 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\addlinespace[2pt]
0.6B pretrained-only & 48 & 0.002 & 0.004 & 0.008 & 0.016 & 0.030 & 0.052 & 0.067 \\
0.6B non-thinking route & 48 & 0.017 & 0.031 & 0.052 & 0.075 & 0.096 & 0.119 & 0.133 \\
0.6B short-solution start & 48 & 0.004 & 0.008 & 0.016 & 0.029 & 0.049 & 0.077 & 0.100 \\
\quad + thinking route & 48 & 0.001 & 0.001 & 0.003 & 0.006 & 0.011 & 0.022 & 0.033 \\
0.6B teacher-solution start & 48 & 0.001 & 0.001 & 0.003 & 0.006 & 0.011 & 0.022 & 0.033 \\
\quad + thinking route & 48 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\addlinespace[2pt]
officially post-trained 0.6B & 16 & 0.110 & 0.162 & 0.208 & 0.249 & 0.267 & -- & -- \\
\midrule
\multicolumn{9}{@{}l}{\textbf{AMC23}\quad 40 problems, 48 samples each, 30{,}720-token cap} \\*
Teacher (thinking) & 48 & 0.955 & 0.983 & 0.995 & 0.999 & 1.000 & 1.000 & 1.000 \\
Teacher (non-thinking) & 48 & 0.692 & 0.787 & 0.863 & 0.915 & 0.947 & 0.966 & 0.975 \\
\addlinespace[2pt]
4B pretrained-only & 48 & 0.436 & 0.564 & 0.673 & 0.765 & 0.832 & 0.878 & 0.900 \\
4B non-thinking route & 48 & 0.486 & 0.613 & 0.723 & 0.808 & 0.861 & 0.889 & 0.900 \\
4B short-solution start & 48 & 0.543 & 0.650 & 0.752 & 0.844 & 0.898 & 0.917 & 0.925 \\
\quad + thinking route & 48 & 0.721 & 0.793 & 0.835 & 0.862 & 0.881 & 0.896 & 0.900 \\
4B teacher-solution start & 48 & 0.285 & 0.432 & 0.569 & 0.677 & 0.764 & 0.830 & 0.875 \\
\quad + thinking route & 48 & 0.719 & 0.801 & 0.851 & 0.881 & 0.905 & 0.921 & 0.925 \\
\quad + thinking route, 212 steps & 48 & 0.750 & 0.825 & 0.867 & 0.901 & 0.934 & 0.963 & 0.975 \\
\addlinespace[2pt]
1.7B pretrained-only & 48 & 0.266 & 0.394 & 0.517 & 0.615 & 0.693 & 0.771 & 0.825 \\
1.7B non-thinking route & 48 & 0.403 & 0.512 & 0.623 & 0.726 & 0.812 & 0.871 & 0.900 \\
1.7B short-solution start & 48 & 0.287 & 0.381 & 0.474 & 0.568 & 0.661 & 0.744 & 0.775 \\
\quad + thinking route & 48 & 0.330 & 0.395 & 0.448 & 0.496 & 0.546 & 0.610 & 0.650 \\
1.7B teacher-solution start & 48 & 0.065 & 0.116 & 0.191 & 0.280 & 0.365 & 0.437 & 0.475 \\
\quad + thinking route & 48 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\addlinespace[2pt]
0.6B pretrained-only & 48 & 0.051 & 0.093 & 0.160 & 0.258 & 0.381 & 0.509 & 0.575 \\
0.6B non-thinking route & 48 & 0.275 & 0.383 & 0.483 & 0.561 & 0.623 & 0.676 & 0.700 \\
0.6B short-solution start & 48 & 0.147 & 0.232 & 0.328 & 0.429 & 0.537 & 0.635 & 0.675 \\
\quad + thinking route & 48 & 0.149 & 0.209 & 0.264 & 0.309 & 0.353 & 0.420 & 0.475 \\
0.6B teacher-solution start & 48 & 0.017 & 0.032 & 0.061 & 0.109 & 0.182 & 0.282 & 0.350 \\
\quad + thinking route & 48 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\addlinespace[2pt]
officially post-trained 0.6B & 16 & 0.491 & 0.625 & 0.744 & 0.840 & 0.900 & -- & -- \\
\midrule
\multicolumn{9}{@{}l}{\textbf{GSM8K-200}\quad 200 problems, 32 samples each, 8{,}192-token cap} \\*
Teacher (thinking) & 32 & 0.934 & 0.944 & 0.949 & 0.953 & 0.956 & 0.960 & -- \\
Teacher (non-thinking) & 32 & 0.928 & 0.944 & 0.953 & 0.959 & 0.963 & 0.965 & -- \\
\addlinespace[2pt]
4B pretrained-only & 32 & 0.758 & 0.894 & 0.946 & 0.962 & 0.970 & 0.975 & -- \\
4B non-thinking route & 32 & 0.913 & 0.940 & 0.953 & 0.964 & 0.973 & 0.980 & -- \\
4B short-solution start & 32 & 0.899 & 0.936 & 0.955 & 0.967 & 0.975 & 0.980 & -- \\
\quad + thinking route & 32 & 0.891 & 0.926 & 0.944 & 0.954 & 0.960 & 0.965 & -- \\
4B teacher-solution start & 32 & 0.312 & 0.497 & 0.687 & 0.819 & 0.886 & 0.925 & -- \\
\quad + thinking route & 32 & 0.884 & 0.922 & 0.940 & 0.950 & 0.958 & 0.965 & -- \\
\quad + thinking route, 212 steps & 32 & 0.852 & 0.920 & 0.947 & 0.959 & 0.964 & 0.965 & -- \\
\addlinespace[2pt]
1.7B pretrained-only & 32 & 0.601 & 0.777 & 0.883 & 0.936 & 0.965 & 0.980 & -- \\
1.7B non-thinking route & 32 & 0.830 & 0.888 & 0.920 & 0.941 & 0.958 & 0.975 & -- \\
1.7B short-solution start & 32 & 0.705 & 0.838 & 0.906 & 0.942 & 0.965 & 0.985 & -- \\
\quad + thinking route & 32 & 0.734 & 0.835 & 0.890 & 0.923 & 0.944 & 0.960 & -- \\
1.7B teacher-solution start & 32 & 0.126 & 0.228 & 0.379 & 0.557 & 0.716 & 0.825 & -- \\
\quad + thinking route & 32 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & -- \\
\addlinespace[2pt]
0.6B pretrained-only & 32 & 0.086 & 0.154 & 0.261 & 0.408 & 0.577 & 0.730 & -- \\
0.6B non-thinking route & 32 & 0.687 & 0.774 & 0.836 & 0.881 & 0.918 & 0.945 & -- \\
0.6B short-solution start & 32 & 0.450 & 0.622 & 0.748 & 0.827 & 0.876 & 0.910 & -- \\
\quad + thinking route & 32 & 0.602 & 0.714 & 0.776 & 0.822 & 0.859 & 0.885 & -- \\
0.6B teacher-solution start & 32 & 0.075 & 0.141 & 0.250 & 0.404 & 0.572 & 0.720 & -- \\
\quad + thinking route & 32 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & -- \\
\addlinespace[2pt]
0.6B short-solution start, 1{,}024-token budget & 4 & 0.226 & 0.361 & 0.495 & -- & -- & -- & -- \\
officially post-trained 0.6B & 4 & 0.769 & 0.842 & 0.890 & -- & -- & -- & -- \\
\quad + 20 thinking steps (16{,}384) & 4 & 0.749 & 0.803 & 0.850 & -- & -- & -- & -- \\
\end{longtable}
\endgroup



==> tables/app_reflection.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{Rollouts lengthen in every run, and the loop rate falls in every run except the 16{,}384-token run.}
Training rollouts in the first five steps against a late window (steps 101 to the last logged step, every
fifth step; for shorter runs, the last window they reached). \emph{Median characters}: median rollout length
in characters and its late-to-early ratio. \emph{Loop rate}: among rollouts longer than 5{,}000 characters,
the fraction whose last 4{,}000 characters contain one substring of 30, 60, 120 or 240 characters repeated at
least five times. This is a different rule from the one in Table~\ref{tab:app-unfinished-train} (one line repeated at
least five times in the last 2{,}000 characters), and the two rates are not comparable. \emph{Reflection
words}: occurrences of \emph{Wait}, \emph{wait} and \emph{Hmm} (and the Chinese word for \emph{wait}) per
1{,}000 characters, counted over the first 20{,}000 characters of each rollout. The runs cold-started on the
teacher's own solutions are not included in this analysis. Rows as in Table~\ref{tab:app-windows}.}
\label{tab:app-reflection}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccccccc}
\toprule
& late & \multicolumn{3}{c}{median characters} & \multicolumn{2}{c}{loop rate} & \multicolumn{2}{c}{reflection words} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
Run & steps & 1--5 & late & ratio & 1--5 & late & 1--5 & late \\
\midrule
\multicolumn{9}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 105--170 & 13,415 & 18,326 & 1.37 & 0.007 & 0.002 & 2.29 & 1.92 \\
\quad 4B, run 2$^\dagger$ & 105--165 & 13,198 & 18,228 & 1.38 & 0.005 & 0.003 & 2.33 & 1.91 \\
\quad 1.7B & 105--210 & 14,270 & 20,730 & 1.45 & 0.032 & 0.010 & 2.16 & 2.99 \\
\quad 0.6B, run 1 & 55--80 & 11,071 & 21,592 & 1.95 & 0.029 & 0.013 & 1.99 & 3.97 \\
\quad 0.6B, run 2$^\dagger$ & 105--210 & 11,376 & 20,260 & 1.78 & 0.051 & 0.018 & 3.21 & 3.39 \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{0.6B cold-started on short external solutions, other rollout budgets}} \\
\quad 16,384-token budget & 6--7 & 11,043 & 43,326 & 3.92 & 0.044 & 0.531 & 2.33 & 6.87 \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{Non-thinking route, pretrained-only start}} \\
\quad 4B & 105--210 & 2,218 & 4,510 & 2.03 & 0.580 & 0.115 & 0.02 & 0.10 \\
\quad 1.7B & 105--210 & 1,428 & 5,374 & 3.76 & 0.484 & 0.031 & 0.02 & 0.17 \\
\quad 0.6B & 105--210 & 1,762 & 6,766 & 3.84 & 0.379 & 0.034 & 0.03 & 0.19 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_reliability.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{Stop reliability before training, and how much closure each run keeps.} Stop reliability is
P(correct $\mid$ closed) on a run's first four steps of training rollouts, before training has moved the student
far; for the thinking teacher, on its own samples of the training problems (12,947 closed
samples). \emph{Solved and stopped}: closed and correct, as a fraction of all rollouts. \emph{Late window}:
steps 101 to the last logged step, or the last 20 logged steps for shorter runs, or steps 11--20 for the 20-step
runs. \emph{Retained closure}: late closure divided by steps 1--4 closure. Among the 7{,}168-token runs
cold-started on short external solutions, the size ordering of stop reliability (4B, then 1.7B, then 0.6B) is
also the ordering of retained closure. Rows and $\dagger$ as in Table~\ref{tab:app-windows}.}
\label{tab:app-reliability}
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccccccc}
\toprule
& logged & \multicolumn{3}{c}{steps 1--4} & \multicolumn{3}{c}{late window} & retained \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
Run & steps & closure & \makecell{stop\\reliability} & \makecell{solved and\\stopped} & steps & closure & \makecell{solved and\\stopped} & closure \\
\midrule
Teacher (thinking), own samples & -- & -- & 0.885 & -- & -- & -- & -- & -- \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 170 & 0.648 & 0.521 & 0.338 & 101--170 & 0.226 & 0.151 & 0.349 \\
\quad 4B, run 2$^\dagger$ & 167 & 0.652 & 0.509 & 0.332 & 101--167 & 0.226 & 0.153 & 0.347 \\
\quad 1.7B & 212 & 0.459 & 0.128 & 0.059 & 101--212 & 0.064 & 0.029 & 0.139 \\
\quad 0.6B, run 1 & 80 & 0.611 & 0.042 & 0.025 & 61--80 & 0.023 & 0.005 & 0.038 \\
\quad 0.6B, run 2$^\dagger$ & 212 & 0.586 & 0.033 & 0.020 & 101--212 & 0.026 & 0.005 & 0.044 \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 212 & 0.219 & 0.259 & 0.057 & 101--212 & 0.211 & 0.140 & 0.963 \\
\quad 1.7B & 142 & 0.078 & 0.025 & 0.002 & 123--142 & 0.003 & 0.000 & 0.038 \\
\quad 0.6B & 142 & 0.119 & 0.000 & 0.000 & 123--142 & 0.002 & 0.000 & 0.017 \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{Officially post-trained 0.6B, 16,384-token budget}} \\
\quad thinking template, run 1 & 20 & 0.756 & 0.349 & 0.264 & 11--20 & 0.410 & 0.270 & 0.542 \\
\quad thinking template, run 2$^\dagger$ & 20 & 0.750 & 0.362 & 0.271 & 11--20 & 0.438 & 0.287 & 0.584 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_runs.tex <==
\begin{table}[!htbp]
\centering
\footnotesize
\caption{\textbf{Every training run in the study.} Eighteen on-policy distillation runs from the same
13{,}597 training problems (the two curriculum runs use 12{,}741) and the same teacher, Qwen3-8B, in the mode
shown; the student always runs in the teacher's mode. \emph{Short-solution start}: the student after
supervised fine-tuning on 5{,}878 short external solutions; \emph{teacher-solution start}: after fine-tuning on
1{,}524 of the teacher's own correct solutions. \emph{Steps}: the last step whose training rollouts are archived,
over the planned length; two epochs are 212 steps and no run went past step 212. \emph{Evaluated}: the step
whose checkpoint was evaluated; runs marked $^\ast$ were evaluated on fewer benchmarks or samples
(Appendix~\ref{app:perbench}). Runs 1 and 2 of the same configuration are
independent reruns over the same data order: the seed label did not reach the trainer (Appendix~\ref{app:notes}). Run 2 of the officially post-trained start is also the
model of the probes in Appendix~\ref{app:probes}. No curriculum run, no 4B or 1.7B run at a budget other than
7{,}168, and no forward-divergence run exists in the thinking arm.}
\label{tab:app-runs}
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{\linewidth}{@{}lllcc>{\raggedright\arraybackslash}X@{}}
\toprule
Student start & Teacher & Budget & Steps & Evaluated & Role \\
\midrule
\multicolumn{6}{@{}l}{\textit{The three routes: every evaluated endpoint of the main study}} \\
4B pretrained-only & non-thinking & 7,168 & 212 / 212 & 212 & non-thinking route \\
1.7B pretrained-only & non-thinking & 7,168 & 212 / 212 & 212 & non-thinking route \\
0.6B pretrained-only & non-thinking & 7,168 & 212 / 212 & 212 & non-thinking route \\
4B short-solution start & thinking & 7,168 & 167 / 214 & 142 & thinking route, run 2 \\
1.7B short-solution start & thinking & 7,168 & 212 / 214 & 142 & thinking route \\
0.6B short-solution start & thinking & 7,168 & 212 / 214 & 142 & thinking route, run 2 \\
4B teacher-solution start & thinking & 7,168 & 212 / 212 & 142, 212 & thinking route \\
1.7B teacher-solution start & thinking & 7,168 & 142 / 142 & 142 & thinking route \\
0.6B teacher-solution start & thinking & 7,168 & 142 / 142 & 142 & thinking route \\
\midrule
\multicolumn{6}{@{}l}{\textit{Controls in the thinking arm}} \\
4B short-solution start & thinking & 7,168 & 170 / 214 & -- & rerun, run 1 \\
0.6B short-solution start & thinking & 7,168 & 80 / 214 & -- & rerun, run 1; stopped early \\
0.6B short-solution start & thinking & 16,384 & 7 / 40 & -- & larger rollout budget; stopped early \\
0.6B short-solution start & thinking & 1,024 & 212 / 212 & 212$^\ast$ & smaller rollout budget; one update per step \\
officially post-trained 0.6B & thinking & 16,384 & 20 / 20 & -- & post-trained start, run 1 \\
officially post-trained 0.6B & thinking & 16,384 & 20 / 20 & 20$^\ast$ & post-trained start, run 2; also probed \\
\midrule
\multicolumn{6}{@{}l}{\textit{Controls in the non-thinking arm (they say nothing about the collapse)}} \\
officially post-trained 0.6B & non-thinking & 16,384 & 20 / 20 & -- & the two runs above, non-thinking template \\
4B pretrained-only & non-thinking & 7,168 & 99 / 99 & -- & easy-to-hard curriculum \\
1.7B pretrained-only & non-thinking & 7,168 & 99 / 99 & -- & easy-to-hard curriculum \\
\bottomrule
\end{tabularx}
\end{table}



==> tables/app_sameprompt.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{Which closes are lost, on identical prompts.} The officially post-trained 0.6B before training and
after 20 steps of distillation from the thinking teacher (16{,}384-token budget, run~2) each answer the same
128 training problems four times. Problems are grouped by how many of the start model's four samples were
stopped and correct; cells are fractions of samples that close, close with a correct answer, and close with a
wrong one. Closure falls in every group. On the problems the start model never solved, the closes that
disappear are wrong ones and some correct closes appear; on the problems it solved three or four times out
of four, correct closes are lost as well.}
\label{tab:app-sameprompt}
\footnotesize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccc}
\toprule
start model solved & & \multicolumn{2}{c}{closed} & \multicolumn{2}{c}{closed and correct} & \multicolumn{2}{c}{closed and wrong} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
(of 4 samples) & problems & before & after & before & after & before & after \\
\midrule
0/4 & 68 & 0.691 & 0.243 & 0.000 & 0.085 & 0.691 & 0.158 \\
1--2/4 & 28 & 0.830 & 0.464 & 0.375 & 0.348 & 0.455 & 0.116 \\
3--4/4 & 32 & 0.992 & 0.828 & 0.891 & 0.758 & 0.102 & 0.070 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_scores.tex <==
\begingroup
\scriptsize
\setlength{\tabcolsep}{4pt}
\setlength{\LTcapwidth}{\linewidth}
\begin{longtable}{>{\raggedright\arraybackslash}p{4.1cm}ccccccccc@{}}
\caption{\textbf{Every score of every evaluated model, per benchmark.} Three scorings of the same samples,
never mixed: \emph{lenient} credits a sample if any marked answer in it is correct; \emph{committed} if the last
one is; \emph{strict} if the sample closed its reasoning (thinking mode) or stopped before the cap
(non-thinking mode) and its answer is correct. $p@1$ is the mean over samples, $p@n$ the fraction of problems
with at least one correct sample, \emph{all $n$} the fraction with every sample correct (lenient).
\emph{First answer $p@1$} scores the first marked answer written. \emph{Majority} votes over the committed
answers of the $n$ samples. The mean rows weight the three benchmarks equally. Names: \emph{short-solution
start}, the student after fine-tuning on 5{,}878 short external solutions; \emph{teacher-solution start}, after
fine-tuning on 1{,}524 of the teacher's own solutions; \emph{+ thinking route}, that start distilled from the
thinking teacher for 142 steps; \emph{non-thinking route}, the pretrained-only student distilled from the
non-thinking teacher for 212 steps. $^\dagger$\,Evaluated with fewer samples: the officially post-trained 0.6B with 16 per problem on AIME 2026 and AMC23 and 4 on GSM8K-200; that model after 20 thinking steps and the 1{,}024-token run with 4 per problem, on GSM8K-200 only.}\label{tab:app-scores}\\
\toprule
& \multicolumn{3}{c}{Lenient} & \multicolumn{2}{c}{Committed} & \multicolumn{2}{c}{Strict} & First answer & Majority \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Model & $p@1$ & $p@n$ & all $n$ & $p@1$ & $p@n$ & $p@1$ & $p@n$ & $p@1$ & maj@$n$ \\
\midrule
\endfirsthead
\multicolumn{10}{l}{\textit{Table~\ref{tab:app-scores}, continued}}\\
\toprule
& \multicolumn{3}{c}{Lenient} & \multicolumn{2}{c}{Committed} & \multicolumn{2}{c}{Strict} & First answer & Majority \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Model & $p@1$ & $p@n$ & all $n$ & $p@1$ & $p@n$ & $p@1$ & $p@n$ & $p@1$ & maj@$n$ \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{\textit{continued on the next page}}\\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{10}{@{}l}{\textbf{AIME 2026}\quad 30 problems, 48 samples each, 30{,}720-token cap} \\*
Teacher (thinking) & 0.674 & 0.900 & 0.233 & 0.669 & 0.900 & 0.667 & 0.900 & 0.671 & 0.800 \\
Teacher (non-thinking) & 0.163 & 0.667 & 0.000 & 0.163 & 0.667 & 0.163 & 0.667 & 0.156 & 0.200 \\
\addlinespace[2pt]
4B pretrained-only & 0.083 & 0.333 & 0.000 & 0.083 & 0.333 & 0.083 & 0.333 & 0.083 & 0.133 \\
4B non-thinking route & 0.141 & 0.467 & 0.067 & 0.140 & 0.467 & 0.117 & 0.400 & 0.133 & 0.167 \\
4B short-solution start & 0.148 & 0.400 & 0.000 & 0.148 & 0.400 & 0.146 & 0.400 & 0.148 & 0.233 \\
\quad + thinking route & 0.329 & 0.700 & 0.033 & 0.327 & 0.700 & 0.322 & 0.700 & 0.329 & 0.567 \\
4B teacher-solution start & 0.116 & 0.400 & 0.000 & 0.113 & 0.367 & 0.084 & 0.367 & 0.113 & 0.300 \\
\quad + thinking route & 0.316 & 0.733 & 0.100 & 0.312 & 0.733 & 0.304 & 0.733 & 0.313 & 0.567 \\
\quad + thinking route, 212 steps & 0.334 & 0.633 & 0.100 & 0.326 & 0.633 & 0.319 & 0.633 & 0.331 & 0.533 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.014 & 0.133 & 0.000 & 0.014 & 0.133 & 0.014 & 0.133 & 0.014 & 0.067 \\
1.7B non-thinking route & 0.079 & 0.300 & 0.000 & 0.078 & 0.267 & 0.078 & 0.267 & 0.074 & 0.133 \\
1.7B short-solution start & 0.029 & 0.233 & 0.000 & 0.028 & 0.200 & 0.026 & 0.200 & 0.028 & 0.100 \\
\quad + thinking route & 0.057 & 0.200 & 0.000 & 0.053 & 0.167 & 0.051 & 0.167 & 0.056 & 0.133 \\
1.7B teacher-solution start & 0.013 & 0.100 & 0.000 & 0.013 & 0.100 & 0.008 & 0.100 & 0.011 & 0.100 \\
\quad + thinking route & 0.067 & 0.233 & 0.000 & 0.031 & 0.200 & 0.000 & 0.000 & 0.066 & 0.200 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.004 & 0.167 & 0.000 & 0.002 & 0.067 & 0.002 & 0.067 & 0.002 & 0.033 \\
0.6B non-thinking route & 0.018 & 0.133 & 0.000 & 0.017 & 0.133 & 0.017 & 0.133 & 0.014 & 0.067 \\
0.6B short-solution start & 0.006 & 0.167 & 0.000 & 0.004 & 0.100 & 0.004 & 0.100 & 0.005 & 0.000 \\
\quad + thinking route & 0.004 & 0.067 & 0.000 & 0.002 & 0.067 & 0.001 & 0.033 & 0.004 & 0.000 \\
0.6B teacher-solution start & 0.001 & 0.033 & 0.000 & 0.001 & 0.033 & 0.001 & 0.033 & 0.001 & 0.000 \\
\quad + thinking route & 0.003 & 0.067 & 0.000 & 0.002 & 0.067 & 0.000 & 0.000 & 0.003 & 0.000 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 0.117 & 0.300 & 0.000 & 0.110 & 0.267 & 0.110 & 0.267 & 0.115 & 0.233 \\
\midrule
\multicolumn{10}{@{}l}{\textbf{AMC23}\quad 40 problems, 48 samples each, 30{,}720-token cap} \\*
Teacher (thinking) & 0.960 & 1.000 & 0.775 & 0.958 & 1.000 & 0.955 & 1.000 & 0.958 & 0.975 \\
Teacher (non-thinking) & 0.694 & 0.975 & 0.325 & 0.692 & 0.975 & 0.692 & 0.975 & 0.633 & 0.825 \\
\addlinespace[2pt]
4B pretrained-only & 0.438 & 0.900 & 0.000 & 0.436 & 0.900 & 0.436 & 0.900 & 0.436 & 0.600 \\
4B non-thinking route & 0.587 & 0.925 & 0.225 & 0.585 & 0.925 & 0.486 & 0.900 & 0.509 & 0.700 \\
4B short-solution start & 0.548 & 0.925 & 0.150 & 0.547 & 0.925 & 0.543 & 0.925 & 0.546 & 0.800 \\
\quad + thinking route & 0.728 & 0.900 & 0.350 & 0.727 & 0.900 & 0.721 & 0.900 & 0.726 & 0.875 \\
4B teacher-solution start & 0.412 & 0.900 & 0.000 & 0.410 & 0.900 & 0.285 & 0.875 & 0.409 & 0.825 \\
\quad + thinking route & 0.728 & 0.950 & 0.375 & 0.726 & 0.950 & 0.719 & 0.925 & 0.727 & 0.900 \\
\quad + thinking route, 212 steps & 0.766 & 0.975 & 0.350 & 0.756 & 0.975 & 0.750 & 0.975 & 0.764 & 0.925 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.266 & 0.825 & 0.000 & 0.266 & 0.825 & 0.266 & 0.825 & 0.265 & 0.500 \\
1.7B non-thinking route & 0.410 & 0.900 & 0.125 & 0.406 & 0.900 & 0.403 & 0.900 & 0.365 & 0.550 \\
1.7B short-solution start & 0.299 & 0.775 & 0.025 & 0.296 & 0.775 & 0.287 & 0.775 & 0.294 & 0.500 \\
\quad + thinking route & 0.362 & 0.725 & 0.100 & 0.350 & 0.700 & 0.330 & 0.650 & 0.356 & 0.525 \\
1.7B teacher-solution start & 0.129 & 0.550 & 0.000 & 0.123 & 0.550 & 0.065 & 0.475 & 0.126 & 0.500 \\
\quad + thinking route & 0.372 & 0.675 & 0.100 & 0.180 & 0.650 & 0.000 & 0.000 & 0.366 & 0.575 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.053 & 0.625 & 0.000 & 0.052 & 0.575 & 0.051 & 0.575 & 0.051 & 0.375 \\
0.6B non-thinking route & 0.278 & 0.700 & 0.000 & 0.276 & 0.700 & 0.275 & 0.700 & 0.231 & 0.475 \\
0.6B short-solution start & 0.173 & 0.675 & 0.000 & 0.165 & 0.675 & 0.147 & 0.675 & 0.152 & 0.400 \\
\quad + thinking route & 0.212 & 0.600 & 0.000 & 0.189 & 0.575 & 0.149 & 0.475 & 0.196 & 0.375 \\
0.6B teacher-solution start & 0.029 & 0.400 & 0.000 & 0.024 & 0.375 & 0.017 & 0.350 & 0.026 & 0.250 \\
\quad + thinking route & 0.165 & 0.475 & 0.000 & 0.126 & 0.450 & 0.000 & 0.000 & 0.147 & 0.400 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 0.505 & 0.900 & 0.100 & 0.491 & 0.900 & 0.491 & 0.900 & 0.492 & 0.675 \\
\midrule
\multicolumn{10}{@{}l}{\textbf{GSM8K-200}\quad 200 problems, 32 samples each, 8{,}192-token cap} \\*
Teacher (thinking) & 0.937 & 0.965 & 0.875 & 0.935 & 0.960 & 0.934 & 0.960 & 0.933 & 0.940 \\
Teacher (non-thinking) & 0.929 & 0.965 & 0.825 & 0.928 & 0.965 & 0.928 & 0.965 & 0.924 & 0.940 \\
\addlinespace[2pt]
4B pretrained-only & 0.761 & 0.975 & 0.065 & 0.759 & 0.975 & 0.758 & 0.975 & 0.755 & 0.925 \\
4B non-thinking route & 0.919 & 0.980 & 0.770 & 0.917 & 0.980 & 0.913 & 0.980 & 0.903 & 0.930 \\
4B short-solution start & 0.899 & 0.980 & 0.655 & 0.899 & 0.980 & 0.899 & 0.980 & 0.898 & 0.935 \\
\quad + thinking route & 0.896 & 0.965 & 0.640 & 0.896 & 0.965 & 0.891 & 0.965 & 0.894 & 0.935 \\
4B teacher-solution start & 0.461 & 0.945 & 0.000 & 0.460 & 0.945 & 0.312 & 0.925 & 0.460 & 0.910 \\
\quad + thinking route & 0.903 & 0.965 & 0.780 & 0.889 & 0.965 & 0.884 & 0.965 & 0.901 & 0.935 \\
\quad + thinking route, 212 steps & 0.914 & 0.965 & 0.805 & 0.856 & 0.965 & 0.852 & 0.965 & 0.912 & 0.940 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.601 & 0.980 & 0.010 & 0.598 & 0.980 & 0.601 & 0.980 & 0.597 & 0.875 \\
1.7B non-thinking route & 0.830 & 0.975 & 0.520 & 0.830 & 0.975 & 0.830 & 0.975 & 0.804 & 0.875 \\
1.7B short-solution start & 0.747 & 0.985 & 0.170 & 0.737 & 0.985 & 0.705 & 0.985 & 0.732 & 0.905 \\
\quad + thinking route & 0.757 & 0.960 & 0.250 & 0.756 & 0.960 & 0.734 & 0.960 & 0.754 & 0.875 \\
1.7B teacher-solution start & 0.243 & 0.900 & 0.000 & 0.237 & 0.895 & 0.126 & 0.825 & 0.239 & 0.850 \\
\quad + thinking route & 0.743 & 0.950 & 0.180 & 0.551 & 0.950 & 0.000 & 0.000 & 0.737 & 0.870 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.087 & 0.745 & 0.000 & 0.086 & 0.730 & 0.086 & 0.730 & 0.083 & 0.625 \\
0.6B non-thinking route & 0.689 & 0.945 & 0.350 & 0.688 & 0.945 & 0.687 & 0.945 & 0.670 & 0.805 \\
0.6B short-solution start & 0.536 & 0.930 & 0.015 & 0.525 & 0.925 & 0.450 & 0.910 & 0.503 & 0.800 \\
\quad + thinking route & 0.667 & 0.895 & 0.220 & 0.651 & 0.895 & 0.602 & 0.885 & 0.658 & 0.820 \\
0.6B teacher-solution start & 0.135 & 0.765 & 0.000 & 0.126 & 0.760 & 0.075 & 0.720 & 0.131 & 0.710 \\
\quad + thinking route & 0.620 & 0.880 & 0.160 & 0.546 & 0.875 & 0.000 & 0.000 & 0.616 & 0.800 \\
\addlinespace[2pt]
0.6B short-solution start, 1{,}024-token budget$^\dagger$ & 0.554 & 0.760 & 0.300 & 0.539 & 0.760 & 0.226 & 0.495 & 0.535 & 0.735 \\
officially post-trained 0.6B$^\dagger$ & 0.777 & 0.890 & 0.640 & 0.771 & 0.890 & 0.769 & 0.890 & 0.767 & 0.825 \\
\quad + 20 thinking steps (16{,}384)$^\dagger$ & 0.757 & 0.860 & 0.660 & 0.755 & 0.855 & 0.749 & 0.850 & 0.754 & 0.805 \\
\midrule
\multicolumn{10}{@{}l}{\textbf{Mean of the three}\quad unweighted mean over AIME 2026, AMC23 and GSM8K-200} \\*
Teacher (thinking) & 0.857 & 0.955 & 0.628 & 0.854 & 0.953 & 0.852 & 0.953 & 0.854 & 0.905 \\
Teacher (non-thinking) & 0.595 & 0.869 & 0.383 & 0.594 & 0.869 & 0.594 & 0.869 & 0.571 & 0.655 \\
\addlinespace[2pt]
4B pretrained-only & 0.427 & 0.736 & 0.022 & 0.426 & 0.736 & 0.426 & 0.736 & 0.425 & 0.553 \\
4B non-thinking route & 0.549 & 0.791 & 0.354 & 0.547 & 0.791 & 0.505 & 0.760 & 0.515 & 0.599 \\
4B short-solution start & 0.532 & 0.768 & 0.268 & 0.531 & 0.768 & 0.529 & 0.768 & 0.531 & 0.656 \\
\quad + thinking route & 0.651 & 0.855 & 0.341 & 0.650 & 0.855 & 0.645 & 0.855 & 0.649 & 0.792 \\
4B teacher-solution start & 0.330 & 0.748 & 0.000 & 0.328 & 0.737 & 0.227 & 0.722 & 0.327 & 0.678 \\
\quad + thinking route & 0.649 & 0.883 & 0.418 & 0.643 & 0.883 & 0.636 & 0.874 & 0.647 & 0.801 \\
\quad + thinking route, 212 steps & 0.671 & 0.858 & 0.418 & 0.646 & 0.858 & 0.640 & 0.858 & 0.669 & 0.799 \\
\addlinespace[2pt]
1.7B pretrained-only & 0.294 & 0.646 & 0.003 & 0.293 & 0.646 & 0.294 & 0.646 & 0.292 & 0.481 \\
1.7B non-thinking route & 0.440 & 0.725 & 0.215 & 0.438 & 0.714 & 0.437 & 0.714 & 0.414 & 0.519 \\
1.7B short-solution start & 0.358 & 0.664 & 0.065 & 0.353 & 0.653 & 0.339 & 0.653 & 0.351 & 0.502 \\
\quad + thinking route & 0.392 & 0.628 & 0.117 & 0.387 & 0.609 & 0.372 & 0.592 & 0.388 & 0.511 \\
1.7B teacher-solution start & 0.128 & 0.517 & 0.000 & 0.124 & 0.515 & 0.066 & 0.467 & 0.125 & 0.483 \\
\quad + thinking route & 0.394 & 0.619 & 0.093 & 0.254 & 0.600 & 0.000 & 0.000 & 0.390 & 0.548 \\
\addlinespace[2pt]
0.6B pretrained-only & 0.048 & 0.512 & 0.000 & 0.047 & 0.457 & 0.046 & 0.457 & 0.045 & 0.344 \\
0.6B non-thinking route & 0.328 & 0.593 & 0.117 & 0.327 & 0.593 & 0.327 & 0.593 & 0.305 & 0.449 \\
0.6B short-solution start & 0.238 & 0.591 & 0.005 & 0.232 & 0.567 & 0.201 & 0.562 & 0.220 & 0.400 \\
\quad + thinking route & 0.294 & 0.521 & 0.073 & 0.281 & 0.512 & 0.251 & 0.464 & 0.286 & 0.398 \\
0.6B teacher-solution start & 0.055 & 0.399 & 0.000 & 0.050 & 0.389 & 0.031 & 0.368 & 0.053 & 0.320 \\
\quad + thinking route & 0.262 & 0.474 & 0.053 & 0.225 & 0.464 & 0.000 & 0.000 & 0.256 & 0.400 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 0.466 & 0.697 & 0.247 & 0.457 & 0.686 & 0.457 & 0.686 & 0.458 & 0.578 \\
\end{longtable}
\endgroup



==> tables/app_signal.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{The teacher's stop signal on each student's own first-step rollouts: high where the student stopped,
near zero along truncated trajectories, and a per-token advantage that is flat along the rollout.} The teacher
scores every token of about 120 rollouts per student from the first training step (7{,}168-token rollout
budget), where the student's log-probabilities are reproduced exactly by the initial model. The advantage is
$\mathrm{clip}(\log\pi_{\text{teacher}} - \log\pi_{\text{student}}, -1, 1)$ on the sampled token;
$p_{\text{stop}}$ and $q_{\text{stop}}$ are the teacher's and the student's probability of \think{} (for the
non-thinking row, of the end-of-turn tokens). (a)~Samples that stopped: the probabilities and the advantage at
the stop. (b)~Samples truncated at the budget: the fraction in which the teacher's $p_{\text{stop}}$ exceeds
0.5 or 0.1 at any position; the median over samples of its maximum; at positions where it exceeds 0.5, the mean
advantage of the token the student wrote instead and the student's own $q_{\text{stop}}$. \emph{Length
aligned}: the fraction of truncated samples whose re-encoded length equals the budget (rollouts were stored as
text and re-tokenized). (c)~All tokens: mean advantage and the fraction clipped at each end; reflection tokens
are \emph{Wait}, \emph{Hmm}, \emph{Actually} and two Chinese equivalents. (d)~Mean advantage by position decile.
Rows 4B, 1.7B and 0.6B are the students cold-started on short external solutions (run~1 at 4B, run~2 at
0.6B), distilled from the thinking teacher; the last row is the pretrained-only 0.6B under the non-thinking
teacher.}
\label{tab:app-signal}
\scriptsize
\setlength{\tabcolsep}{3.5pt}
{\small (a) Samples that stopped}\par\smallskip
\begin{tabular}{lccccccc}
\toprule
& rollouts & & \multicolumn{5}{c}{samples that stopped} \\
\cmidrule(lr){4-8}
& probed & excluded & $n$ & teacher $p_{\text{stop}}$ & student $q_{\text{stop}}$ & advantage & fraction $>0$ \\
Student & & & & at the stop & at the stop & on the stop token & \\
\midrule
4B & 126 & 2 & 83 & 0.976 & 0.928 & $+0.027$ & 0.976 \\
1.7B & 117 & 11 & 57 & 0.764 & 0.590 & $+0.032$ & 0.754 \\
0.6B & 122 & 6 & 75 & 0.673 & 0.529 & $-0.062$ & 0.680 \\
0.6B, non-thinking & 128 & 0 & 127 & 0.246 & 0.298 & $-1.000$ & 0.000 \\
\bottomrule
\end{tabular}
\par\medskip
{\small (b) Samples truncated at the rollout budget}\par\smallskip
\begin{tabular}{lccccccc}
\toprule
& & length & \multicolumn{2}{c}{teacher $p_{\text{stop}}$ ever} & median of the & \multicolumn{2}{c}{where teacher $p_{\text{stop}}>0.5$} \\
\cmidrule(lr){4-5}\cmidrule(lr){7-8}
Student & $n$ & aligned & $>0.5$ & $>0.1$ & teacher's max $p_{\text{stop}}$ & advantage & student $q_{\text{stop}}$ \\
\midrule
4B & 36 & 0.917 & 0.000 & 0.000 & $4.4\times 10^{-9}$ & -- & -- \\
1.7B & 40 & 0.650 & 0.100 & 0.175 & $5.8\times 10^{-8}$ & $-0.900$ & 0.273 \\
0.6B & 23 & 0.348 & 0.043 & 0.043 & $1.0\times 10^{-7}$ & $-1.000$ & 0.294 \\
0.6B, non-thinking & 1 & 1.000 & 0.000 & 0.000 & $1.6\times 10^{-3}$ & -- & -- \\
\bottomrule
\end{tabular}
\par\medskip
{\small (c) Per-token advantage over whole rollouts}\par\smallskip
\begin{tabular}{lccccccc}
\toprule
& \multicolumn{4}{c}{all tokens} & \multicolumn{3}{c}{reflection tokens} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-8}
Student & tokens & mean advantage & at $+1$ & at $-1$ & tokens & mean advantage & fraction $>0$ \\
\midrule
4B & 591,459 & $-0.133$ & 0.019 & 0.133 & 3,054 & $-0.067$ & 0.521 \\
1.7B & 598,106 & $-0.201$ & 0.027 & 0.209 & 2,983 & $+0.016$ & 0.529 \\
0.6B & 524,976 & $-0.229$ & 0.029 & 0.231 & 5,548 & $+0.030$ & 0.652 \\
0.6B, non-thinking & 223,786 & $-0.310$ & 0.044 & 0.299 & 37 & $-0.364$ & 0.108 \\
\bottomrule
\end{tabular}
\par\medskip
{\small (d) Mean advantage by relative position}\par\smallskip
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{10}{c}{decile of the rollout (position / length)} \\
\cmidrule(lr){2-11}
Student & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
4B & $-0.114$ & $-0.128$ & $-0.131$ & $-0.130$ & $-0.140$ & $-0.141$ & $-0.141$ & $-0.138$ & $-0.136$ & $-0.132$ \\
1.7B & $-0.161$ & $-0.196$ & $-0.200$ & $-0.208$ & $-0.215$ & $-0.217$ & $-0.208$ & $-0.215$ & $-0.203$ & $-0.189$ \\
0.6B & $-0.219$ & $-0.247$ & $-0.250$ & $-0.246$ & $-0.241$ & $-0.240$ & $-0.227$ & $-0.218$ & $-0.204$ & $-0.197$ \\
0.6B, non-thinking & $-0.345$ & $-0.307$ & $-0.301$ & $-0.307$ & $-0.322$ & $-0.307$ & $-0.303$ & $-0.302$ & $-0.308$ & $-0.302$ \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_steps.tex <==
\begin{table}[p]
\centering
\caption{\textbf{The first 30 training steps of every run (the data behind Figure~\ref{fig:collapse}).} Means over
step windows of the student's own training rollouts. \emph{Finished}: the closure rate for thinking runs; for
non-thinking runs, the fraction of rollouts that stop before the rollout budget. \emph{Length}: median
response tokens divided by the rollout budget. \emph{Stop precision}: P(correct $\mid$ closed), thinking runs
only. \emph{Answer rate}: the fraction of rollouts that contain a marked answer (a
\texttt{\textbackslash boxed\{\}} or an \emph{Answer:} line). \emph{First-answer position}: mean position of
the first \texttt{\textbackslash boxed\{\}} as a fraction of the rollout's characters, among rollouts that
contain one, with their number in the window in parentheses. Once the median length reaches the budget, the
denominator is the budget itself, so a falling position can be produced by lengthening alone; it is not a
trend to read on its own. Dashes mark windows a run did not reach and runs whose rollouts were not
re-tokenized for length. Rows and $\dagger$ as in Table~\ref{tab:app-windows}.}
\label{tab:app-steps}
\scriptsize
\setlength{\tabcolsep}{3pt}
{\small (a) Finished, length and stop precision}\par\smallskip
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{4}{c}{finished} & \multicolumn{4}{c}{length (median / budget)} & \multicolumn{4}{c}{stop precision} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Run & 1--5 & 6--10 & 11--20 & 21--30 & 1--5 & 6--10 & 11--20 & 21--30 & 1--5 & 6--10 & 11--20 & 21--30 \\
\midrule
\multicolumn{13}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 0.617 & 0.211 & 0.155 & 0.189 & 0.747 & 1.000 & 1.000 & 1.000 & 0.527 & 0.656 & 0.654 & 0.634 \\
\quad 4B, run 2$^\dagger$ & 0.633 & 0.208 & 0.170 & 0.212 & 0.698 & 1.000 & 1.000 & 1.000 & 0.508 & 0.636 & 0.587 & 0.698 \\
\quad 1.7B & 0.445 & 0.128 & 0.071 & 0.051 & 0.737 & 1.000 & 1.000 & 1.000 & 0.121 & 0.198 & 0.146 & 0.256 \\
\quad 0.6B, run 1 & 0.605 & 0.145 & 0.058 & 0.042 & -- & -- & -- & -- & 0.039 & 0.035 & 0.039 & 0.000 \\
\quad 0.6B, run 2$^\dagger$ & 0.583 & 0.113 & 0.055 & 0.052 & 0.558 & 1.000 & 1.000 & 1.000 & 0.033 & 0.032 & 0.011 & 0.000 \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 0.225 & 0.231 & 0.145 & 0.148 & 1.000 & 1.000 & 1.000 & 1.000 & 0.222 & 0.278 & 0.397 & 0.473 \\
\quad 1.7B & 0.078 & 0.033 & 0.039 & 0.023 & 1.000 & 1.000 & 1.000 & 1.000 & 0.018 & 0.000 & 0.085 & 0.183 \\
\quad 0.6B & 0.117 & 0.070 & 0.032 & 0.055 & 1.000 & 1.000 & 1.000 & 1.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{0.6B cold-started on short external solutions, other rollout budgets}} \\
\quad 1,024-token budget & 0.125 & 0.105 & 0.080 & 0.064 & 1.000 & 1.000 & 1.000 & 1.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\quad 16,384-token budget & 0.608 & 0.297 & -- & -- & 0.232 & 0.795 & -- & -- & 0.041 & 0.036 & -- & -- \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Officially post-trained 0.6B, 16,384-token budget}} \\
\quad thinking template, run 1 & 0.736 & 0.372 & 0.410 & -- & 0.747 & 1.000 & 1.000 & -- & 0.344 & 0.672 & 0.658 & -- \\
\quad thinking template, run 2$^\dagger$ & 0.731 & 0.366 & 0.438 & -- & 0.745 & 1.000 & 1.000 & -- & 0.375 & 0.703 & 0.657 & -- \\
\quad non-thinking template & 1.000 & 1.000 & 0.999 & -- & 0.057 & 0.140 & 0.154 & -- & -- & -- & -- & -- \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Non-thinking route, pretrained-only start}} \\
\quad 4B & 0.923 & 0.931 & 0.955 & 0.980 & 0.122 & 0.146 & 0.258 & 0.262 & -- & -- & -- & -- \\
\quad 1.7B & 0.964 & 0.955 & 0.948 & 0.970 & 0.072 & 0.098 & 0.236 & 0.301 & -- & -- & -- & -- \\
\quad 0.6B & 0.983 & 0.963 & 0.930 & 0.978 & 0.107 & 0.116 & 0.237 & 0.338 & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
\par\medskip
{\small (b) Answer rate and first-answer position}\par\smallskip
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{4}{c}{answer rate} & \multicolumn{4}{c}{first-answer position (rollouts with an answer)} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
Run & 1--5 & 6--10 & 11--20 & 21--30 & 1--5 & 6--10 & 11--20 & 21--30 \\
\midrule
\multicolumn{9}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 0.689 & 0.266 & 0.197 & 0.237 & 0.80 (441) & 0.74 (164) & 0.73 (241) & 0.71 (297) \\
\quad 4B, run 2$^\dagger$ & 0.714 & 0.267 & 0.208 & 0.243 & 0.80 (453) & 0.74 (164) & 0.72 (263) & 0.72 (307) \\
\quad 1.7B & 0.694 & 0.198 & 0.064 & 0.087 & 0.79 (435) & 0.66 (118) & 0.49 (67) & 0.57 (97) \\
\quad 0.6B, run 1 & 0.814 & 0.134 & 0.055 & 0.042 & 0.77 (515) & 0.60 (83) & 0.39 (60) & 0.33 (51) \\
\quad 0.6B, run 2$^\dagger$ & 0.809 & 0.138 & 0.041 & 0.040 & 0.78 (517) & 0.65 (84) & 0.42 (47) & 0.23 (44) \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 0.222 & 0.186 & 0.233 & 0.232 & 0.77 (141) & 0.73 (114) & 0.71 (291) & 0.71 (291) \\
\quad 1.7B & 0.423 & 0.417 & 0.220 & 0.174 & 0.51 (270) & 0.51 (264) & 0.70 (270) & 0.78 (215) \\
\quad 0.6B & 0.372 & 0.277 & 0.238 & 0.158 & 0.55 (234) & 0.47 (171) & 0.63 (299) & 0.72 (197) \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{0.6B cold-started on short external solutions, other rollout budgets}} \\
\quad 1,024-token budget & 0.080 & 0.061 & 0.039 & 0.022 & 0.74 (47) & 0.65 (37) & 0.52 (49) & 0.53 (27) \\
\quad 16,384-token budget & 0.845 & 0.398 & -- & -- & 0.77 (539) & 0.70 (98) & -- & -- \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{Officially post-trained 0.6B, 16,384-token budget}} \\
\quad thinking template, run 1 & 0.748 & 0.400 & 0.431 & -- & 0.86 (475) & 0.83 (250) & 0.82 (549) & -- \\
\quad thinking template, run 2$^\dagger$ & 0.745 & 0.389 & 0.459 & -- & 0.87 (474) & 0.85 (244) & 0.83 (581) & -- \\
\quad non-thinking template & 1.000 & 1.000 & 1.000 & -- & 0.96 (640) & 0.94 (640) & 0.91 (1,280) & -- \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{Non-thinking route, pretrained-only start}} \\
\quad 4B & 0.495 & 0.794 & 0.961 & 0.985 & 0.87 (314) & 0.91 (507) & 0.91 (1,230) & 0.92 (1,258) \\
\quad 1.7B & 0.311 & 0.516 & 0.934 & 0.980 & 0.86 (190) & 0.88 (325) & 0.92 (1,191) & 0.88 (1,251) \\
\quad 0.6B & 0.292 & 0.453 & 0.898 & 0.984 & 0.84 (177) & 0.83 (281) & 0.88 (1,140) & 0.88 (1,259) \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_stoplogit.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{On identical prefixes, 20 thinking steps leave the stop token where it was.} The officially post-trained
0.6B before and after 20 steps of distillation from the thinking teacher (16{,}384-token budget, run~2) read
exactly the same prefixes, cut from the start model's own outputs on the same prompts, and we compare the
log-probability each assigns to \think{} as the next token. The two prefix sets are disjoint (cut from the start
model's first two and last two samples per prompt). Positions: where the
start model actually closed its reasoning; just after the first marked answer written inside the reasoning,
split by whether that answer is correct; and at token 500. $\Delta$ is after minus before, with a 95\%
bootstrap interval; rank 0 means \think{} is the most likely next token. Where the start model closes, \think{}
is the most likely token in both models; everywhere else it lies tens of thousands of ranks deep in both, so
the changes there move a probability that is negligible in both models.}
\label{tab:app-stoplogit}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lcccccc}
\toprule
& & \multicolumn{2}{c}{$\log p(\think)$} & \multicolumn{2}{c}{change (nats)} & median rank \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Position in the prefix & $n$ & before & after & $\Delta$ & 95\% CI & before\,$\to$\,after \\
\midrule
\multicolumn{7}{l}{\textit{Prefix set 1 (667 prefixes)}} \\
\quad where the start model closed & 205 & $-0.000$ & $-0.001$ & $-0.001$ & [$-0.003$, $-0.000$] & 0\,$\to$\,0 \\
\quad just after a correct answer & 71 & $-25.865$ & $-27.235$ & $-1.370$ & [$-1.591$, $-1.157$] & 64,401\,$\to$\,67,323 \\
\quad just after a wrong answer & 135 & $-23.113$ & $-24.032$ & $-0.919$ & [$-1.089$, $-0.753$] & 48,935\,$\to$\,38,821 \\
\quad at token 500 & 256 & $-31.530$ & $-36.190$ & $-4.660$ & [$-4.953$, $-4.360$] & 79,233\,$\to$\,80,691 \\
\addlinespace[3pt]
\multicolumn{7}{l}{\textit{Prefix set 2 (663 prefixes)}} \\
\quad where the start model closed & 203 & $-0.000$ & $-0.001$ & $-0.000$ & [$-0.000$, $-0.000$] & 0\,$\to$\,0 \\
\quad just after a correct answer & 86 & $-25.913$ & $-27.273$ & $-1.360$ & [$-1.572$, $-1.158$] & 63,738\,$\to$\,65,571 \\
\quad just after a wrong answer & 118 & $-24.355$ & $-25.397$ & $-1.042$ & [$-1.220$, $-0.869$] & 53,955\,$\to$\,43,624 \\
\quad at token 500 & 256 & $-31.874$ & $-36.346$ & $-4.472$ & [$-4.754$, $-4.197$] & 77,146\,$\to$\,77,038 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_teacher.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{Inside the 7{,}168-token rollout budget, the thinking teacher finishes about a third of its samples
and the non-thinking teacher almost all of them.} (a)~The teacher in both modes on 5{,}000 training problems,
four samples each, generated with a 12{,}288-token cap (so the thinking mode's 90th percentile sits at the cap).
\emph{Stops within budget}: the sample ends on its own (in thinking mode, after closing its reasoning) within
7{,}168 tokens. \emph{Correct $\mid$ stop in budget}: accuracy among those samples. \emph{Stops and correct}:
both, as a fraction of all samples. \emph{Strict at 12{,}288}: stopped and correct at the full generation cap.
(b)~A problem counts as solved by a mode if at least one of its four samples is stopped and correct; the last
column is the Pearson correlation across problems of the two modes' per-problem accuracy. (c)~How the students'
stops line up with the teacher's, problem by problem, on the students' own training rollouts in the first 20 and
the last 20 logged steps. A student stops when it closes its reasoning (thinking) or ends before the budget
(non-thinking); $r$ is the Pearson correlation across problems between the student's stop rate and the
teacher's rate of stopping within the budget, in each teacher mode.}
\label{tab:app-teacher}
\scriptsize
\setlength{\tabcolsep}{4pt}
{\small (a) The teacher against the rollout budget}\par\smallskip
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{3}{c}{length (tokens)} & over & stops within & correct $\mid$ & stops and & strict \\
\cmidrule(lr){2-4}
Teacher mode & mean & median & p90 & budget & budget & stop in budget & correct & at 12{,}288 \\
\midrule
thinking & 9,105 & 9,630 & 12,288 & 0.685 & 0.315 & 0.885 & 0.278 & 0.573 \\
non-thinking & 2,432 & 1,592 & 4,783 & 0.061 & 0.939 & 0.500 & 0.470 & 0.473 \\
\bottomrule
\end{tabular}
\par\medskip
{\small (b) Which training problems each teacher mode solves}\par\smallskip
\begin{tabular}{ccccc}
\toprule
thinking only & non-thinking only & both & neither & correlation of per-problem accuracy \\
\midrule
0.105 & 0.088 & 0.581 & 0.226 & 0.639 \\
\bottomrule
\end{tabular}
\par\medskip
{\small (c) Per-problem agreement of the students' stops with the teacher's}\par\smallskip
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{4}{c}{first 20 steps} & \multicolumn{4}{c}{last 20 logged steps} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
& & stop & \multicolumn{2}{c}{$r$ with the teacher} & & stop & \multicolumn{2}{c}{$r$ with the teacher} \\
\cmidrule(lr){4-5}\cmidrule(lr){8-9}
Student run & steps & rate & thinking & non-thinking & steps & rate & thinking & non-thinking \\
\midrule
4B, short-solution start, run 1 & 1--20 & 0.285 & 0.372 & 0.126 & 151--170 & 0.233 & 0.662 & 0.115 \\
1.7B, short-solution start & 1--20 & 0.186 & 0.076 & 0.021 & 193--212 & 0.075 & 0.373 & 0.059 \\
0.6B, short-solution start, run 2 & 1--20 & 0.205 & $-0.022$ & $-0.049$ & 193--212 & 0.027 & 0.136 & 0.037 \\
\addlinespace[3pt]
4B, non-thinking route & 1--20 & 0.948 & 0.046 & 0.054 & 193--212 & 0.877 & 0.116 & 0.140 \\
1.7B, non-thinking route & 1--20 & 0.957 & 0.037 & 0.136 & 193--212 & 0.966 & 0.088 & 0.170 \\
0.6B, non-thinking route & 1--20 & 0.954 & $-0.013$ & $-0.025$ & 193--212 & 0.979 & $-0.017$ & 0.124 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_unfinished.tex <==
\begin{table}[p]
\centering
\caption{\textbf{What the truncated evaluation samples of every thinking-mode model contain, per benchmark.} Samples that
reached the evaluation cap. \emph{With a marked answer}: the share of them that contain a
\texttt{\textbackslash boxed\{\}} or an \emph{Answer:} line. \emph{Eligible}: truncated samples on problems whose
answer is an integer of at least three digits that does not occur in the statement; \emph{present}: the share of
those in which the correct value occurs anywhere in the text, marked or not (a diagnostic, not a score);
\emph{chance}: the same test with the answer of a random other eligible problem; \emph{first at}: median position of
its first occurrence as a fraction of the text; \emph{characters after it}: median characters written after that.
\emph{Loop}: a non-empty line repeated at least five times in the last 2{,}000 characters (the rule of
Table~\ref{tab:app-unfinished-train}). \emph{Wait/Hmm}: occurrences per 1{,}000 characters. Dashes: no eligible sample, or
none with the value present. Eligible problems: 22 of 30 on AIME 2026, 6 of 40 on AMC23, 59 of 200 on GSM8K-200, so the
AMC23 shares rest on few problems.
$^\dagger$\,Fewer samples: the officially post-trained 0.6B with 16 per problem on AIME 2026 and AMC23 and 4 on GSM8K-200; that model after 20 thinking steps and the 1{,}024-token run with 4 per problem, on GSM8K-200 only.}
\label{tab:app-unfinished-bench}
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
& \multicolumn{2}{c}{truncated samples} & \multicolumn{5}{c}{is the correct value in the text?} & & \\
\cmidrule(lr){2-3}\cmidrule(lr){4-8}
Model & $n$ & \makecell{with a\\marked answer} & eligible & present & chance & \makecell{first\\at} & \makecell{characters\\after it} & loop & \makecell{\emph{Wait}/\emph{Hmm}\\per 1{,}000} \\
\midrule
\multicolumn{10}{@{}l}{\textbf{AIME 2026}\quad 30 problems, 30{,}720-token cap} \\*
Teacher (thinking) & 154 & 0.143 & 143 & 0.147 & 0.070 & 0.62 & 25,563 & 0.058 & 1.61 \\
\addlinespace[2pt]
4B short-solution start & 786 & 0.017 & 629 & 0.041 & 0.022 & 0.14 & 49,153 & 0.089 & 2.33 \\
\quad + thinking route & 798 & 0.034 & 666 & 0.141 & 0.051 & 0.47 & 44,987 & 0.060 & 2.08 \\
4B teacher-solution start & 1,087 & 0.019 & 824 & 0.084 & 0.021 & 0.12 & 75,728 & 0.147 & 4.45 \\
\quad + thinking route & 802 & 0.047 & 661 & 0.188 & 0.039 & 0.50 & 36,612 & 0.050 & 1.98 \\
\quad + thinking route, 212 steps & 764 & 0.050 & 645 & 0.178 & 0.056 & 0.60 & 33,747 & 0.047 & 1.63 \\
\addlinespace[2pt]
1.7B short-solution start & 950 & 0.030 & 738 & 0.037 & 0.024 & 0.13 & 41,361 & 0.130 & 2.69 \\
\quad + thinking route & 1,242 & 0.024 & 938 & 0.137 & 0.036 & 0.46 & 38,830 & 0.179 & 2.74 \\
1.7B teacher-solution start & 1,181 & 0.023 & 859 & 0.055 & 0.011 & 0.08 & 66,984 & 0.212 & 3.68 \\
\quad + thinking route & 1,440 & 0.139 & 1,056 & 0.179 & 0.025 & 0.19 & 61,362 & 0.267 & 2.48 \\
\addlinespace[2pt]
0.6B short-solution start & 806 & 0.133 & 629 & 0.029 & 0.029 & 0.12 & 31,115 & 0.172 & 2.09 \\
\quad + thinking route & 1,273 & 0.037 & 931 & 0.044 & 0.016 & 0.56 & 30,594 & 0.306 & 2.39 \\
0.6B teacher-solution start & 1,222 & 0.016 & 900 & 0.022 & 0.020 & 0.13 & 41,544 & 0.170 & 3.50 \\
\quad + thinking route & 1,440 & 0.067 & 1,056 & 0.050 & 0.021 & 0.28 & 54,944 & 0.312 & 2.08 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 30 & 0.233 & 30 & 0.100 & 0.100 & 0.67 & 21,699 & 0.267 & 4.73 \\
\midrule
\multicolumn{10}{@{}l}{\textbf{AMC23}\quad 40 problems, 30{,}720-token cap} \\*
Teacher (thinking) & 36 & 0.250 & 1 & 0.000 & 0.000 & -- & -- & 0.111 & 4.34 \\
\addlinespace[2pt]
4B short-solution start & 484 & 0.041 & 32 & 0.188 & 0.031 & 0.06 & 74,636 & 0.163 & 2.61 \\
\quad + thinking route & 460 & 0.039 & 61 & 0.197 & 0.000 & 0.10 & 67,686 & 0.041 & 2.63 \\
4B teacher-solution start & 935 & 0.027 & 130 & 0.462 & 0.008 & 0.05 & 76,944 & 0.210 & 4.13 \\
\quad + thinking route & 465 & 0.058 & 49 & 0.265 & 0.000 & 0.31 & 60,663 & 0.071 & 2.28 \\
\quad + thinking route, 212 steps & 396 & 0.076 & 45 & 0.156 & 0.022 & 0.24 & 60,006 & 0.058 & 1.87 \\
\addlinespace[2pt]
1.7B short-solution start & 776 & 0.034 & 86 & 0.209 & 0.000 & 0.06 & 58,561 & 0.176 & 2.73 \\
\quad + thinking route & 1,090 & 0.049 & 127 & 0.386 & 0.039 & 0.12 & 62,128 & 0.149 & 3.01 \\
1.7B teacher-solution start & 1,448 & 0.075 & 207 & 0.396 & 0.019 & 0.03 & 86,171 & 0.270 & 2.79 \\
\quad + thinking route & 1,920 & 0.446 & 288 & 0.611 & 0.066 & 0.03 & 74,893 & 0.482 & 2.00 \\
\addlinespace[2pt]
0.6B short-solution start & 780 & 0.185 & 79 & 0.253 & 0.013 & 0.04 & 61,144 & 0.209 & 2.18 \\
\quad + thinking route & 1,355 & 0.088 & 165 & 0.145 & 0.012 & 0.25 & 55,217 & 0.450 & 2.47 \\
0.6B teacher-solution start & 1,602 & 0.036 & 231 & 0.216 & 0.022 & 0.02 & 89,054 & 0.277 & 2.62 \\
\quad + thinking route & 1,920 & 0.252 & 288 & 0.403 & 0.031 & 0.03 & 83,292 & 0.531 & 1.93 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 11 & 0.000 & 0 & -- & -- & -- & -- & 0.000 & 19.52 \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[p]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
{\small\textit{Table~\ref{tab:app-unfinished-bench}, continued.}}\par\medskip
\begin{tabular}{@{}lccccccccc@{}}
\toprule
& \multicolumn{2}{c}{truncated samples} & \multicolumn{5}{c}{is the correct value in the text?} & & \\
\cmidrule(lr){2-3}\cmidrule(lr){4-8}
Model & $n$ & \makecell{with a\\marked answer} & eligible & present & chance & \makecell{first\\at} & \makecell{characters\\after it} & loop & \makecell{\emph{Wait}/\emph{Hmm}\\per 1{,}000} \\
\midrule
\multicolumn{10}{@{}l}{\textbf{GSM8K-200}\quad 200 problems, 8{,}192-token cap} \\*
Teacher (thinking) & 58 & 0.207 & 30 & 0.367 & 0.033 & 0.31 & 22,524 & 0.103 & 6.00 \\
\addlinespace[2pt]
4B short-solution start & 144 & 0.111 & 28 & 0.500 & 0.143 & 0.05 & 30,088 & 0.090 & 5.62 \\
\quad + thinking route & 380 & 0.166 & 108 & 0.648 & 0.065 & 0.08 & 27,252 & 0.184 & 1.44 \\
4B teacher-solution start & 2,753 & 0.033 & 828 & 0.770 & 0.058 & 0.05 & 28,579 & 0.259 & 1.66 \\
\quad + thinking route & 347 & 0.303 & 99 & 0.515 & 0.081 & 0.11 & 23,259 & 0.196 & 1.63 \\
\quad + thinking route, 212 steps & 429 & 0.545 & 120 & 0.717 & 0.092 & 0.07 & 22,897 & 0.357 & 1.00 \\
\addlinespace[2pt]
1.7B short-solution start & 617 & 0.089 & 200 & 0.420 & 0.035 & 0.07 & 21,988 & 0.196 & 3.09 \\
\quad + thinking route & 1,215 & 0.093 & 437 & 0.618 & 0.059 & 0.10 & 23,958 & 0.256 & 2.11 \\
1.7B teacher-solution start & 4,114 & 0.112 & 1,234 & 0.614 & 0.055 & 0.05 & 26,865 & 0.331 & 1.82 \\
\quad + thinking route & 6,400 & 0.811 & 1,888 & 0.858 & 0.068 & 0.07 & 22,774 & 0.786 & 1.06 \\
\addlinespace[2pt]
0.6B short-solution start & 1,337 & 0.202 & 414 & 0.367 & 0.051 & 0.06 & 22,197 & 0.216 & 2.88 \\
\quad + thinking route & 1,863 & 0.170 & 626 & 0.557 & 0.075 & 0.19 & 20,354 & 0.129 & 2.62 \\
\quad + thinking route, 1{,}024-token budget$^\dagger$ & 427 & 0.382 & 133 & 0.632 & 0.030 & 0.07 & 24,245 & 0.539 & 2.04 \\
0.6B teacher-solution start & 4,849 & 0.072 & 1,436 & 0.476 & 0.044 & 0.05 & 25,518 & 0.332 & 2.32 \\
\quad + thinking route & 6,400 & 0.681 & 1,888 & 0.776 & 0.061 & 0.07 & 22,605 & 0.636 & 1.51 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 24 & 0.167 & 9 & 0.222 & 0.222 & 0.49 & 12,407 & 0.083 & 4.79 \\
\quad + 20 thinking steps (16{,}384-token budget)$^\dagger$ & 105 & 0.114 & 36 & 0.500 & 0.083 & 0.30 & 19,973 & 0.048 & 2.34 \\
\midrule
\multicolumn{10}{@{}l}{\textbf{Three benchmarks pooled}\quad all truncated samples of the three benchmarks together (Table~\ref{tab:unfinished})} \\*
Teacher (thinking) & 248 & 0.173 & 174 & 0.184 & 0.063 & 0.48 & 23,492 & 0.077 & 3.03 \\
\addlinespace[2pt]
4B short-solution start & 1,414 & 0.035 & 689 & 0.067 & 0.028 & 0.08 & 33,181 & 0.115 & 2.76 \\
\quad + thinking route & 1,638 & 0.066 & 835 & 0.211 & 0.049 & 0.21 & 29,796 & 0.084 & 2.09 \\
4B teacher-solution start & 4,775 & 0.029 & 1,782 & 0.430 & 0.037 & 0.06 & 29,676 & 0.224 & 2.78 \\
\quad + thinking route & 1,614 & 0.105 & 809 & 0.232 & 0.042 & 0.36 & 29,393 & 0.087 & 1.99 \\
\quad + thinking route, 212 steps & 1,589 & 0.190 & 810 & 0.257 & 0.059 & 0.30 & 26,027 & 0.133 & 1.52 \\
\addlinespace[2pt]
1.7B short-solution start & 2,343 & 0.047 & 1,024 & 0.126 & 0.024 & 0.07 & 25,693 & 0.163 & 2.81 \\
\quad + thinking route & 3,547 & 0.055 & 1,502 & 0.298 & 0.043 & 0.14 & 26,362 & 0.197 & 2.61 \\
1.7B teacher-solution start & 6,743 & 0.088 & 2,300 & 0.386 & 0.035 & 0.05 & 28,197 & 0.297 & 2.35 \\
\quad + thinking route & 9,760 & 0.640 & 3,232 & 0.614 & 0.053 & 0.07 & 23,486 & 0.650 & 1.45 \\
\addlinespace[2pt]
0.6B short-solution start & 2,923 & 0.178 & 1,122 & 0.169 & 0.036 & 0.06 & 23,474 & 0.202 & 2.47 \\
\quad + thinking route & 4,491 & 0.107 & 1,722 & 0.240 & 0.037 & 0.21 & 20,757 & 0.276 & 2.51 \\
\quad + thinking route, 1{,}024-token budget$^\dagger$ & 427 & 0.382 & 133 & 0.632 & 0.030 & 0.07 & 24,245 & 0.539 & 2.04 \\
0.6B teacher-solution start & 7,673 & 0.055 & 2,567 & 0.293 & 0.034 & 0.05 & 26,395 & 0.295 & 2.57 \\
\quad + thinking route & 9,760 & 0.506 & 3,232 & 0.506 & 0.045 & 0.07 & 22,972 & 0.567 & 1.67 \\
\addlinespace[2pt]
officially post-trained 0.6B$^\dagger$ & 65 & 0.169 & 39 & 0.128 & 0.128 & 0.67 & 20,529 & 0.154 & 7.26 \\
\quad + 20 thinking steps (16{,}384-token budget)$^\dagger$ & 105 & 0.114 & 36 & 0.500 & 0.083 & 0.30 & 19,973 & 0.048 & 2.34 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_unfinished_train.tex <==
\begin{table}[tbp]
\centering
\caption{\textbf{After the collapse, unfinished training rollouts are truncated rather than looping, and at 4B and for the
officially post-trained 0.6B they contain the correct answer far more often than chance.} Unclosed training
rollouts of three runs, in the first four steps and after the collapse (steps in parentheses). (a)~\emph{Truncated}:
the unclosed rollout reached the rollout budget (the rest stopped without closing). \emph{Eligible}: unclosed
rollouts on problems whose answer has at least three digits and does not appear in the statement; \emph{present}:
the fraction of those in which the correct value appears anywhere; \emph{by chance}: the same test with another
training problem's answer; \emph{first at}: median position of its first appearance as a fraction of the rollout.
(b)~\emph{Characters after it}: median characters written after that first appearance. Rates per 1{,}000
characters of \emph{Wait}, of checking phrases (\emph{let me check}, \emph{verify}, \emph{double-check}) and of
alternatives (\emph{alternatively}, \emph{another approach}); the fraction with an answer phrase (\emph{the answer
is}, \emph{final answer}) in the last 1{,}500 characters; \emph{ends in a loop}, the fraction in which some
non-empty line occurs at least five times in the last 2{,}000 characters (a different rule from the loop rate of
Table~\ref{tab:app-reflection}); and the number of rollouts that ended on their own without closing but with a
marked answer in their last 800 characters, a format defect of the cold start.}
\label{tab:app-unfinished-train}
\scriptsize
\setlength{\tabcolsep}{4pt}
{\small (a) Is the answer there?}\par\smallskip
\begin{tabular}{lcccccccc}
\toprule
& & & \multicolumn{2}{c}{unclosed} & \multicolumn{4}{c}{is the correct value in the unclosed rollout?} \\
\cmidrule(lr){4-5}\cmidrule(lr){6-9}
Phase & rollouts & closure & $n$ & truncated & eligible & present & by chance & first at \\
\midrule
\multicolumn{9}{l}{\textit{4B cold-started on short external solutions (run 2), 7,168-token budget}} \\
\quad steps 1--4 & 512 & 0.652 & 178 & 0.809 & 73 & 0.110 & 0.027 & 0.47 \\
\quad after the collapse (steps 10, 15, 20, 30) & 512 & 0.189 & 415 & 0.983 & 162 & 0.309 & 0.019 & 0.39 \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{0.6B cold-started on short external solutions (run 2), 7,168-token budget}} \\
\quad steps 1--4 & 512 & 0.586 & 212 & 0.245 & 78 & 0.064 & 0.013 & 0.39 \\
\quad after the collapse (steps 10, 15, 20, 30) & 512 & 0.041 & 491 & 0.957 & 183 & 0.055 & 0.022 & 0.50 \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{officially post-trained 0.6B, thinking template (run 2), 16,384-token budget}} \\
\quad steps 1--4 & 512 & 0.750 & 128 & 0.992 & 45 & 0.244 & 0.000 & 0.66 \\
\quad after the collapse (steps 10, 12, 15, 20) & 512 & 0.432 & 291 & 0.997 & 116 & 0.250 & 0.000 & 0.40 \\
\bottomrule
\end{tabular}
\par\medskip
{\small (b) What the rollout does after it}\par\smallskip
\begin{tabular}{lccccccc}
\toprule
& characters & \multicolumn{3}{c}{per 1{,}000 characters} & answer phrase & ends in & ended open, \\
\cmidrule(lr){3-5}
Phase & after it & \emph{Wait} & checks & alternatives & near the end & a loop & answer at end \\
\midrule
\multicolumn{7}{l}{\textit{4B cold-started on short external solutions (run 2), 7,168-token budget}} \\
\quad steps 1--4 & 9,517 & 2.39 & 0.14 & 0.44 & 0.213 & 0.039 & 29 \\
\quad after the collapse (steps 10, 15, 20, 30) & 10,720 & 1.88 & 0.41 & 0.61 & 0.116 & 0.002 & 3 \\
\addlinespace[3pt]
\multicolumn{7}{l}{\textit{0.6B cold-started on short external solutions (run 2), 7,168-token budget}} \\
\quad steps 1--4 & 4,886 & 1.94 & 0.15 & 0.23 & 0.387 & 0.123 & 109 \\
\quad after the collapse (steps 10, 15, 20, 30) & 9,231 & 4.09 & 0.26 & 0.59 & 0.081 & 0.008 & 3 \\
\addlinespace[3pt]
\multicolumn{7}{l}{\textit{officially post-trained 0.6B, thinking template (run 2), 16,384-token budget}} \\
\quad steps 1--4 & 17,610 & 1.41 & 0.33 & 0.81 & 0.047 & 0.008 & 0 \\
\quad after the collapse (steps 10, 12, 15, 20) & 23,424 & 1.85 & 0.25 & 0.48 & 0.065 & 0.003 & 0 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_val.tex <==
\begin{table}[p]
\centering
\caption{\textbf{In-training validation every 20 steps (the data behind Figure~\ref{fig:val}).} AIME 2025 (30 problems)
and AMC23 (40 problems), 8 samples each at temperature 0.6, with a 16{,}384-token cap, above the 7{,}168-token
rollout budget; values are pooled over the two benchmarks' 560 samples. (a)~Closure rate, thinking runs only
(every non-thinking run closes 1.00 by construction). (b)~Lenient accuracy: any marked answer in the sample is
correct. (c)~Strict accuracy: the sample closed its reasoning (thinking) or stopped before the cap
(non-thinking), and its answer is correct. (d)~Final answers per sample. \emph{End}: the run's last validation
step when it is not a multiple of 20, in parentheses. Cold-started on the teacher's own solutions, the 1.7B and
0.6B students' closure first rises and then falls to zero, and their strict accuracy with it, while their
lenient accuracy rises and then holds. Neighboring validations differ by a few hundredths through sampling
noise alone. These numbers were logged, not used: every evaluated checkpoint comes from a fixed step. The
16{,}384-token runs and the officially post-trained runs had no in-training validation. Rows and $\dagger$ as
in Table~\ref{tab:app-windows}.}
\label{tab:app-val}
\scriptsize
\setlength{\tabcolsep}{3pt}
{\small (a) Closure rate}\par\smallskip
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{11}{c}{training step} & end \\
\cmidrule(lr){2-12}
Run & 0 & 20 & 40 & 60 & 80 & 100 & 120 & 140 & 160 & 180 & 200 & (step) \\
\midrule
\multicolumn{13}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 0.68 & 0.40 & 0.43 & 0.44 & 0.43 & 0.48 & 0.46 & 0.50 & 0.48 & -- & -- & -- \\
\quad 4B, run 2$^\dagger$ & 0.63 & 0.43 & 0.44 & 0.44 & 0.45 & 0.51 & 0.45 & 0.48 & 0.50 & -- & -- & -- \\
\quad 1.7B & 0.47 & 0.18 & 0.22 & 0.25 & 0.25 & 0.27 & 0.26 & 0.27 & 0.26 & 0.27 & 0.27 & -- \\
\quad 0.6B, run 1 & 0.48 & 0.00 & 0.04 & 0.08 & -- & -- & -- & -- & -- & -- & -- & -- \\
\quad 0.6B, run 2$^\dagger$ & 0.45 & 0.01 & 0.04 & 0.11 & 0.11 & 0.09 & 0.07 & 0.09 & 0.14 & 0.12 & 0.10 & -- \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 0.38 & 0.29 & 0.36 & 0.38 & 0.46 & 0.45 & 0.48 & 0.46 & 0.48 & 0.49 & 0.49 & 0.52 (212) \\
\quad 1.7B & 0.54 & 0.80 & 0.14 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & -- & -- & -- & 0.00 (142) \\
\quad 0.6B & 0.53 & 0.70 & 0.08 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & -- & -- & -- & 0.00 (142) \\
\bottomrule
\end{tabular}
\par\medskip
{\small (b) Lenient accuracy}\par\smallskip
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{11}{c}{training step} & end \\
\cmidrule(lr){2-12}
Run & 0 & 20 & 40 & 60 & 80 & 100 & 120 & 140 & 160 & 180 & 200 & (step) \\
\midrule
\multicolumn{13}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 0.418 & 0.379 & 0.423 & 0.425 & 0.416 & 0.448 & 0.452 & 0.479 & 0.464 & -- & -- & -- \\
\quad 4B, run 2$^\dagger$ & 0.405 & 0.396 & 0.407 & 0.425 & 0.438 & 0.486 & 0.441 & 0.466 & 0.482 & -- & -- & -- \\
\quad 1.7B & 0.196 & 0.170 & 0.195 & 0.214 & 0.238 & 0.221 & 0.225 & 0.225 & 0.218 & 0.232 & 0.232 & -- \\
\quad 0.6B, run 1 & 0.105 & 0.027 & 0.079 & 0.098 & -- & -- & -- & -- & -- & -- & -- & -- \\
\quad 0.6B, run 2$^\dagger$ & 0.105 & 0.029 & 0.064 & 0.114 & 0.104 & 0.109 & 0.082 & 0.082 & 0.114 & 0.098 & 0.080 & -- \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 0.273 & 0.411 & 0.409 & 0.421 & 0.459 & 0.432 & 0.457 & 0.441 & 0.471 & 0.471 & 0.468 & 0.491 (212) \\
\quad 1.7B & 0.070 & 0.184 & 0.214 & 0.202 & 0.211 & 0.234 & 0.239 & 0.223 & -- & -- & -- & 0.202 (142) \\
\quad 0.6B & 0.020 & 0.048 & 0.098 & 0.095 & 0.105 & 0.096 & 0.084 & 0.118 & -- & -- & -- & 0.088 (142) \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Non-thinking route, pretrained-only start}} \\
\quad 4B & 0.268 & 0.393 & 0.389 & 0.389 & 0.425 & 0.386 & 0.430 & 0.413 & 0.398 & 0.421 & 0.409 & 0.386 (212) \\
\quad 1.7B & 0.141 & 0.230 & 0.252 & 0.232 & 0.243 & 0.243 & 0.254 & 0.259 & 0.288 & 0.255 & 0.245 & 0.271 (212) \\
\quad 0.6B & 0.025 & 0.139 & 0.146 & 0.150 & 0.166 & 0.159 & 0.152 & 0.170 & 0.173 & 0.150 & 0.179 & 0.187 (212) \\
\quad 4B, easy-to-hard curriculum & 0.229 & 0.373 & 0.402 & 0.395 & 0.400 & -- & -- & -- & -- & -- & -- & 0.421 (99) \\
\quad 1.7B, easy-to-hard curriculum & 0.146 & 0.245 & 0.252 & 0.262 & 0.248 & -- & -- & -- & -- & -- & -- & 0.273 (99) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[p]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
{\small\textit{Table~\ref{tab:app-val}, continued: in-training validation.}}\par\medskip
{\small (c) Strict accuracy}\par\smallskip
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{11}{c}{training step} & end \\
\cmidrule(lr){2-12}
Run & 0 & 20 & 40 & 60 & 80 & 100 & 120 & 140 & 160 & 180 & 200 & (step) \\
\midrule
\multicolumn{13}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 0.418 & 0.370 & 0.407 & 0.407 & 0.389 & 0.432 & 0.427 & 0.452 & 0.454 & -- & -- & -- \\
\quad 4B, run 2$^\dagger$ & 0.405 & 0.379 & 0.396 & 0.398 & 0.423 & 0.470 & 0.421 & 0.445 & 0.466 & -- & -- & -- \\
\quad 1.7B & 0.191 & 0.157 & 0.182 & 0.188 & 0.221 & 0.214 & 0.211 & 0.211 & 0.198 & 0.223 & 0.221 & -- \\
\quad 0.6B, run 1 & 0.082 & 0.000 & 0.027 & 0.059 & -- & -- & -- & -- & -- & -- & -- & -- \\
\quad 0.6B, run 2$^\dagger$ & 0.089 & 0.009 & 0.032 & 0.075 & 0.071 & 0.068 & 0.052 & 0.064 & 0.096 & 0.077 & 0.068 & -- \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 0.175 & 0.261 & 0.330 & 0.345 & 0.412 & 0.407 & 0.437 & 0.430 & 0.457 & 0.439 & 0.455 & 0.471 (212) \\
\quad 1.7B & 0.030 & 0.121 & 0.046 & 0.004 & 0.000 & 0.000 & 0.000 & 0.000 & -- & -- & -- & 0.000 (142) \\
\quad 0.6B & 0.011 & 0.029 & 0.004 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & -- & -- & -- & 0.000 (142) \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Non-thinking route, pretrained-only start}} \\
\quad 4B & 0.268 & 0.393 & 0.389 & 0.389 & 0.423 & 0.386 & 0.430 & 0.411 & 0.398 & 0.409 & 0.396 & 0.375 (212) \\
\quad 1.7B & 0.141 & 0.227 & 0.252 & 0.232 & 0.243 & 0.239 & 0.252 & 0.257 & 0.284 & 0.255 & 0.243 & 0.268 (212) \\
\quad 0.6B & 0.025 & 0.138 & 0.145 & 0.146 & 0.161 & 0.157 & 0.148 & 0.168 & 0.170 & 0.148 & 0.179 & 0.186 (212) \\
\quad 4B, easy-to-hard curriculum & 0.229 & 0.370 & 0.398 & 0.393 & 0.398 & -- & -- & -- & -- & -- & -- & 0.421 (99) \\
\quad 1.7B, easy-to-hard curriculum & 0.145 & 0.241 & 0.246 & 0.262 & 0.245 & -- & -- & -- & -- & -- & -- & 0.271 (99) \\
\bottomrule
\end{tabular}
\par\medskip
{\small (d) Final answers per sample}\par\smallskip
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{11}{c}{training step} & end \\
\cmidrule(lr){2-12}
Run & 0 & 20 & 40 & 60 & 80 & 100 & 120 & 140 & 160 & 180 & 200 & (step) \\
\midrule
\multicolumn{13}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 3.3 & 1.0 & 1.3 & 1.2 & 1.1 & 1.2 & 1.3 & 1.4 & 1.3 & -- & -- & -- \\
\quad 4B, run 2$^\dagger$ & 1.8 & 1.1 & 1.3 & 1.2 & 1.2 & 1.4 & 1.2 & 1.3 & 1.4 & -- & -- & -- \\
\quad 1.7B & 1.7 & 0.5 & 0.6 & 0.8 & 1.5 & 1.0 & 1.2 & 0.9 & 1.3 & 1.5 & 1.8 & -- \\
\quad 0.6B, run 1 & 11.6 & 0.4 & 1.6 & 1.1 & -- & -- & -- & -- & -- & -- & -- & -- \\
\quad 0.6B, run 2$^\dagger$ & 10.0 & 0.6 & 0.2 & 0.5 & 0.4 & 0.6 & 0.4 & 0.4 & 0.5 & 0.5 & 0.4 & -- \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 0.9 & 1.9 & 2.1 & 1.5 & 1.6 & 1.4 & 1.4 & 1.3 & 1.3 & 1.4 & 1.4 & 1.5 (212) \\
\quad 1.7B & 0.7 & 56.9 & 41.7 & 27.7 & 34.3 & 120.6 & 75.9 & 61.4 & -- & -- & -- & 32.9 (142) \\
\quad 0.6B & 2.8 & 10.2 & 22.1 & 34.1 & 38.3 & 42.9 & 39.9 & 48.0 & -- & -- & -- & 31.7 (142) \\
\addlinespace[3pt]
\multicolumn{13}{l}{\textit{Non-thinking route, pretrained-only start}} \\
\quad 4B & 0.8 & 8.3 & 4.9 & 3.1 & 6.1 & 7.3 & 15.1 & 7.1 & 28.0 & 293.3 & 254.3 & 135.2 (212) \\
\quad 1.7B & 0.7 & 7.0 & 5.1 & 8.8 & 6.0 & 10.9 & 6.5 & 5.2 & 14.2 & 7.8 & 15.9 & 11.1 (212) \\
\quad 0.6B & 8.7 & 8.5 & 5.0 & 12.2 & 11.7 & 15.0 & 7.1 & 6.8 & 9.3 & 8.7 & 9.4 & 7.3 (212) \\
\quad 4B, easy-to-hard curriculum & 3.5 & 18.1 & 2.8 & 3.6 & 5.1 & -- & -- & -- & -- & -- & -- & 8.8 (99) \\
\quad 1.7B, easy-to-hard curriculum & 0.8 & 7.9 & 5.8 & 6.4 & 6.8 & -- & -- & -- & -- & -- & -- & 8.3 (99) \\
\bottomrule
\end{tabular}
\end{table}



==> tables/app_windows.tex <==
\begin{table}[p]
\centering
\caption{\textbf{Closure, stop precision and committed accuracy on training rollouts, by step window, for every run.}
Means over the student's own training rollouts (one sample for each of 128 prompts per step); rollout budget
7{,}168 tokens unless the row says otherwise. (a)~Closure rate, the fraction of rollouts that emit \think.
\emph{Steps 1--4}: its mean over the first four steps; \emph{onset}: the first later step at which it falls
below 0.75 times that mean; \emph{last step}: the last logged step, where the last window ends. Closure
crosses that line at step~6 in every 7{,}168-token run cold-started on short external solutions and in both
officially post-trained runs, and at step~7 with a 16{,}384-token budget; the runs cold-started on the
teacher's own solutions and the 1{,}024-token run start low. Non-thinking runs have no closure to lose (the
thinking block is closed in the prompt). (b)~Stop precision: closed and correct divided by closed, thinking
runs only; committed accuracy: the last marked answer in the rollout is correct, closed or not. Where two runs
exist, $\dagger$ marks the run whose checkpoint is evaluated in the main text; the two runs used the same data
order (Appendix~\ref{app:notes}).}
\label{tab:app-windows}
\scriptsize
\setlength{\tabcolsep}{4pt}
{\small (a) Closure rate}\par\smallskip
\begin{tabular}{lcccccccc}
\toprule
& last & steps & onset & \multicolumn{5}{c}{training steps} \\
\cmidrule(lr){5-9}
Run & step & 1--4 & step & 1--5 & 6--20 & 21--50 & 51--100 & 101--212 \\
\midrule
\multicolumn{9}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 170 & 0.648 & 6 & 0.617 & 0.173 & 0.201 & 0.218 & 0.226 \\
\quad 4B, run 2$^\dagger$ & 167 & 0.652 & 6 & 0.633 & 0.182 & 0.207 & 0.205 & 0.226 \\
\quad 1.7B & 212 & 0.459 & 6 & 0.445 & 0.090 & 0.053 & 0.057 & 0.064 \\
\quad 0.6B, run 1 & 80 & 0.611 & 6 & 0.605 & 0.087 & 0.034 & 0.025 & -- \\
\quad 0.6B, run 2$^\dagger$ & 212 & 0.586 & 6 & 0.583 & 0.074 & 0.035 & 0.021 & 0.026 \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 212 & 0.219 & 11 & 0.225 & 0.173 & 0.151 & 0.174 & 0.211 \\
\quad 1.7B & 142 & 0.078 & 6 & 0.078 & 0.037 & 0.032 & 0.012 & 0.003 \\
\quad 0.6B & 142 & 0.119 & 6 & 0.117 & 0.045 & 0.048 & 0.011 & 0.003 \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{0.6B cold-started on short external solutions, other rollout budgets}} \\
\quad 1,024-token budget & 212 & 0.135 & 5 & 0.125 & 0.089 & 0.045 & 0.021 & 0.006 \\
\quad 16,384-token budget & 7 & 0.604 & 7 & 0.608 & 0.297 & -- & -- & -- \\
\addlinespace[3pt]
\multicolumn{9}{l}{\textit{Officially post-trained 0.6B, 16,384-token budget}} \\
\quad thinking template, run 1 & 20 & 0.756 & 6 & 0.736 & 0.397 & -- & -- & -- \\
\quad thinking template, run 2$^\dagger$ & 20 & 0.750 & 6 & 0.731 & 0.414 & -- & -- & -- \\
\bottomrule
\end{tabular}
\par\medskip
{\small (b) Stop precision and committed accuracy}\par\smallskip
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{5}{c}{stop precision, P(correct $\mid$ closed)} & \multicolumn{5}{c}{committed accuracy} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
Run & 1--5 & 6--20 & 21--50 & 51--100 & 101--212 & 1--5 & 6--20 & 21--50 & 51--100 & 101--212 \\
\midrule
\multicolumn{11}{l}{\textit{Thinking route, cold-started on short external solutions}} \\
\quad 4B, run 1 & 0.527 & 0.643 & 0.640 & 0.658 & 0.669 & 0.366 & 0.154 & 0.187 & 0.193 & 0.208 \\
\quad 4B, run 2$^\dagger$ & 0.509 & 0.614 & 0.664 & 0.652 & 0.677 & 0.358 & 0.168 & 0.186 & 0.188 & 0.203 \\
\quad 1.7B & 0.123 & 0.162 & 0.384 & 0.416 & 0.458 & 0.095 & 0.031 & 0.039 & 0.042 & 0.052 \\
\quad 0.6B, run 1 & 0.039 & 0.036 & 0.031 & 0.158 & -- & 0.042 & 0.006 & 0.003 & 0.010 & -- \\
\quad 0.6B, run 2$^\dagger$ & 0.032 & 0.028 & 0.015 & 0.125 & 0.177 & 0.033 & 0.007 & 0.003 & 0.007 & 0.010 \\
\addlinespace[3pt]
\multicolumn{11}{l}{\textit{Thinking route, cold-started on the teacher's own solutions}} \\
\quad 4B & 0.222 & 0.345 & 0.525 & 0.603 & 0.657 & 0.147 & 0.158 & 0.187 & 0.204 & 0.214 \\
\quad 1.7B & 0.020 & 0.056 & 0.106 & 0.063 & 0.187 & 0.056 & 0.058 & 0.054 & 0.048 & 0.053 \\
\quad 0.6B & 0.000 & 0.000 & 0.005 & 0.015 & 0.067 & 0.020 & 0.012 & 0.008 & 0.011 & 0.011 \\
\addlinespace[3pt]
\multicolumn{11}{l}{\textit{0.6B cold-started on short external solutions, other rollout budgets}} \\
\quad 1,024-token budget & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.003 & 0.001 & 0.000 & 0.000 \\
\quad 16,384-token budget & 0.041 & 0.026 & -- & -- & -- & 0.033 & 0.019 & -- & -- & -- \\
\addlinespace[3pt]
\multicolumn{11}{l}{\textit{Officially post-trained 0.6B, 16,384-token budget}} \\
\quad thinking template, run 1 & 0.346 & 0.659 & -- & -- & -- & 0.259 & 0.286 & -- & -- & -- \\
\quad thinking template, run 2$^\dagger$ & 0.374 & 0.668 & -- & -- & -- & 0.277 & 0.297 & -- & -- & -- \\
\quad non-thinking template & -- & -- & -- & -- & -- & 0.086 & 0.167 & -- & -- & -- \\
\addlinespace[3pt]
\multicolumn{11}{l}{\textit{Non-thinking route, pretrained-only start}} \\
\quad 4B & -- & -- & -- & -- & -- & 0.089 & 0.249 & 0.364 & 0.352 & 0.369 \\
\quad 1.7B & -- & -- & -- & -- & -- & 0.020 & 0.104 & 0.182 & 0.201 & 0.209 \\
\quad 0.6B & -- & -- & -- & -- & -- & 0.009 & 0.044 & 0.090 & 0.095 & 0.105 \\
\quad 4B, easy-to-hard curriculum & -- & -- & -- & -- & -- & 0.303 & 0.630 & 0.488 & 0.103 & -- \\
\quad 1.7B, easy-to-hard curriculum & -- & -- & -- & -- & -- & 0.106 & 0.234 & 0.197 & 0.059 & -- \\
\bottomrule
\end{tabular}
\end{table}



==> tables/lean_perbench.tex <==
\begin{table}[h]
\centering
\footnotesize
\caption{\textbf{Lenient scores per benchmark.} p@1 and p@n for every evaluated model; the last two columns are the
unweighted mean used in the main text. Starting points in gray.}
\label{tab:app-perbench}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
 & \multicolumn{2}{c}{AIME 2026} & \multicolumn{2}{c}{AMC23} & \multicolumn{2}{c}{GSM8K-200} & \multicolumn{2}{c}{Mean} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
Model & p@1 & p@n & p@1 & p@n & p@1 & p@n & p@1 & p@n \\
\midrule
Teacher (thinking) & 0.674 & 0.900 & 0.960 & 1.000 & 0.937 & 0.965 & 0.857 & 0.955 \\
Teacher (non-thinking) & 0.163 & 0.667 & 0.694 & 0.975 & 0.929 & 0.965 & 0.595 & 0.869 \\
\midrule
\textcolor{cMuted}{4B pretrained-only} & \textcolor{cMuted}{0.083} & \textcolor{cMuted}{0.333} & \textcolor{cMuted}{0.438} & \textcolor{cMuted}{0.900} & \textcolor{cMuted}{0.761} & \textcolor{cMuted}{0.975} & \textcolor{cMuted}{0.427} & \textcolor{cMuted}{0.736} \\
\quad + non-thinking route & 0.141 & 0.467 & 0.587 & 0.925 & 0.919 & 0.980 & 0.549 & 0.791 \\
\textcolor{cMuted}{4B short-solution start} & \textcolor{cMuted}{0.148} & \textcolor{cMuted}{0.400} & \textcolor{cMuted}{0.548} & \textcolor{cMuted}{0.925} & \textcolor{cMuted}{0.899} & \textcolor{cMuted}{0.980} & \textcolor{cMuted}{0.532} & \textcolor{cMuted}{0.768} \\
\quad + thinking-mode distillation & 0.329 & 0.700 & 0.728 & 0.900 & 0.896 & 0.965 & 0.651 & 0.855 \\
\textcolor{cMuted}{4B teacher-solution start} & \textcolor{cMuted}{0.116} & \textcolor{cMuted}{0.400} & \textcolor{cMuted}{0.412} & \textcolor{cMuted}{0.900} & \textcolor{cMuted}{0.461} & \textcolor{cMuted}{0.945} & \textcolor{cMuted}{0.330} & \textcolor{cMuted}{0.748} \\
\quad + thinking-mode distillation & 0.316 & 0.733 & 0.728 & 0.950 & 0.903 & 0.965 & 0.649 & 0.883 \\
\midrule
\textcolor{cMuted}{1.7B pretrained-only} & \textcolor{cMuted}{0.014} & \textcolor{cMuted}{0.133} & \textcolor{cMuted}{0.266} & \textcolor{cMuted}{0.825} & \textcolor{cMuted}{0.601} & \textcolor{cMuted}{0.980} & \textcolor{cMuted}{0.294} & \textcolor{cMuted}{0.646} \\
\quad + non-thinking route & 0.079 & 0.300 & 0.410 & 0.900 & 0.830 & 0.975 & 0.440 & 0.725 \\
\textcolor{cMuted}{1.7B short-solution start} & \textcolor{cMuted}{0.029} & \textcolor{cMuted}{0.233} & \textcolor{cMuted}{0.299} & \textcolor{cMuted}{0.775} & \textcolor{cMuted}{0.747} & \textcolor{cMuted}{0.985} & \textcolor{cMuted}{0.358} & \textcolor{cMuted}{0.664} \\
\quad + thinking-mode distillation & 0.057 & 0.200 & 0.362 & 0.725 & 0.757 & 0.960 & 0.392 & 0.628 \\
\textcolor{cMuted}{1.7B teacher-solution start} & \textcolor{cMuted}{0.013} & \textcolor{cMuted}{0.100} & \textcolor{cMuted}{0.129} & \textcolor{cMuted}{0.550} & \textcolor{cMuted}{0.243} & \textcolor{cMuted}{0.900} & \textcolor{cMuted}{0.128} & \textcolor{cMuted}{0.517} \\
\quad + thinking-mode distillation & 0.067 & 0.233 & 0.372 & 0.675 & 0.743 & 0.950 & 0.394 & 0.619 \\
\midrule
\textcolor{cMuted}{0.6B pretrained-only} & \textcolor{cMuted}{0.004} & \textcolor{cMuted}{0.167} & \textcolor{cMuted}{0.053} & \textcolor{cMuted}{0.625} & \textcolor{cMuted}{0.087} & \textcolor{cMuted}{0.745} & \textcolor{cMuted}{0.048} & \textcolor{cMuted}{0.512} \\
\quad + non-thinking route & 0.018 & 0.133 & 0.278 & 0.700 & 0.689 & 0.945 & 0.328 & 0.593 \\
\textcolor{cMuted}{0.6B short-solution start} & \textcolor{cMuted}{0.006} & \textcolor{cMuted}{0.167} & \textcolor{cMuted}{0.173} & \textcolor{cMuted}{0.675} & \textcolor{cMuted}{0.536} & \textcolor{cMuted}{0.930} & \textcolor{cMuted}{0.238} & \textcolor{cMuted}{0.591} \\
\quad + thinking-mode distillation & 0.004 & 0.067 & 0.212 & 0.600 & 0.667 & 0.895 & 0.294 & 0.521 \\
\textcolor{cMuted}{0.6B teacher-solution start} & \textcolor{cMuted}{0.001} & \textcolor{cMuted}{0.033} & \textcolor{cMuted}{0.029} & \textcolor{cMuted}{0.400} & \textcolor{cMuted}{0.135} & \textcolor{cMuted}{0.765} & \textcolor{cMuted}{0.055} & \textcolor{cMuted}{0.399} \\
\quad + thinking-mode distillation & 0.003 & 0.067 & 0.165 & 0.475 & 0.620 & 0.880 & 0.262 & 0.474 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/tab1_main.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Distilling the thinking teacher raises accuracy given a marked answer at every size, but
from short external solutions the answer rate holds only at 4B.} Three-benchmark means; gray rows are
starting points. Lenient: any marked answer is correct; strict: correct and closed
(non-thinking: stopped before the cap); maj@$n$: majority vote over last answers. Per benchmark, committed
scoring and intervals: Appendices~\ref{app:perbench} and~\ref{app:ci}.}
\label{tab:main}
\footnotesize
\setlength{\tabcolsep}{4.8pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
 & \multicolumn{2}{c}{Two factors} & \multicolumn{2}{c}{Lenient} & Vote & Strict & \multicolumn{2}{c}{Stopping} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-9}
 & \makecell{Answer\\rate} & \makecell{Accuracy given\\an answer} & $p@1$ & $p@n$ & maj@$n$ & $p@1$ & Closure & Trunc. \\
\midrule
Teacher (thinking) & 0.962 & 0.887 & 0.857 & 0.955 & 0.905 & 0.852 & 0.962 & 0.045 \\
Teacher (non-thinking) & 0.969 & 0.604 & 0.595 & 0.869 & 0.655 & 0.594 & -- & 0.037 \\
\midrule
\textcolor{cMuted}{\textit{4B pretrained-only}} & \textcolor{cMuted}{0.830} & \textcolor{cMuted}{0.502} & \textcolor{cMuted}{0.427} & \textcolor{cMuted}{0.736} & \textcolor{cMuted}{0.553} & \textcolor{cMuted}{0.426} & \textcolor{cMuted}{--} & \textcolor{cMuted}{0.133} \\
4B non-thinking route & 0.946 & 0.563 & 0.549 & 0.791 & 0.599 & 0.505 & -- & 0.242 \\
\addlinespace[1.5pt]
\textcolor{cMuted}{\textit{4B external-SFT start}} & \textcolor{cMuted}{0.734} & \textcolor{cMuted}{0.653} & \textcolor{cMuted}{0.532} & \textcolor{cMuted}{0.768} & \textcolor{cMuted}{0.656} & \textcolor{cMuted}{0.529} & \textcolor{cMuted}{0.726} & \textcolor{cMuted}{0.274} \\
\quad + thinking route & 0.728 & 0.866 & 0.651 & 0.855 & 0.792 & 0.645 & 0.725 & 0.284 \\
\addlinespace[1.5pt]
\textcolor{cMuted}{\textit{4B teacher-SFT start}} & \textcolor{cMuted}{0.366} & \textcolor{cMuted}{0.848} & \textcolor{cMuted}{0.330} & \textcolor{cMuted}{0.748} & \textcolor{cMuted}{0.678} & \textcolor{cMuted}{0.227} & \textcolor{cMuted}{0.333} & \textcolor{cMuted}{0.557} \\
\quad + thinking route & 0.734 & 0.852 & 0.649 & 0.883 & 0.801 & 0.636 & 0.732 & 0.284 \\
\midrule
\textcolor{cMuted}{\textit{1.7B pretrained-only}} & \textcolor{cMuted}{0.752} & \textcolor{cMuted}{0.376} & \textcolor{cMuted}{0.294} & \textcolor{cMuted}{0.646} & \textcolor{cMuted}{0.481} & \textcolor{cMuted}{0.294} & \textcolor{cMuted}{--} & \textcolor{cMuted}{0.145} \\
1.7B non-thinking route & 0.886 & 0.462 & 0.440 & 0.725 & 0.519 & 0.437 & -- & 0.141 \\
\addlinespace[1.5pt]
\textcolor{cMuted}{\textit{1.7B external-SFT start}} & \textcolor{cMuted}{0.627} & \textcolor{cMuted}{0.464} & \textcolor{cMuted}{0.358} & \textcolor{cMuted}{0.664} & \textcolor{cMuted}{0.502} & \textcolor{cMuted}{0.339} & \textcolor{cMuted}{0.585} & \textcolor{cMuted}{0.387} \\
\quad + thinking route & 0.482 & 0.688 & 0.392 & 0.628 & 0.511 & 0.372 & 0.451 & 0.540 \\
\addlinespace[1.5pt]
\textcolor{cMuted}{\textit{1.7B teacher-SFT start}} & \textcolor{cMuted}{0.151} & \textcolor{cMuted}{0.706} & \textcolor{cMuted}{0.128} & \textcolor{cMuted}{0.517} & \textcolor{cMuted}{0.483} & \textcolor{cMuted}{0.066} & \textcolor{cMuted}{0.397} & \textcolor{cMuted}{0.739} \\
\quad + thinking route & 0.466 & 0.745 & 0.394 & 0.619 & 0.548 & 0.000 & 0.000 & 1.000 \\
\midrule
\textcolor{cMuted}{\textit{0.6B pretrained-only}} & \textcolor{cMuted}{0.194} & \textcolor{cMuted}{0.266} & \textcolor{cMuted}{0.048} & \textcolor{cMuted}{0.512} & \textcolor{cMuted}{0.344} & \textcolor{cMuted}{0.046} & \textcolor{cMuted}{--} & \textcolor{cMuted}{0.781} \\
0.6B non-thinking route & 0.827 & 0.350 & 0.328 & 0.593 & 0.449 & 0.327 & -- & 0.199 \\
\addlinespace[1.5pt]
\textcolor{cMuted}{\textit{0.6B external-SFT start}} & \textcolor{cMuted}{0.672} & \textcolor{cMuted}{0.304} & \textcolor{cMuted}{0.238} & \textcolor{cMuted}{0.591} & \textcolor{cMuted}{0.400} & \textcolor{cMuted}{0.201} & \textcolor{cMuted}{0.556} & \textcolor{cMuted}{0.392} \\
\quad + thinking route & 0.421 & 0.499 & 0.294 & 0.521 & 0.398 & 0.251 & 0.340 & 0.627 \\
\addlinespace[1.5pt]
\textcolor{cMuted}{\textit{0.6B teacher-SFT start}} & \textcolor{cMuted}{0.089} & \textcolor{cMuted}{0.425} & \textcolor{cMuted}{0.055} & \textcolor{cMuted}{0.399} & \textcolor{cMuted}{0.320} & \textcolor{cMuted}{0.031} & \textcolor{cMuted}{0.323} & \textcolor{cMuted}{0.814} \\
\quad + thinking route & 0.333 & 0.535 & 0.262 & 0.474 & 0.400 & 0.000 & 0.000 & 1.000 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/tab3_capacity.tex <==
\begin{table}[t]
\centering
\caption{\textbf{The share of the mode-matched teacher falls as the student shrinks, on every readout
and in both modes; only at 4B is coverage ($p@n$) unchanged by the teacher's mode.} (a) Student score over
teacher score (gray row), three-benchmark mean; a smaller share of the stronger thinking teacher is not a
lower score. (b) Per-token divergence, fitted as $c+a\,e^{-t/\tau}$; accuracy on training
problems the teacher solved 4/4.}
\label{tab:capacity}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{}lccccccccc@{}}
\multicolumn{10}{@{}l}{\textbf{(a)} Share of the mode-matched teacher} \\[1pt]
\toprule
 & \multicolumn{3}{c}{Non-thinking route} & \multicolumn{3}{c}{\makecell{Thinking route,\\external-SFT start}} & \multicolumn{3}{c}{\makecell{Thinking route,\\teacher-SFT start}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Student & $p@1$ & $p@n$ & maj@$n$ & $p@1$ & $p@n$ & maj@$n$ & $p@1$ & $p@n$ & maj@$n$ \\
\midrule
4B & 0.922 & 0.910 & 0.914 & 0.760 & 0.895 & 0.875 & 0.757 & 0.924 & 0.885 \\
1.7B & 0.739 & 0.834 & 0.793 & 0.458 & 0.658 & 0.565 & 0.460 & 0.649 & 0.606 \\
0.6B & 0.551 & 0.682 & 0.685 & 0.343 & 0.545 & 0.440 & 0.306 & 0.496 & 0.442 \\
\midrule
\textcolor{cMuted}{\textit{Teacher score}} & \textcolor{cMuted}{0.595} & \textcolor{cMuted}{0.869} & \textcolor{cMuted}{0.655} & \textcolor{cMuted}{0.857} & \textcolor{cMuted}{0.955} & \textcolor{cMuted}{0.905} & \textcolor{cMuted}{0.857} & \textcolor{cMuted}{0.955} & \textcolor{cMuted}{0.905} \\
\bottomrule
\end{tabular}
\par\vspace{5pt}
\begin{tabular}{@{}lccc@{}}
\multicolumn{4}{@{}l}{\textbf{(b)} The non-thinking route against its teacher} \\[1pt]
\toprule
Student & \makecell{Divergence floor $c$\\{[}95\% CI{]}} & \makecell{Time constant\\$\tau$ (steps)} & \makecell{Accuracy on problems\\the teacher solved 4/4} \\
\midrule
4B & 0.161 [0.159, 0.162] & 6.0 & 0.756 \\
1.7B & 0.254 [0.252, 0.255] & 8.4 & 0.485 \\
0.6B & 0.341 [0.338, 0.343] & 8.5 & 0.224 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/tab_ceiling.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Distillation raises lenient $p@1$ toward the student's own starting $p@n$ but never past
it; the share of the mode-matched teacher falls with size.} Lenient scoring, three-benchmark mean; $p@n$ over
$n=48$ samples (AIME 2026, AMC23) or 32 (GSM8K-200). Difference: paired problem bootstrap, 95\% interval. Gray:
the starting point. Per benchmark: Table~\ref{tab:app-ceiling}.}
\label{tab:ceiling}
\footnotesize
\setlength{\tabcolsep}{4.6pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
 & \multicolumn{2}{c}{Start} & \multicolumn{2}{c}{After distillation} & \multicolumn{2}{c}{After $p@1$ against start $p@n$} & \multicolumn{2}{c}{\makecell{Share of the\\mode-matched teacher}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
Student & $p@1$ & $p@n$ & $p@1$ & $p@n$ & ratio & difference [95\% CI] & $p@1$ & $p@n$ \\
\midrule
\multicolumn{9}{@{}l}{\textit{Non-thinking route}\enspace\textcolor{cMuted}{(non-thinking teacher: $p@1$ 0.595, $p@n$ 0.869)}} \\
\quad 4B & \textcolor{cMuted}{0.427} & \textcolor{cMuted}{0.736} & 0.549 & 0.791 & 0.75 & $-0.187$\,{\scriptsize$[-0.246, -0.133]$} & 0.922 & 0.910 \\
\quad 1.7B & \textcolor{cMuted}{0.294} & \textcolor{cMuted}{0.646} & 0.440 & 0.725 & 0.68 & $-0.206$\,{\scriptsize$[-0.255, -0.160]$} & 0.739 & 0.834 \\
\quad 0.6B & \textcolor{cMuted}{0.048} & \textcolor{cMuted}{0.512} & 0.328 & 0.593 & 0.64 & $-0.184$\,{\scriptsize$[-0.247, -0.126]$} & 0.551 & 0.682 \\
\addlinespace[3pt]
\multicolumn{9}{@{}l}{\textit{Thinking mode, external-SFT start}\enspace\textcolor{cMuted}{(thinking teacher: $p@1$ 0.857, $p@n$ 0.955)}} \\
\quad 4B & \textcolor{cMuted}{0.532} & \textcolor{cMuted}{0.768} & 0.651 & 0.855 & 0.85 & $-0.117$\,{\scriptsize$[-0.165, -0.074]$} & 0.760 & 0.895 \\
\quad 1.7B & \textcolor{cMuted}{0.358} & \textcolor{cMuted}{0.664} & 0.392 & 0.628 & 0.59 & $-0.272$\,{\scriptsize$[-0.335, -0.212]$} & 0.458 & 0.658 \\
\quad 0.6B & \textcolor{cMuted}{0.238} & \textcolor{cMuted}{0.591} & 0.294 & 0.521 & 0.50 & $-0.296$\,{\scriptsize$[-0.365, -0.234]$} & 0.343 & 0.545 \\
\addlinespace[3pt]
\multicolumn{9}{@{}l}{\textit{Thinking mode, teacher-SFT start}\enspace\textcolor{cMuted}{(thinking teacher: $p@1$ 0.857, $p@n$ 0.955)}} \\
\quad 4B & \textcolor{cMuted}{0.330} & \textcolor{cMuted}{0.748} & 0.649 & 0.883 & 0.87 & $-0.099$\,{\scriptsize$[-0.146, -0.058]$} & 0.757 & 0.924 \\
\quad 1.7B & \textcolor{cMuted}{0.128} & \textcolor{cMuted}{0.517} & 0.394 & 0.619 & 0.76 & $-0.123$\,{\scriptsize$[-0.166, -0.083]$} & 0.460 & 0.649 \\
\quad 0.6B & \textcolor{cMuted}{0.055} & \textcolor{cMuted}{0.399} & 0.262 & 0.474 & 0.66 & $-0.137$\,{\scriptsize$[-0.186, -0.092]$} & 0.306 & 0.496 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/tab_nonthinking.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Distilling the non-thinking teacher helps at every size, on the open-ended mean and
on GPQA-Diamond, where only the distilled 4B clears chance (0.250).} Each cell: pretrained-only start (gray)
$\to$ after 212 steps, with the non-thinking teacher beside; changes with paired bootstrap 95\% intervals
(Appendix~\ref{app:ci}). GPQA-Diamond is multiple choice, so it is scored on the last answer only
(Appendix~\ref{app:scoring}), at a 16{,}384-token cap.}
\label{tab:nonthinking}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{}lcccc@{}}
\toprule
 & 4B & 1.7B & 0.6B & Teacher \\
\midrule
\multicolumn{5}{@{}l}{\textit{Open-ended benchmarks, lenient $p@1$}} \\
\quad AIME 2026 & \textcolor{cMuted}{0.083} $\to$ 0.141 & \textcolor{cMuted}{0.014} $\to$ 0.079 & \textcolor{cMuted}{0.004} $\to$ 0.018 & 0.163 \\
\quad AMC23 & \textcolor{cMuted}{0.438} $\to$ 0.587 & \textcolor{cMuted}{0.266} $\to$ 0.410 & \textcolor{cMuted}{0.053} $\to$ 0.278 & 0.694 \\
\quad GSM8K-200 & \textcolor{cMuted}{0.761} $\to$ 0.919 & \textcolor{cMuted}{0.601} $\to$ 0.830 & \textcolor{cMuted}{0.087} $\to$ 0.689 & 0.929 \\
\quad Mean & \textcolor{cMuted}{0.427} $\to$ 0.549 & \textcolor{cMuted}{0.294} $\to$ 0.440 & \textcolor{cMuted}{0.048} $\to$ 0.328 & 0.595 \\
\quad\quad change & $+0.121$\,{\scriptsize$[+0.097, +0.149]$} & $+0.146$\,{\scriptsize$[+0.118, +0.177]$} & $+0.280$\,{\scriptsize$[+0.249, +0.310]$} &  \\
\addlinespace[2pt]
\multicolumn{5}{@{}l}{\textit{GPQA-Diamond}} \\
\quad Committed $p@1$ & \textcolor{cMuted}{0.157} $\to$ 0.397 & \textcolor{cMuted}{0.191} $\to$ 0.275 & \textcolor{cMuted}{0.049} $\to$ 0.234 & 0.499 \\
\quad\quad change & $+0.239$\,{\scriptsize$[+0.198, +0.282]$} & $+0.084$\,{\scriptsize$[+0.050, +0.117]$} & $+0.185$\,{\scriptsize$[+0.155, +0.215]$} &  \\
\quad Strict $p@1$ & \textcolor{cMuted}{0.157} $\to$ 0.361 & \textcolor{cMuted}{0.189} $\to$ 0.270 & \textcolor{cMuted}{0.049} $\to$ 0.233 & 0.497 \\
\quad\quad change & $+0.204$\,{\scriptsize$[+0.163, +0.247]$} & $+0.081$\,{\scriptsize$[+0.048, +0.114]$} & $+0.184$\,{\scriptsize$[+0.155, +0.214]$} &  \\
\quad Truncated & \textcolor{cMuted}{0.462} $\to$ 0.125 & \textcolor{cMuted}{0.181} $\to$ 0.111 & \textcolor{cMuted}{0.581} $\to$ 0.154 & 0.026 \\
\bottomrule
\end{tabular}
\end{table}


